Physical Parameters of Stars in NGC 6397 Using ANN-Based Interpolation and Full Spectrum Fitting

Stellar spectral interpolation is critical technique employed by fitting software to derive the physical parameters of stars. This approach is necessary because on-the-go generation of synthetic stellar spectra is not possible due to the complex and high cost of computation. The goal of this study is to develop a spectral interpolator for a synthetic spectral library using artificial neural networks (ANNs). The study aims to test the accuracy of the trained interpolator through self-inversion and, subsequently, to utilize the interpolator to derive the physical parameters of stars in the globular cluster NGC 6397 using spectra obtained from the Multi Unit Spectroscopic Explorer (MUSE) on the Very Large Telescope (VLT). In this study, ANNs were trained to function as spectral interpolators. The ULySS full-spectrum fitting package, integrated with the trained interpolators, was then used to extract the physical parameters of 1587 spectra of 1063 stars in NGC 6397. The trained ANN interpolator achieved precise determination of stellar parameters with a mean difference of 31 K for $T_{\rm eff}$ and 0.01 dex for [Fe/H] compared to previous studies. This study demonstrates the efficacy of ANN-based spectral interpolation in stellar parameter determination, offering faster and more accurate analysis.

==> table/Table_2.tex <==
\begin{tabular}{rrrcccr}
\hline\hline
      ID &   RA (deg) &  Dec (deg) &  T$_{\rm eff}$ (K) &     log g (dex) &     [Fe/H] (dex) &  QF \\
\hline
     5314 &  265.181095 & -53.676578 &   5143 $\pm$ 7 &  2.08  &  -2.10 $\pm$ 0.01 &   0 \\
     7321 &  265.148376 & -53.674232 &  6432 $\pm$ 17 &  4.13  &  -2.34 $\pm$ 0.08 &   0 \\
     4685 &  265.191895 & -53.674614 &  6445 $\pm$ 28 &  4.11  &  -2.13 $\pm$ 0.11 &   0 \\
     4944 &  265.186951 & -53.677929 &  6386 $\pm$ 14 &  4.07  &  -2.33 $\pm$ 0.06 &   0 \\
     4440 &  265.197364 & -53.675969 &  5741 $\pm$ 38 &  3.42  &  -2.22 $\pm$ 0.09 &   0 \\
     \vdots & \vdots  & \vdots  &  \vdots   & \vdots  & \vdots  &   \vdots \\
 %     8634 &  265.211548 & -53.667427 &  6135 $\pm$ 14 &  3.94  &  -2.65 $\pm$ 0.06 &   0 \\
 %     2454 &  265.158966 & -53.696049 &  6055 $\pm$ 14 &  3.75  &  -2.16 $\pm$ 0.04 &   1 \\
 %      975 &  265.198913 & -53.692122 &  5517 $\pm$ 11 &   3.2  &  -2.08 $\pm$ 0.02 &   0 \\
 %     9291 &  265.195129 & -53.671154 &  6125 $\pm$ 16 &  3.84  &  -2.45 $\pm$ 0.06 &   0 \\
 %    14955 &  265.152516 & -53.658706 &  6334 $\pm$ 17 &  4.19  &  -2.22 $\pm$ 0.06 &   0 \\
 %     7034 &  265.155606 & -53.676289 &  5735 $\pm$ 14 &  3.74  &  -2.17 $\pm$ 0.03 &   0 \\
 % 14000063 &  265.214319 & -53.701635 &  6301 $\pm$ 15 &  4.13  &  -2.68 $\pm$ 0.07 &   0 \\
 % 22000009 &  265.242749 & -53.673715 &  6091 $\pm$ 16 &  3.87  &  -2.57 $\pm$ 0.06 &   0 \\
 %     8093 &  265.125490 & -53.673969 &  5837 $\pm$ 11 &  3.64  &  -2.24 $\pm$ 0.03 &   0 \\
 %     7310 &  265.148404 & -53.681148 &  5590 $\pm$ 11 &  3.32  &  -2.09 $\pm$ 0.02 &   0 \\
 %    11922 &  265.149750 & -53.660301 &  6337 $\pm$ 21 &  4.03  &  -2.37 $\pm$ 0.09 &   0 \\
 %     4659 &  265.191620 & -53.683134 &  6425 $\pm$ 18 &  4.13  &   -2.63 $\pm$ 0.1 &   0 \\
 %     2106 &  265.168243 & -53.688007 &  6293 $\pm$ 14 &  4.04  &  -2.58 $\pm$ 0.07 &   1 \\
 %     5744 &  265.175873 & -53.678322 &  6321 $\pm$ 11 &  3.98  &  -2.53 $\pm$ 0.05 &   0 \\
 %     7141 &  265.152618 & -53.682697 &  6378 $\pm$ 16 &  4.14  &  -2.68 $\pm$ 0.08 &   0 \\
 %     2277 &  265.163971 & -53.693985 &  6321 $\pm$ 13 &  4.05  &  -2.67 $\pm$ 0.06 &   0 \\
 %    14802 &  265.158054 & -53.648262 &  5626 $\pm$ 11 &  3.41  &  -2.01 $\pm$ 0.02 &   0 \\
 % 14000526 &  265.198103 & -53.702253 &  6408 $\pm$ 16 &  4.18  &  -2.25 $\pm$ 0.06 &   1 \\
 %    10062 &  265.181152 & -53.664360 &  6400 $\pm$ 22 &  4.06  &  -2.23 $\pm$ 0.09 &   0 \\
 %     4918 &  265.188013 & -53.680890 &  6288 $\pm$ 14 &  4.03  &  -2.36 $\pm$ 0.06 &   0 \\
 %     4079 &  265.206512 & -53.673862 &  6371 $\pm$ 18 &  4.09  &  -2.64 $\pm$ 0.09 &   0 \\
 %    10737 &  265.171649 & -53.660422 &  5535 $\pm$ 11 &  3.32  &  -2.08 $\pm$ 0.02 &   0 \\
 %     7597 &  265.141632 & -53.676437 &  5933 $\pm$ 12 &  3.69  &   -2.5 $\pm$ 0.04 &   1 \\
 %     8671 &  265.210716 & -53.662482 &  6285 $\pm$ 18 &  4.17  &   -2.7 $\pm$ 0.09 &   0 \\
 % 23000082 &  265.216402 & -53.658703 &  6338 $\pm$ 11 &   4  &  -2.29 $\pm$ 0.04 &   0 \\
 %     9100 &  265.200104 & -53.666302 &  6442 $\pm$ 19 &  4.18  &  -2.41 $\pm$ 0.09 &   0 \\
 %     8553 &  265.214325 & -53.668133 &  6082 $\pm$ 18 &  3.86  &   -2.6 $\pm$ 0.07 &   0 \\
 %    12160 &  265.142822 & -53.664536 &  6155 $\pm$ 12 &  3.84  &   -2.3 $\pm$ 0.04 &   0 \\
 %    14926 &  265.153870 & -53.654381 &  6264 $\pm$ 21 &  3.99  &  -2.28 $\pm$ 0.08 &   0 \\
 %     9865 &  265.184082 & -53.667587 &  6286 $\pm$ 15 &  3.96  &  -2.51 $\pm$ 0.07 &   0 \\
 %    15659 &  265.192068 & -53.639713 &  6341 $\pm$ 12 &  4.04  &  -2.34 $\pm$ 0.05 &   0 \\
 %     3437 &  265.226247 & -53.676967 &  6210 $\pm$ 11 &  3.87  &  -2.45 $\pm$ 0.05 &   0 \\
 %     1222 &  265.191467 & -53.688541 &  5643 $\pm$ 12 &  3.42  &  -2.21 $\pm$ 0.03 &   0 \\
 %     6379 &  265.168091 & -53.674004 &  5527 $\pm$ 11 &  3.24  &   -2.2 $\pm$ 0.02 &   0 \\
 %    11549 &  265.157077 & -53.664095 &  6330 $\pm$ 15 &  3.98  &  -2.37 $\pm$ 0.06 &   0 \\
 %     5744 &  265.175871 & -53.678323 &  6311 $\pm$ 16 &  3.98  &  -2.41 $\pm$ 0.07 &   0 \\
 %     3766 &  265.215302 & -53.687019 &  6258 $\pm$ 19 &  4.12  &  -2.19 $\pm$ 0.07 &   0 \\
 %    14003 &  265.180359 & -53.647686 &  5321 $\pm$ 10 &  2.57  &   -2.3 $\pm$ 0.02 &   0 \\
 % 21000127 &  265.258348 & -53.679970 &  6302 $\pm$ 10 &  4.03  &  -2.41 $\pm$ 0.04 &   0 \\
 %    10160 &  265.179230 & -53.669949 &  5561 $\pm$ 15 &  3.39  &   -2.1 $\pm$ 0.03 &   0 \\
 % 16000063 &  265.158134 & -53.638223 &  6374 $\pm$ 14 &  4.19  &  -2.45 $\pm$ 0.06 &   0 \\
 % 18000165 &  265.117018 & -53.649533 &  6104 $\pm$ 10 &  3.82  &  -2.24 $\pm$ 0.03 &   0 \\
 %    11384 &  265.160694 & -53.669060 &  6317 $\pm$ 17 &  4.07  &  -2.48 $\pm$ 0.08 &   0 \\
 % 12000096 &  265.161949 & -53.715250 &  5581 $\pm$ 10 &  3.19  &  -2.07 $\pm$ 0.02 &   0 \\
 %     5948 &  265.173706 & -53.675892 &  7005 $\pm$ 11 &  4.01  &  -2.59 $\pm$ 0.08 &   0 \\
 %    14672 &  265.161713 & -53.655113 &  6378 $\pm$ 27 &  4.17  &  -2.73 $\pm$ 0.14 &   0 \\
 % 16000061 &  265.174288 & -53.638860 &   5159 $\pm$ 8 &   2.1  &  -2.12 $\pm$ 0.01 &   0 \\
 % 15000061 &  265.217097 & -53.644767 &  5375 $\pm$ 10 &  2.72  &  -2.12 $\pm$ 0.02 &   0 \\
 %     7115 &  265.153414 & -53.683228 &  6280 $\pm$ 12 &  3.96  &   -2.4 $\pm$ 0.05 &   0 \\
 %     3847 &  265.212860 & -53.683834 &  6443 $\pm$ 20 &  4.05  &  -2.26 $\pm$ 0.09 &   0 \\
 %    11230 &  265.163971 & -53.667603 &  5438 $\pm$ 14 &  2.75  &  -2.19 $\pm$ 0.03 &   0 \\
 %    14480 &  265.167084 & -53.658150 &  5962 $\pm$ 28 &  3.68  &  -2.09 $\pm$ 0.08 &   0 \\
 %     2158 &  265.166382 & -53.698704 &  6017 $\pm$ 13 &  3.74  &  -2.45 $\pm$ 0.05 &   0 \\
 %     1030 &  265.196838 & -53.688828 &  5820 $\pm$ 13 &  3.64  &  -2.24 $\pm$ 0.03 &   0 \\
 %     7152 &  265.152687 & -53.678143 &   5595 $\pm$ 6 &  2.37  &  -2.32 $\pm$ 0.01 &   0 \\
 % 15000371 &  265.198754 & -53.639292 &  6206 $\pm$ 15 &  3.93  &  -2.48 $\pm$ 0.06 &   0 \\
 % 14000187 &  265.201611 & -53.699471 &  6351 $\pm$ 14 &  4.15  &   -2.3 $\pm$ 0.06 &   0 \\
 %    11616 &  265.155212 & -53.672745 &  6067 $\pm$ 12 &  3.81  &  -2.46 $\pm$ 0.05 &   0 \\
 %     9211 &  265.197236 & -53.670855 &  6492 $\pm$ 27 &  4.01  &  -2.12 $\pm$ 0.11 &   0 \\
 % 19000400 &  265.104495 & -53.668232 &  6428 $\pm$ 17 &  4.18  &  -2.24 $\pm$ 0.07 &   0 \\
 %    11140 &  265.165192 & -53.665771 &  6321 $\pm$ 20 &  3.91  &  -2.34 $\pm$ 0.08 &   0 \\
 %     5696 &  265.176880 & -53.674388 &  6425 $\pm$ 37 &  4.02  &   -2.2 $\pm$ 0.12 &   0 \\
 % 13000041 &  265.172534 & -53.712821 &  6316 $\pm$ 14 &  3.94  &   -2.6 $\pm$ 0.07 &   0 \\
 % 17000338 &  265.142646 & -53.642252 &  6417 $\pm$ 15 &  4.19  &   -2.1 $\pm$ 0.05 &   0 \\
 %     6904 &  265.158142 & -53.678204 &  6048 $\pm$ 13 &  3.79  &  -2.27 $\pm$ 0.04 &   0 \\
 %     6758 &  265.161041 & -53.682842 &  6084 $\pm$ 13 &  4.02  &  -2.13 $\pm$ 0.04 &   0 \\
 %     6910 &  265.158722 & -53.676258 &  6325 $\pm$ 15 &  4.02  &  -2.49 $\pm$ 0.07 &   0 \\
 %      160 &  265.168977 & -53.704179 &  6421 $\pm$ 16 &  4.11  &  -2.46 $\pm$ 0.07 &   0 \\
 %     6460 &  265.165877 & -53.687070 &  6319 $\pm$ 15 &  3.97  &  -2.49 $\pm$ 0.07 &   0 \\
 %    14080 &  265.178558 & -53.646053 &  5705 $\pm$ 22 &  3.57  &  -2.41 $\pm$ 0.06 &   0 \\
 %    11682 &  265.154358 & -53.671890 &  5467 $\pm$ 11 &  2.99  &   -2.3 $\pm$ 0.02 &   0 \\
 %    15700 &  265.189310 & -53.640135 &  6244 $\pm$ 16 &  4.06  &  -2.35 $\pm$ 0.07 &   0 \\
 %     2579 &  265.155914 & -53.691158 &  5969 $\pm$ 15 &  3.73  &  -2.28 $\pm$ 0.04 &   0 \\
 %     8071 &  265.126276 & -53.682098 &  6350 $\pm$ 17 &  4.14  &  -2.03 $\pm$ 0.05 &   1 \\
 %     8352 &  265.220002 & -53.669847 &  6151 $\pm$ 11 &  3.83  &   -2.2 $\pm$ 0.04 &   0 \\
 %     5201 &  265.182458 & -53.681623 &  5990 $\pm$ 14 &  3.75  &  -2.12 $\pm$ 0.04 &   1 \\
 %     6994 &  265.156158 & -53.683285 &  6365 $\pm$ 15 &  4.16  &  -2.41 $\pm$ 0.07 &   0 \\
 %    13954 &  265.181274 & -53.658611 &   5058 $\pm$ 3 &  1.46  &  -2.04 $\pm$ 0.01 &   0 \\
 % 21000073 &  265.260214 & -53.687100 &  6097 $\pm$ 11 &  3.78  &  -2.18 $\pm$ 0.03 &   0 \\
 %    11217 &  265.163940 & -53.672791 &  6180 $\pm$ 14 &  3.86  &  -2.58 $\pm$ 0.06 &   0 \\
 %     9188 &  265.197662 & -53.666775 &  6452 $\pm$ 16 &  4.18  &  -2.45 $\pm$ 0.08 &   0 \\
 %    11578 &  265.156387 & -53.664537 &  6179 $\pm$ 13 &  3.89  &  -2.23 $\pm$ 0.04 &   0 \\
 % 23000151 &  265.233686 & -53.657115 &  6366 $\pm$ 11 &  4.07  &  -2.33 $\pm$ 0.05 &   1 \\
 %    12032 &  265.146271 & -53.665901 &   5148 $\pm$ 7 &  1.74  &  -2.32 $\pm$ 0.02 &   0 \\
 %     6697 &  265.161987 & -53.679424 &  5382 $\pm$ 11 &  2.75  &  -2.23 $\pm$ 0.02 &   0 \\
 %     5842 &  265.174936 & -53.678606 &  6222 $\pm$ 19 &  3.86  &  -2.32 $\pm$ 0.07 &   0 \\
 %     5796 &  265.175496 & -53.678024 &  6487 $\pm$ 38 &  4.15  &  -2.74 $\pm$ 0.23 &   0 \\
 %    14213 &  265.174469 & -53.659340 &  6169 $\pm$ 18 &  3.88  &  -2.47 $\pm$ 0.07 &   0 \\
 %     5595 &  265.177551 & -53.674202 &  6319 $\pm$ 16 &  3.93  &  -2.46 $\pm$ 0.07 &   0 \\
 %    14081 &  265.178314 & -53.646076 &  6402 $\pm$ 28 &  3.94  &  -2.82 $\pm$ 0.15 &   0 \\
 %     7947 &  265.131714 & -53.676231 &  5586 $\pm$ 11 &  3.21  &  -2.12 $\pm$ 0.02 &   0 \\
 % 17000156 &  265.135367 & -53.649581 &  6397 $\pm$ 13 &  3.96  &  -2.38 $\pm$ 0.06 &   0 \\
 %    11433 &  265.159637 & -53.670353 &  6417 $\pm$ 15 &  4.15  &   -2.9 $\pm$ 0.08 &   0 \\
 %     9272 &  265.195923 & -53.668190 &  5601 $\pm$ 12 &  3.32  &  -2.19 $\pm$ 0.02 &   0 \\
 %     7202 &  265.151527 & -53.681282 &  6364 $\pm$ 14 &  4.03  &  -2.21 $\pm$ 0.05 &   0 \\
 %    10171 &  265.179718 & -53.668186 &  6199 $\pm$ 13 &  3.78  &  -2.39 $\pm$ 0.06 &   0 \\
 %     5651 &  265.176819 & -53.682590 &  5596 $\pm$ 17 &  3.04  &  -2.14 $\pm$ 0.03 &   0 \\
 %     1669 &  265.179382 & -53.687901 &  5935 $\pm$ 13 &  3.68  &  -2.35 $\pm$ 0.04 &   0 \\
 %     5747 &  265.175754 & -53.677838 &  5852 $\pm$ 20 &  3.65  &  -2.28 $\pm$ 0.05 &   0 \\
 %     2298 &  265.163940 & -53.687859 &  6366 $\pm$ 17 &  4.18  &  -2.62 $\pm$ 0.08 &   1 \\
 %    11745 &  265.153198 & -53.673069 &  6130 $\pm$ 13 &  3.94  &  -2.33 $\pm$ 0.05 &   0 \\
 %     5497 &  265.179077 & -53.673862 &  5700 $\pm$ 14 &  3.52  &  -2.17 $\pm$ 0.03 &   0 \\
 %     5616 &  265.177094 & -53.680241 &  6375 $\pm$ 13 &  4.14  &   -2.9 $\pm$ 0.07 &   0 \\
 %      700 &  265.212006 & -53.688423 &  6290 $\pm$ 16 &  4.02  &  -2.57 $\pm$ 0.08 &   0 \\
 %     5566 &  265.177478 & -53.679704 &  5711 $\pm$ 18 &  3.54  &  -2.09 $\pm$ 0.04 &   0 \\
 %    10315 &  265.176910 & -53.673122 &  6361 $\pm$ 16 &  4.11  &  -2.11 $\pm$ 0.06 &   0 \\
 %    11627 &  265.155334 & -53.667297 &  6386 $\pm$ 24 &  4.11  &  -2.79 $\pm$ 0.12 &   0 \\
 % 11000001 &  265.132970 & -53.698240 &   5161 $\pm$ 8 &  2.16  &  -2.06 $\pm$ 0.01 &   0 \\
 %     6014 &  265.172455 & -53.681885 &  6347 $\pm$ 13 &   4.1  &  -2.46 $\pm$ 0.06 &   0 \\
 %     4223 &  265.202454 & -53.683018 &  5979 $\pm$ 14 &  3.74  &  -2.38 $\pm$ 0.05 &   0 \\
 %    15761 &  265.186461 & -53.639336 &  5829 $\pm$ 21 &  3.59  &  -2.05 $\pm$ 0.05 &   0 \\
 %    11269 &  265.162231 & -53.673702 &  6364 $\pm$ 19 &   4.1  &  -2.34 $\pm$ 0.08 &   0 \\
 %     9253 &  265.196404 & -53.662557 &   5435 $\pm$ 9 &  2.95  &  -2.07 $\pm$ 0.02 &   0 \\
 % 24000164 &  265.204711 & -53.627163 &  6383 $\pm$ 13 &  4.16  &  -2.37 $\pm$ 0.06 &   0 \\
 % 15000108 &  265.199795 & -53.637100 &  6033 $\pm$ 12 &  3.82  &  -2.23 $\pm$ 0.04 &   0 \\
 %    14842 &  265.156691 & -53.649829 &  6356 $\pm$ 12 &  4.07  &   -2.3 $\pm$ 0.05 &   0 \\
 %     9306 &  265.195435 & -53.663574 &  6075 $\pm$ 14 &  3.81  &  -2.27 $\pm$ 0.04 &   0 \\
 %    10477 &  265.175293 & -53.669857 &  6451 $\pm$ 12 &  4.12  &  -2.41 $\pm$ 0.06 &   0 \\
 % 20000038 &  265.110042 & -53.685541 &  6350 $\pm$ 12 &  4.03  &  -2.25 $\pm$ 0.05 &   0 \\
 %    11106 &  265.165791 & -53.667367 &  6431 $\pm$ 17 &  4.17  &  -2.63 $\pm$ 0.08 &   0 \\
 % 11000100 &  265.121436 & -53.688243 &  6397 $\pm$ 13 &  4.17  &  -2.39 $\pm$ 0.06 &   0 \\
 %     2746 &  265.150848 & -53.696404 &   5053 $\pm$ 3 &  1.49  &  -2.04 $\pm$ 0.01 &   0 \\
 %     8764 &  265.208496 & -53.669357 &  6470 $\pm$ 14 &  4.05  &  -2.47 $\pm$ 0.08 &   0 \\
 % 14000112 &  265.207970 & -53.700663 &  5599 $\pm$ 11 &   3.4  &  -2.08 $\pm$ 0.02 &   1 \\
 % 18000178 &  265.125040 & -53.646122 &  5664 $\pm$ 10 &  3.46  &  -2.13 $\pm$ 0.02 &   0 \\
 %     1594 &  265.181021 & -53.695374 &  6301 $\pm$ 26 &  4.16  &  -2.49 $\pm$ 0.11 &   0 \\
 %     7682 &  265.138763 & -53.685332 &  6430 $\pm$ 16 &  4.06  &  -2.67 $\pm$ 0.09 &   0 \\
 %    13200 &  265.205292 & -53.659264 &  6308 $\pm$ 14 &  3.96  &  -2.68 $\pm$ 0.07 &   0 \\
 % 22000149 &  265.238082 & -53.677047 &  5959 $\pm$ 10 &  3.72  &   -2.1 $\pm$ 0.03 &   1 \\
 % 16000259 &  265.173338 & -53.638382 &  6320 $\pm$ 13 &  4.09  &  -2.19 $\pm$ 0.05 &   0 \\
 %     4778 &  265.190211 & -53.681445 &  6204 $\pm$ 15 &   3.9  &  -2.28 $\pm$ 0.06 &   0 \\
 %    15822 &  265.183617 & -53.640520 &  6199 $\pm$ 35 &  3.98  &  -2.82 $\pm$ 0.15 &   0 \\
 %     9865 &  265.184067 & -53.667586 &  6337 $\pm$ 16 &  3.96  &  -2.53 $\pm$ 0.07 &   0 \\
 %    10447 &  265.175934 & -53.664280 &  6069 $\pm$ 23 &  3.95  &  -2.37 $\pm$ 0.08 &   1 \\
 %    13089 &  265.106550 & -53.665668 &  5447 $\pm$ 10 &  2.91  &  -2.12 $\pm$ 0.02 &   0 \\
 %     8296 &  265.223012 & -53.665779 &  6301 $\pm$ 11 &  3.99  &  -2.36 $\pm$ 0.05 &   0 \\
 %     6245 &  265.169281 & -53.679497 &  6401 $\pm$ 15 &  4.15  &  -2.47 $\pm$ 0.07 &   0 \\
 %     5714 &  265.175766 & -53.684454 &  6254 $\pm$ 14 &  4.06  &  -2.14 $\pm$ 0.05 &   0 \\
 %    10502 &  265.175539 & -53.662743 &  6202 $\pm$ 14 &  3.88  &  -2.23 $\pm$ 0.05 &   0 \\
 % 12000243 &  265.171355 & -53.716409 &  6319 $\pm$ 14 &   4  &  -2.31 $\pm$ 0.06 &   0 \\
 %     6343 &  265.167603 & -53.683117 &  5510 $\pm$ 11 &  3.14  &  -2.21 $\pm$ 0.02 &   0 \\
 %    10163 &  265.179413 & -53.669903 &  6070 $\pm$ 16 &   3.8  &  -2.56 $\pm$ 0.06 &   0 \\
 %     9142 &  265.198767 & -53.672020 &  6874 $\pm$ 12 &  3.97  &  -2.14 $\pm$ 0.05 &   0 \\
 % 21000086 &  265.238901 & -53.685817 &  6248 $\pm$ 11 &  3.95  &  -2.11 $\pm$ 0.04 &   0 \\
 % 23000088 &  265.229450 & -53.657953 &   5329 $\pm$ 9 &   2.6  &  -2.12 $\pm$ 0.01 &   0 \\
 % 19000160 &  265.089869 & -53.666857 &  6377 $\pm$ 13 &  4.15  &  -2.03 $\pm$ 0.05 &   0 \\
 %    14401 &  265.169803 & -53.647456 &  5331 $\pm$ 10 &  2.67  &   -2.1 $\pm$ 0.02 &   0 \\
 %     4886 &  265.188038 & -53.678982 &  6228 $\pm$ 22 &  4.14  &   -2.79 $\pm$ 0.1 &   0 \\
 %     4547 &  265.194885 & -53.674660 &  6084 $\pm$ 15 &  3.77  &   -2.3 $\pm$ 0.05 &   0 \\
 %     8998 &  265.201782 & -53.671101 &  6215 $\pm$ 13 &  4.01  &  -2.19 $\pm$ 0.05 &   0 \\
 %     6441 &  265.166626 & -53.679317 &  6396 $\pm$ 13 &  4.08  &  -2.81 $\pm$ 0.07 &   0 \\
 %     9358 &  265.194153 & -53.668320 &  5745 $\pm$ 13 &  3.58  &  -2.12 $\pm$ 0.03 &   0 \\
 %     9208 &  265.196930 & -53.671490 &  5498 $\pm$ 12 &  3.08  &   -2.2 $\pm$ 0.02 &   0 \\
 %     2019 &  265.170135 & -53.697006 &  6454 $\pm$ 16 &  4.07  &  -2.56 $\pm$ 0.08 &   0 \\
 %     7608 &  265.141022 & -53.683697 &  5342 $\pm$ 11 &   2.6  &  -2.25 $\pm$ 0.02 &   0 \\
 %     2327 &  265.162567 & -53.693222 &  6400 $\pm$ 17 &  4.15  &  -2.37 $\pm$ 0.07 &   0 \\
 %     5842 &  265.174927 & -53.678604 &  6197 $\pm$ 14 &  3.86  &  -2.36 $\pm$ 0.06 &   0 \\
 % 12000057 &  265.150869 & -53.721424 &  6385 $\pm$ 11 &  3.99  &  -2.56 $\pm$ 0.06 &   0 \\
 %     1824 &  265.175910 & -53.689729 &   5036 $\pm$ 3 &  1.35  &  -1.91 $\pm$ 0.01 &   0 \\
 %    11274 &  265.162811 & -53.669834 &  5908 $\pm$ 12 &  3.36  &  -2.11 $\pm$ 0.03 &   0 \\
 %    15466 &  265.129941 & -53.653272 &  6347 $\pm$ 12 &  4.13  &  -2.39 $\pm$ 0.05 &   0 \\
 % 23000371 &  265.219341 & -53.656727 &   5243 $\pm$ 7 &  1.94  &  -2.39 $\pm$ 0.01 &   0 \\
 %    12068 &  265.145111 & -53.666935 &  6393 $\pm$ 17 &  4.19  &  -2.36 $\pm$ 0.07 &   0 \\
 %    13630 &  265.191162 & -53.646152 &  6383 $\pm$ 16 &  4.13  &  -2.34 $\pm$ 0.07 &   0 \\
 % 13000031 &  265.188996 & -53.714796 &   5505 $\pm$ 9 &  3.07  &  -2.13 $\pm$ 0.02 &   1 \\
 %    10772 &  265.171182 & -53.664794 &  6479 $\pm$ 19 &   4.1  &   -2.62 $\pm$ 0.1 &   0 \\
 %     5882 &  265.174255 & -53.681492 &  5809 $\pm$ 13 &  3.64  &  -2.28 $\pm$ 0.03 &   0 \\
 % 11000486 &  265.121604 & -53.694151 &  6368 $\pm$ 11 &  4.03  &  -2.25 $\pm$ 0.04 &   0 \\
 %    15700 &  265.189310 & -53.640135 &  5939 $\pm$ 50 &  4.06  &  -2.52 $\pm$ 0.16 &   0 \\
 % 24000092 &  265.204019 & -53.629795 &  6323 $\pm$ 11 &  4.03  &  -2.21 $\pm$ 0.04 &   0 \\
 %     9897 &  265.183380 & -53.667782 &  6446 $\pm$ 26 &  4.11  &  -2.29 $\pm$ 0.13 &   0 \\
 %     3987 &  265.208801 & -53.681602 &  6337 $\pm$ 14 &  4.01  &   -2.6 $\pm$ 0.07 &   0 \\
 % 21000130 &  265.247082 & -53.679266 &  5409 $\pm$ 10 &  2.78  &  -2.08 $\pm$ 0.02 &   0 \\
 %     3640 &  265.218933 & -53.684696 &   5177 $\pm$ 7 &  1.83  &  -2.33 $\pm$ 0.01 &   0 \\
 % 14000111 &  265.220083 & -53.701337 &  5533 $\pm$ 19 &  3.06  &  -1.95 $\pm$ 0.03 &   0 \\
 %    13683 &  265.189301 & -53.648991 &  6376 $\pm$ 18 &   4.1  &  -2.82 $\pm$ 0.09 &   0 \\
 %     8473 &  265.216592 & -53.665239 &  5531 $\pm$ 12 &  3.54  &  -1.16 $\pm$ 0.02 &   1 \\
 %     6565 &  265.164276 & -53.686089 &   5093 $\pm$ 5 &  1.66  &  -2.15 $\pm$ 0.01 &   0 \\
 %     1352 &  265.187500 & -53.690186 &  6400 $\pm$ 16 &  4.11  &  -2.32 $\pm$ 0.07 &   0 \\
 % 18000215 &  265.122944 & -53.647266 &  6396 $\pm$ 12 &  4.15  &  -2.21 $\pm$ 0.05 &   0 \\
 % 17000155 &  265.138170 & -53.649604 &  6424 $\pm$ 12 &  4.14  &  -2.35 $\pm$ 0.05 &   0 \\
 %     5032 &  265.185322 & -53.679728 &  6143 $\pm$ 21 &  3.84  &  -2.52 $\pm$ 0.09 &   0 \\
 % 19000126 &  265.101626 & -53.659498 &  5730 $\pm$ 11 &  3.53  &  -2.05 $\pm$ 0.02 &   0 \\
 %       83 &  265.174878 & -53.705443 &  6313 $\pm$ 12 &  3.96  &  -2.45 $\pm$ 0.05 &   0 \\
 %     4871 &  265.188475 & -53.685418 &   5198 $\pm$ 7 &  2.25  &  -2.23 $\pm$ 0.01 &   0 \\
 %     4795 &  265.189728 & -53.686371 &  6058 $\pm$ 13 &  3.78  &  -2.44 $\pm$ 0.05 &   0 \\
 % 13000132 &  265.174731 & -53.711099 &  6382 $\pm$ 14 &  4.18  &  -2.23 $\pm$ 0.05 &   0 \\
 %     5497 &  265.179071 & -53.673864 &  5725 $\pm$ 18 &  3.52  &  -2.09 $\pm$ 0.04 &   0 \\
 % 15000064 &  265.224300 & -53.644599 &  6270 $\pm$ 12 &  4.01  &  -2.24 $\pm$ 0.05 &   0 \\
 %    11233 &  265.163866 & -53.664393 &  6281 $\pm$ 15 &  4.11  &  -2.02 $\pm$ 0.05 &   1 \\
 %     5437 &  265.179463 & -53.677335 &  5748 $\pm$ 20 &  3.46  &  -2.17 $\pm$ 0.04 &   0 \\
 %    10165 &  265.179810 & -53.669205 &  5514 $\pm$ 10 &  2.99  &  -2.18 $\pm$ 0.02 &   0 \\
 %     5603 &  265.177032 & -53.685940 &  6392 $\pm$ 14 &  4.07  &  -2.86 $\pm$ 0.07 &   0 \\
 %     4795 &  265.189715 & -53.686372 &  6034 $\pm$ 12 &  3.78  &  -2.39 $\pm$ 0.04 &   0 \\
 %     1030 &  265.196849 & -53.688827 &  5824 $\pm$ 13 &  3.64  &  -2.14 $\pm$ 0.03 &   0 \\
 %    15047 &  265.150495 & -53.650175 &  6366 $\pm$ 11 &  4.08  &  -2.32 $\pm$ 0.05 &   0 \\
 %    11435 &  265.159851 & -53.670071 &  6177 $\pm$ 12 &  3.85  &  -2.43 $\pm$ 0.05 &   0 \\
 %     5032 &  265.185322 & -53.679728 &  6165 $\pm$ 20 &  3.84  &  -1.95 $\pm$ 0.05 &   0 \\
 % 21000133 &  265.256817 & -53.678771 &  6400 $\pm$ 11 &  4.04  &  -2.38 $\pm$ 0.05 &   0 \\
 % 18000038 &  265.123771 & -53.653577 &  6026 $\pm$ 11 &  3.79  &  -2.16 $\pm$ 0.03 &   0 \\
 %     9830 &  265.184662 & -53.669460 &  6256 $\pm$ 18 &  3.99  &  -2.58 $\pm$ 0.08 &   0 \\
 % 22000112 &  265.235195 & -53.661234 &  6268 $\pm$ 14 &  4.02  &  -2.38 $\pm$ 0.06 &   0 \\
 %    14151 &  265.176270 & -53.656490 &  6352 $\pm$ 14 &  4.02  &  -2.94 $\pm$ 0.07 &   0 \\
 %     5373 &  265.180121 & -53.683444 &  6470 $\pm$ 20 &  4.16  &   -2.41 $\pm$ 0.1 &   0 \\
 %    10281 &  265.177582 & -53.670681 &  6357 $\pm$ 20 &  4.09  &   -2.47 $\pm$ 0.1 &   0 \\
 %    14762 &  265.159003 & -53.656523 &  6426 $\pm$ 20 &  4.19  &  -2.08 $\pm$ 0.07 &   0 \\
 %     1439 &  265.185228 & -53.694636 &  6273 $\pm$ 15 &  3.97  &  -2.26 $\pm$ 0.06 &   0 \\
 %     2745 &  265.151062 & -53.697441 &  5975 $\pm$ 13 &  3.74  &  -2.25 $\pm$ 0.04 &   0 \\
 % 13000051 &  265.194225 & -53.711535 &   5156 $\pm$ 7 &  2.04  &  -2.14 $\pm$ 0.01 &   0 \\
 %    15648 &  265.192616 & -53.641792 &  6431 $\pm$ 29 &  4.12  &  -2.15 $\pm$ 0.12 &   0 \\
 %     4746 &  265.190520 & -53.681263 &  6360 $\pm$ 41 &  4.16  &   -2.48 $\pm$ 0.2 &   0 \\
 %    15021 &  265.150909 & -53.658020 &  6367 $\pm$ 24 &  4.14  &   -2.9 $\pm$ 0.12 &   0 \\
 %     4950 &  265.187176 & -53.673816 &  6349 $\pm$ 15 &  4.02  &  -2.38 $\pm$ 0.07 &   0 \\
 %     2205 &  265.165283 & -53.698940 &  6138 $\pm$ 14 &  3.86  &  -2.59 $\pm$ 0.06 &   0 \\
 %     1237 &  265.190674 & -53.690884 &  6362 $\pm$ 15 &  4.09  &  -2.66 $\pm$ 0.08 &   0 \\
 %    11551 &  265.157421 & -53.663136 &  5809 $\pm$ 12 &  3.63  &  -2.15 $\pm$ 0.03 &   0 \\
 %     8484 &  265.216286 & -53.661780 &  6139 $\pm$ 10 &  3.85  &  -2.29 $\pm$ 0.03 &   0 \\
 %     4322 &  265.199921 & -53.676994 &  6328 $\pm$ 15 &  4.08  &  -2.56 $\pm$ 0.07 &   0 \\
 %     5110 &  265.184418 & -53.675556 &  5621 $\pm$ 12 &  3.39  &  -2.27 $\pm$ 0.03 &   1 \\
 %     5863 &  265.174909 & -53.674515 &  6193 $\pm$ 16 &  3.86  &  -2.42 $\pm$ 0.06 &   0 \\
 %    13520 &  265.193878 & -53.650230 &  6229 $\pm$ 14 &  3.95  &  -2.39 $\pm$ 0.05 &   0 \\
 % 15000145 &  265.210940 & -53.650552 &  6324 $\pm$ 20 &  4.06  &   -2.4 $\pm$ 0.09 &   0 \\
 %     8172 &  265.120754 & -53.677272 &  6336 $\pm$ 13 &  4.08  &  -2.18 $\pm$ 0.05 &   0 \\
 %     6284 &  265.169006 & -53.680447 &  5617 $\pm$ 12 &  3.32  &  -2.24 $\pm$ 0.03 &   0 \\
 %    11551 &  265.157410 & -53.663136 &  5837 $\pm$ 20 &  3.63  &  -2.27 $\pm$ 0.05 &   0 \\
 %    11035 &  265.166992 & -53.667866 &  6112 $\pm$ 12 &  3.85  &  -2.37 $\pm$ 0.04 &   1 \\
 %     7067 &  265.154157 & -53.684746 &  6244 $\pm$ 13 &  3.97  &  -2.22 $\pm$ 0.05 &   0 \\
 %    12630 &  265.125946 & -53.673428 &  6328 $\pm$ 14 &  4.02  &  -2.41 $\pm$ 0.06 &   0 \\
 %    10319 &  265.176971 & -53.672630 &  5907 $\pm$ 12 &  3.71  &  -2.27 $\pm$ 0.03 &   0 \\
 % 21000149 &  265.253663 & -53.675387 &  6040 $\pm$ 10 &  3.75  &   -2.3 $\pm$ 0.03 &   0 \\
 %     1222 &  265.191458 & -53.688542 &  5623 $\pm$ 12 &  3.42  &  -2.11 $\pm$ 0.02 &   0 \\
 %    13690 &  265.189148 & -53.657951 &  6440 $\pm$ 19 &  4.17  &  -2.06 $\pm$ 0.07 &   0 \\
 % 23000645 &  265.233766 & -53.655906 &  6338 $\pm$ 20 &  4.14  &  -1.97 $\pm$ 0.06 &   0 \\
 %     1330 &  265.188568 & -53.690540 &  6238 $\pm$ 15 &  3.91  &  -2.52 $\pm$ 0.06 &   0 \\
 % 12000129 &  265.173402 & -53.721243 &  6374 $\pm$ 13 &  4.11  &   -2.4 $\pm$ 0.06 &   0 \\
 % 22000196 &  265.227474 & -53.668389 &  5763 $\pm$ 11 &  3.55  &  -2.12 $\pm$ 0.03 &   0 \\
 %    15021 &  265.150901 & -53.658019 &  6316 $\pm$ 15 &  4.14  &  -2.47 $\pm$ 0.07 &   0 \\
 %    13802 &  265.185211 & -53.659492 &  6383 $\pm$ 14 &  4.11  &  -2.43 $\pm$ 0.07 &   0 \\
 %     9414 &  265.193106 & -53.667794 &   5232 $\pm$ 9 &  2.52  &  -2.15 $\pm$ 0.01 &   0 \\
 %     8998 &  265.201796 & -53.671101 &  6241 $\pm$ 15 &  4.01  &  -2.08 $\pm$ 0.05 &   0 \\
 %     1793 &  265.176361 & -53.689163 &  6215 $\pm$ 14 &  4.08  &  -2.11 $\pm$ 0.04 &   0 \\
 %    15456 &  265.130620 & -53.652834 &   5454 $\pm$ 9 &  2.98  &  -2.04 $\pm$ 0.02 &   0 \\
 %    14942 &  265.152942 & -53.658353 &  6282 $\pm$ 14 &  3.98  &  -2.42 $\pm$ 0.06 &   0 \\
 %     5092 &  265.184389 & -53.683074 &  5843 $\pm$ 15 &  3.66  &  -2.26 $\pm$ 0.04 &   0 \\
 %    14480 &  265.167094 & -53.658150 &  5814 $\pm$ 17 &  3.68  &  -2.45 $\pm$ 0.05 &   0 \\
 %    12348 &  265.136505 & -53.663784 &  5561 $\pm$ 12 &  3.18  &  -2.28 $\pm$ 0.03 &   0 \\
 % 22000072 &  265.243296 & -53.670685 &  5582 $\pm$ 11 &   3.3  &  -2.08 $\pm$ 0.02 &   0 \\
 %     4958 &  265.186371 & -53.683292 &  6419 $\pm$ 13 &  4.03  &   -3  &   0 \\
 %    11371 &  265.160583 & -53.673252 &  6015 $\pm$ 12 &  3.79  &  -2.37 $\pm$ 0.04 &   0 \\
 %     9739 &  265.186420 & -53.665000 &  5697 $\pm$ 13 &   3.5  &  -2.09 $\pm$ 0.03 &   0 \\
 %     5595 &  265.177563 & -53.674202 &  6257 $\pm$ 26 &  3.93  &  -2.96 $\pm$ 0.12 &   0 \\
 %    14788 &  265.157631 & -53.658451 &   5365 $\pm$ 8 &  2.62  &   -2.1 $\pm$ 0.01 &   0 \\
 %     1168 &  265.192355 & -53.696840 &  6208 $\pm$ 12 &  3.87  &  -2.31 $\pm$ 0.04 &   0 \\
 %     6942 &  265.157462 & -53.686033 &  6412 $\pm$ 17 &  4.19  &  -2.31 $\pm$ 0.08 &   0 \\
 %    10515 &  265.174652 & -53.673027 &  5508 $\pm$ 10 &  3.04  &  -2.19 $\pm$ 0.02 &   0 \\
 %     7117 &  265.153412 & -53.681853 &   5141 $\pm$ 7 &  2.09  &  -2.12 $\pm$ 0.01 &   0 \\
 %     6343 &  265.167600 & -53.683118 &  5471 $\pm$ 11 &  3.14  &  -2.13 $\pm$ 0.02 &   0 \\
 %    13899 &  265.183075 & -53.649582 &  6379 $\pm$ 17 &  4.16  &  -2.51 $\pm$ 0.07 &   0 \\
 %     5031 &  265.185638 & -53.679897 &  5410 $\pm$ 10 &  2.35  &  -2.27 $\pm$ 0.02 &   0 \\
 %     3274 &  265.233093 & -53.680732 &  6146 $\pm$ 17 &  3.87  &  -2.23 $\pm$ 0.06 &   0 \\
 %     7355 &  265.147156 & -53.680016 &  6174 $\pm$ 12 &  3.89  &  -2.62 $\pm$ 0.05 &   0 \\
 %     7079 &  265.154223 & -53.676991 &  6383 $\pm$ 15 &  4.11  &   -2 $\pm$ 0.05 &   0 \\
 %    10903 &  265.169495 & -53.666779 &  5399 $\pm$ 13 &  2.68  &  -2.19 $\pm$ 0.03 &   0 \\
 % 22000289 &  265.228673 & -53.667991 &   5257 $\pm$ 9 &  2.42  &  -2.16 $\pm$ 0.01 &   0 \\
 %     5212 &  265.182588 & -53.678569 &  5374 $\pm$ 12 &  2.89  &   -2.1 $\pm$ 0.02 &   0 \\
 %     5366 &  265.180695 & -53.674236 &  5955 $\pm$ 14 &  3.71  &  -2.37 $\pm$ 0.05 &   0 \\
 %     5310 &  265.181458 & -53.677017 &  6320 $\pm$ 14 &  4.07  &  -2.21 $\pm$ 0.05 &   0 \\
 %     4758 &  265.190491 & -53.674477 &  5748 $\pm$ 23 &   3.6  &  -2.19 $\pm$ 0.05 &   0 \\
 %     3418 &  265.226912 & -53.678058 &  6443 $\pm$ 18 &  4.11  &  -2.49 $\pm$ 0.09 &   1 \\
 %     8983 &  265.202240 & -53.664429 &  5803 $\pm$ 15 &  3.65  &  -2.31 $\pm$ 0.04 &   0 \\
 %     7321 &  265.148376 & -53.674232 &  6432 $\pm$ 15 &  4.13  &  -2.72 $\pm$ 0.09 &   0 \\
 % 19000058 &  265.101763 & -53.668888 &  6397 $\pm$ 13 &  4.18  &  -2.23 $\pm$ 0.05 &   0 \\
 %      638 &  265.216095 & -53.687801 &  5720 $\pm$ 23 &  3.54  &  -2.29 $\pm$ 0.06 &   0 \\
 %     7437 &  265.145051 & -53.687302 &   5417 $\pm$ 9 &   3  &  -2.16 $\pm$ 0.02 &   0 \\
 % 13000035 &  265.180055 & -53.713990 &   5486 $\pm$ 9 &   3  &  -2.06 $\pm$ 0.02 &   0 \\
 %     5498 &  265.178717 & -53.673793 &  6311 $\pm$ 21 &  3.92  &  -2.11 $\pm$ 0.07 &   0 \\
 %     5645 &  265.176595 & -53.685051 &   5412 $\pm$ 9 &  2.93  &  -2.17 $\pm$ 0.02 &   0 \\
 %     5698 &  265.176331 & -53.674404 &  6399 $\pm$ 32 &  4.12  &   -3  &   0 \\
 % 22000168 &  265.247345 & -53.672742 &  6384 $\pm$ 12 &  4.09  &  -2.31 $\pm$ 0.05 &   0 \\
 %    12534 &  265.129791 & -53.663338 &  5570 $\pm$ 11 &  3.13  &  -2.19 $\pm$ 0.02 &   0 \\
 %    13360 &  265.199603 & -53.646712 &  5649 $\pm$ 11 &  3.44  &  -2.17 $\pm$ 0.02 &   0 \\
 %     5692 &  265.176514 & -53.674820 &  6184 $\pm$ 28 &  4.17  &  -2.81 $\pm$ 0.12 &   0 \\
 %     2298 &  265.163949 & -53.687859 &  6373 $\pm$ 17 &  4.18  &  -2.25 $\pm$ 0.07 &   1 \\
 %     5498 &  265.178711 & -53.673794 &  6341 $\pm$ 12 &  3.92  &  -2.49 $\pm$ 0.06 &   0 \\
 % 22000292 &  265.249011 & -53.667576 &  5721 $\pm$ 12 &   3.5  &  -2.08 $\pm$ 0.03 &   0 \\
 % 22000120 &  265.248617 & -53.674687 &  6415 $\pm$ 12 &  4.07  &  -2.45 $\pm$ 0.06 &   0 \\
 %     6929 &  265.157928 & -53.678604 &  5693 $\pm$ 13 &   3.5  &  -2.23 $\pm$ 0.03 &   0 \\
 %    10012 &  265.182129 & -53.669735 &  5561 $\pm$ 12 &  3.27  &  -2.17 $\pm$ 0.02 &   0 \\
 %    15610 &  265.195143 & -53.645002 &  6386 $\pm$ 14 &   4.2  &  -2.37 $\pm$ 0.06 &   0 \\
 %     6139 &  265.170471 & -53.686638 &  5403 $\pm$ 13 &  2.72  &  -2.15 $\pm$ 0.02 &   0 \\
 %     6747 &  265.161438 & -53.675060 &  6416 $\pm$ 14 &  4.13  &  -2.57 $\pm$ 0.07 &   0 \\
 %     4885 &  265.188299 & -53.679142 &  6474 $\pm$ 28 &  4.05  &  -2.62 $\pm$ 0.14 &   0 \\
 % 19000028 &  265.095612 & -53.659653 &  5562 $\pm$ 10 &  3.15  &  -2.09 $\pm$ 0.02 &   1 \\
 %     6139 &  265.170456 & -53.686638 &  5471 $\pm$ 21 &  2.72  &   -2.1 $\pm$ 0.04 &   0 \\
 %     5031 &  265.185635 & -53.679897 &   5342 $\pm$ 8 &  2.35  &  -2.21 $\pm$ 0.01 &   0 \\
 %     4593 &  265.193507 & -53.679570 &  6293 $\pm$ 14 &  3.97  &  -2.23 $\pm$ 0.05 &   0 \\
 %    10903 &  265.169495 & -53.666779 &  5396 $\pm$ 11 &  2.68  &  -2.25 $\pm$ 0.02 &   0 \\
 %     8656 &  265.211165 & -53.662162 &   5489 $\pm$ 9 &  2.95  &  -2.13 $\pm$ 0.02 &   0 \\
 %     7403 &  265.146089 & -53.681866 &  6335 $\pm$ 17 &  4.13  &  -2.22 $\pm$ 0.06 &   0 \\
 %     5668 &  265.176357 & -53.678140 &  5808 $\pm$ 13 &  3.59  &  -2.22 $\pm$ 0.03 &   0 \\
 % 15000199 &  265.200961 & -53.642600 &  6471 $\pm$ 14 &  4.18  &   -2.8 $\pm$ 0.08 &   0 \\
 %     5313 &  265.181549 & -53.676689 &  5511 $\pm$ 14 &  3.06  &  -2.23 $\pm$ 0.03 &   0 \\
 %     9024 &  265.201019 & -53.669941 &  6289 $\pm$ 15 &  4.02  &   -2.4 $\pm$ 0.06 &   0 \\
 %     2169 &  265.166779 & -53.690517 &  5552 $\pm$ 14 &  3.19  &  -2.28 $\pm$ 0.03 &   0 \\
 %     5938 &  265.173370 & -53.677696 &  5604 $\pm$ 14 &  3.21  &  -2.17 $\pm$ 0.03 &   0 \\
 %    15155 &  265.146392 & -53.650689 &  5884 $\pm$ 10 &   3.7  &  -2.13 $\pm$ 0.03 &   0 \\
 %    10734 &  265.171677 & -53.663115 &  6230 $\pm$ 21 &  4.13  &  -2.03 $\pm$ 0.06 &   0 \\
 %     8532 &  265.214966 & -53.669373 &  6303 $\pm$ 16 &  4.05  &  -2.41 $\pm$ 0.07 &   0 \\
 %     5792 &  265.175591 & -53.680158 &  6420 $\pm$ 16 &  4.08  &  -2.14 $\pm$ 0.06 &   1 \\
 %     8583 &  265.212891 & -53.672577 &  5333 $\pm$ 10 &  2.53  &  -2.22 $\pm$ 0.02 &   0 \\
 %    13747 &  265.186981 & -53.654564 &  5635 $\pm$ 11 &  3.25  &  -2.23 $\pm$ 0.03 &   1 \\
 %    12049 &  265.145630 & -53.668301 &  5532 $\pm$ 10 &  3.19  &  -2.19 $\pm$ 0.02 &   0 \\
 % 15000145 &  265.210940 & -53.650552 &  6371 $\pm$ 17 &  4.06  &  -2.32 $\pm$ 0.07 &   0 \\
 %     3556 &  265.221527 & -53.682854 &  5658 $\pm$ 12 &  3.34  &  -2.17 $\pm$ 0.03 &   0 \\
 %    12228 &  265.140625 & -53.659931 &  6567 $\pm$ 14 &   4.1  &  -2.45 $\pm$ 0.08 &   0 \\
 %    13054 &  265.108545 & -53.665325 &  5350 $\pm$ 14 &  2.77  &  -2.12 $\pm$ 0.02 &   0 \\
 %     6691 &  265.162140 & -53.683441 &  5787 $\pm$ 14 &  3.66  &  -2.19 $\pm$ 0.03 &   0 \\
 %     7355 &  265.147149 & -53.680017 &  6241 $\pm$ 14 &  3.89  &  -2.47 $\pm$ 0.06 &   0 \\
 %     9612 &  265.189056 & -53.665134 &  6333 $\pm$ 13 &  3.95  &  -2.41 $\pm$ 0.06 &   0 \\
 %    14213 &  265.174484 & -53.659339 &  6190 $\pm$ 13 &  3.88  &  -2.31 $\pm$ 0.05 &   0 \\
 %     6565 &  265.164276 & -53.686089 &  5026 $\pm$ 15 &  1.66  &  -2.34 $\pm$ 0.05 &   8 \\
 % 18000177 &  265.122184 & -53.646388 &  6253 $\pm$ 10 &   3.9  &  -2.24 $\pm$ 0.04 &   0 \\
 % 17000106 &  265.137587 & -53.644385 &  6381 $\pm$ 12 &  4.13  &  -2.14 $\pm$ 0.04 &   0 \\
 %     4872 &  265.188568 & -53.684628 &   5099 $\pm$ 5 &  1.69  &  -2.18 $\pm$ 0.01 &   0 \\
 %     9270 &  265.196219 & -53.669542 &  6167 $\pm$ 14 &   3.9  &  -2.26 $\pm$ 0.05 &   0 \\
 %    11804 &  265.152008 & -53.673069 &  5668 $\pm$ 14 &  3.49  &   -2.2 $\pm$ 0.03 &   0 \\
 %     5159 &  265.183014 & -53.681065 &  6261 $\pm$ 31 &  3.97  &   -2.08 $\pm$ 0.1 &   0 \\
 %    13794 &  265.186035 & -53.652100 &  5461 $\pm$ 10 &  2.82  &  -2.17 $\pm$ 0.02 &   0 \\
 %    11645 &  265.154938 & -53.672989 &  5747 $\pm$ 14 &  3.59  &  -2.26 $\pm$ 0.03 &   0 \\
 %     9894 &  265.183380 & -53.669239 &  5354 $\pm$ 15 &  2.84  &  -2.45 $\pm$ 0.03 &   0 \\
 %    10127 &  265.180176 & -53.667995 &  5327 $\pm$ 16 &   2.5  &  -2.25 $\pm$ 0.03 &   0 \\
 %     1176 &  265.192291 & -53.690090 &   5163 $\pm$ 9 &  2.09  &  -2.21 $\pm$ 0.02 &   0 \\
 %     5651 &  265.176815 & -53.682589 &  5443 $\pm$ 10 &  3.04  &  -2.13 $\pm$ 0.02 &   1 \\
 % 12000108 &  265.150906 & -53.713160 &  5735 $\pm$ 10 &  3.45  &  -2.18 $\pm$ 0.02 &   0 \\
 %    14464 &  265.167542 & -53.652157 &  6352 $\pm$ 20 &  4.13  &    -2.4 $\pm$ 0.1 &   0 \\
 %     9910 &  265.183745 & -53.662734 &  5663 $\pm$ 15 &  3.61  &  -2.01 $\pm$ 0.03 &   0 \\
 %    14245 &  265.173553 & -53.655834 &  6036 $\pm$ 14 &  3.78  &   -2.3 $\pm$ 0.04 &   0 \\
 %     5661 &  265.176422 & -53.679142 &  6390 $\pm$ 19 &  4.12  &  -2.42 $\pm$ 0.09 &   0 \\
 %    10445 &  265.175903 & -53.664577 &  5219 $\pm$ 13 &  2.27  &  -2.18 $\pm$ 0.02 &   0 \\
 %     4649 &  265.192188 & -53.677902 &  6044 $\pm$ 23 &  3.77  &  -2.47 $\pm$ 0.09 &   0 \\
 %     1856 &  265.174927 & -53.694283 &  6477 $\pm$ 16 &   4.1  &  -2.76 $\pm$ 0.09 &   0 \\
 % 24000157 &  265.185092 & -53.634733 &  5586 $\pm$ 17 &   3.3  &  -2.07 $\pm$ 0.03 &   0 \\
 %     4293 &  265.200378 & -53.684834 &  5613 $\pm$ 14 &  3.36  &  -2.15 $\pm$ 0.03 &   0 \\
 %    10575 &  265.174467 & -53.665221 &  6422 $\pm$ 19 &  4.06  &  -2.24 $\pm$ 0.08 &   1 \\
 % 15000007 &  265.202091 & -53.644879 &  6402 $\pm$ 13 &  4.17  &  -2.29 $\pm$ 0.05 &   0 \\
 %     1594 &  265.181030 & -53.695374 &  6427 $\pm$ 25 &  4.16  &  -2.62 $\pm$ 0.14 &   0 \\
 % 19000147 &  265.103105 & -53.656063 &  6349 $\pm$ 14 &  4.16  &  -2.47 $\pm$ 0.07 &   0 \\
 %    11673 &  265.155136 & -53.662369 &  6340 $\pm$ 14 &  4.03  &  -2.13 $\pm$ 0.05 &   0 \\
 %     4846 &  265.189056 & -53.680962 &  5804 $\pm$ 13 &  3.59  &  -2.27 $\pm$ 0.03 &   0 \\
 %     4872 &  265.188577 & -53.684627 &   5080 $\pm$ 3 &  1.69  &  -2.08 $\pm$ 0.01 &   0 \\
 %    14085 &  265.177551 & -53.656151 &  5579 $\pm$ 13 &  3.33  &  -2.11 $\pm$ 0.02 &   0 \\
 %    15032 &  265.150653 & -53.648981 &   5409 $\pm$ 9 &  2.86  &  -2.08 $\pm$ 0.02 &   0 \\
 %     7221 &  265.151059 & -53.687436 &  6227 $\pm$ 15 &  3.91  &  -2.13 $\pm$ 0.05 &   0 \\
 % 18000204 &  265.114513 & -53.653536 &  6250 $\pm$ 11 &  3.93  &   -2.4 $\pm$ 0.04 &   0 \\
 %      172 &  265.168488 & -53.704308 &  6518 $\pm$ 16 &  4.05  &  -2.65 $\pm$ 0.09 &   0 \\
 %     9088 &  265.199860 & -53.672363 &  6307 $\pm$ 14 &  4.09  &  -2.45 $\pm$ 0.06 &   0 \\
 % 18000166 &  265.119849 & -53.649125 &  6435 $\pm$ 12 &  4.18  &  -2.27 $\pm$ 0.05 &   0 \\
 %     9663 &  265.187656 & -53.668844 &   5365 $\pm$ 8 &   2.7  &  -2.11 $\pm$ 0.01 &   0 \\
 %     5957 &  265.173615 & -53.674103 &  5271 $\pm$ 11 &  2.35  &  -2.16 $\pm$ 0.02 &   0 \\
 %     7321 &  265.148373 & -53.674231 &  6338 $\pm$ 17 &  4.13  &  -2.26 $\pm$ 0.07 &   0 \\
 % 11000076 &  265.121762 & -53.691899 &  6340 $\pm$ 10 &  4.03  &  -2.22 $\pm$ 0.04 &   0 \\
 %     5714 &  265.175751 & -53.684452 &  6315 $\pm$ 15 &  4.06  &  -2.37 $\pm$ 0.07 &   0 \\
 %     4293 &  265.200367 & -53.684834 &  5627 $\pm$ 14 &  3.36  &  -2.04 $\pm$ 0.03 &   0 \\
 % 22000026 &  265.233454 & -53.664833 &  5739 $\pm$ 11 &  3.55  &  -2.11 $\pm$ 0.02 &   0 \\
 %     4527 &  265.195018 & -53.684173 &  5653 $\pm$ 14 &  3.51  &  -2.25 $\pm$ 0.03 &   0 \\
 %    12803 &  265.119528 & -53.671657 &  6319 $\pm$ 15 &  4.14  &  -2.38 $\pm$ 0.06 &   1 \\
 %     1352 &  265.187491 & -53.690186 &  6323 $\pm$ 18 &  4.11  &   -2.2 $\pm$ 0.07 &   0 \\
 % 22000012 &  265.234869 & -53.673104 &  5867 $\pm$ 11 &  3.65  &  -2.17 $\pm$ 0.03 &   0 \\
 %    11391 &  265.160645 & -53.666260 &  5550 $\pm$ 16 &  3.26  &  -2.16 $\pm$ 0.03 &   0 \\
 %     6933 &  265.157619 & -53.676874 &  6401 $\pm$ 16 &  4.15  &   -2.5 $\pm$ 0.08 &   0 \\
 %     1213 &  265.191473 & -53.695849 &  6157 $\pm$ 15 &  3.88  &  -2.17 $\pm$ 0.05 &   0 \\
 %      893 &  265.202393 & -53.688396 &  6358 $\pm$ 23 &  4.18  &   -2.32 $\pm$ 0.1 &   0 \\
 %     6653 &  265.163025 & -53.676964 &  5579 $\pm$ 12 &  3.35  &  -2.15 $\pm$ 0.02 &   0 \\
 %    10244 &  265.178436 & -53.670845 &  6434 $\pm$ 17 &  4.04  &  -2.58 $\pm$ 0.09 &   0 \\
 %    15349 &  265.136781 & -53.658072 &  6391 $\pm$ 13 &  4.16  &  -2.21 $\pm$ 0.05 &   0 \\
 %     9892 &  265.183350 & -53.671150 &  5574 $\pm$ 12 &  3.23  &  -2.26 $\pm$ 0.03 &   0 \\
 %     8769 &  265.208008 & -53.665508 &  5470 $\pm$ 11 &  2.97  &  -2.26 $\pm$ 0.02 &   0 \\
 % 13000076 &  265.189135 & -53.706685 &  6413 $\pm$ 11 &  4.02  &  -2.43 $\pm$ 0.06 &   0 \\
 %     8983 &  265.202236 & -53.664430 &  5790 $\pm$ 14 &  3.65  &  -2.24 $\pm$ 0.03 &   0 \\
 %    11435 &  265.159865 & -53.670071 &  6165 $\pm$ 17 &  3.85  &  -2.21 $\pm$ 0.06 &   0 \\
 %     4642 &  265.192312 & -53.684904 &  6394 $\pm$ 15 &  4.04  &  -2.45 $\pm$ 0.07 &   0 \\
 %     6808 &  265.159973 & -53.676121 &  6295 $\pm$ 14 &  3.99  &  -2.43 $\pm$ 0.06 &   0 \\
 %     4885 &  265.188293 & -53.679142 &  6479 $\pm$ 24 &  4.05  &   -2.24 $\pm$ 0.1 &   0 \\
 %     8671 &  265.210724 & -53.662483 &  6374 $\pm$ 18 &  4.17  &  -2.65 $\pm$ 0.09 &   0 \\
 %    13228 &  265.204814 & -53.653103 &  6072 $\pm$ 11 &  3.82  &  -2.22 $\pm$ 0.03 &   1 \\
 %     7116 &  265.153351 & -53.682575 &  6423 $\pm$ 14 &  4.11  &  -2.33 $\pm$ 0.07 &   0 \\
 %     6691 &  265.162137 & -53.683439 &  5834 $\pm$ 12 &  3.66  &  -2.06 $\pm$ 0.03 &   0 \\
 %    11478 &  265.159181 & -53.664024 &  6375 $\pm$ 16 &  4.14  &  -2.33 $\pm$ 0.07 &   0 \\
 % 23000380 &  265.220591 & -53.656580 &  5859 $\pm$ 11 &  3.61  &  -2.12 $\pm$ 0.03 &   0 \\
 % 22000019 &  265.243476 & -53.671728 &  6403 $\pm$ 12 &  4.12  &  -2.28 $\pm$ 0.05 &   0 \\
 %    14882 &  265.155060 & -53.659477 &  6419 $\pm$ 24 &   4.1  &  -2.91 $\pm$ 0.13 &   0 \\
 %    13540 &  265.193787 & -53.649162 &  6432 $\pm$ 17 &  4.19  &  -2.47 $\pm$ 0.09 &   0 \\
 %     2427 &  265.159363 & -53.700153 &  5798 $\pm$ 14 &  3.61  &  -2.32 $\pm$ 0.04 &   0 \\
 %     6693 &  265.162018 & -53.681976 &  6200 $\pm$ 15 &  4.15  &  -2.15 $\pm$ 0.05 &   0 \\
 % 11000128 &  265.120917 & -53.697000 &   5407 $\pm$ 9 &  2.81  &  -2.12 $\pm$ 0.02 &   0 \\
 %    15103 &  265.148242 & -53.649566 &  6144 $\pm$ 10 &  3.86  &  -2.26 $\pm$ 0.03 &   0 \\
 %     3712 &  265.216980 & -53.677757 &  6344 $\pm$ 19 &  4.11  &  -2.17 $\pm$ 0.07 &   0 \\
 %    10152 &  265.179749 & -53.671654 &  5797 $\pm$ 14 &  3.62  &  -2.31 $\pm$ 0.04 &   0 \\
 %    11264 &  265.163099 & -53.661161 &  6189 $\pm$ 13 &  3.91  &  -2.31 $\pm$ 0.05 &   0 \\
 %     2571 &  265.156219 & -53.698170 &  5878 $\pm$ 13 &  3.62  &  -2.23 $\pm$ 0.03 &   0 \\
 %    11687 &  265.154414 & -53.670368 &  6419 $\pm$ 20 &  4.19  &   -2.62 $\pm$ 0.1 &   0 \\
 %     4976 &  265.186191 & -53.684732 &  6249 $\pm$ 28 &  4.06  &   -2.21 $\pm$ 0.1 &   0 \\
 %     4440 &  265.197357 & -53.675968 &  5691 $\pm$ 26 &  3.42  &  -2.27 $\pm$ 0.06 &   0 \\
 %     6307 &  265.169189 & -53.673920 &  6347 $\pm$ 15 &  4.14  &  -2.79 $\pm$ 0.07 &   0 \\
 %     3300 &  265.231865 & -53.681414 &  5345 $\pm$ 11 &  2.74  &  -2.15 $\pm$ 0.02 &   1 \\
 %     8624 &  265.211823 & -53.673603 &  5469 $\pm$ 10 &  2.91  &  -2.22 $\pm$ 0.02 &   0 \\
 % 20000048 &  265.113547 & -53.681705 &  6242 $\pm$ 12 &   3.9  &  -2.21 $\pm$ 0.04 &   0 \\
 %     2443 &  265.159546 & -53.688152 &  6106 $\pm$ 23 &  3.94  &  -2.43 $\pm$ 0.09 &   0 \\
 %     9897 &  265.183380 & -53.667782 &  6337 $\pm$ 14 &  4.11  &  -2.59 $\pm$ 0.07 &   0 \\
 %     1620 &  265.180790 & -53.692657 &  6354 $\pm$ 14 &  4.02  &  -2.39 $\pm$ 0.06 &   0 \\
 % 20000099 &  265.111980 & -53.673236 &   5127 $\pm$ 7 &  2.04  &  -2.13 $\pm$ 0.01 &   0 \\
 %     2115 &  265.167664 & -53.697929 &   5160 $\pm$ 8 &  2.08  &  -2.17 $\pm$ 0.01 &   0 \\
 %     1602 &  265.181151 & -53.690844 &  5819 $\pm$ 14 &  3.66  &  -2.24 $\pm$ 0.04 &   0 \\
 %    12014 &  265.146667 & -53.668499 &  5348 $\pm$ 10 &  2.54  &  -2.23 $\pm$ 0.02 &   0 \\
 %     9280 &  265.195737 & -53.665639 &   5135 $\pm$ 7 &  2.03  &  -2.16 $\pm$ 0.01 &   0 \\
 % 14000005 &  265.208836 & -53.705706 &  6215 $\pm$ 13 &  3.92  &  -2.22 $\pm$ 0.05 &   0 \\
 %    16097 &  265.155262 & -53.644677 &  6044 $\pm$ 11 &  3.83  &  -2.21 $\pm$ 0.03 &   0 \\
 %     5387 &  265.180328 & -53.679047 &  6331 $\pm$ 13 &  4.08  &  -2.27 $\pm$ 0.05 &   0 \\
 %     1348 &  265.187477 & -53.690805 &  6344 $\pm$ 15 &  4.07  &  -2.13 $\pm$ 0.05 &   0 \\
 %     1981 &  265.171173 & -53.691387 &  5631 $\pm$ 12 &  3.39  &  -2.18 $\pm$ 0.03 &   0 \\
 %     3274 &  265.233093 & -53.680732 &  6251 $\pm$ 21 &  3.87  &  -2.22 $\pm$ 0.08 &   0 \\
 %    11673 &  265.155151 & -53.662369 &  6313 $\pm$ 26 &  4.03  &  -2.65 $\pm$ 0.13 &   0 \\
 %     3418 &  265.226898 & -53.678059 &  6486 $\pm$ 20 &  4.11  &  -2.97 $\pm$ 0.11 &   0 \\
 %    12112 &  265.143799 & -53.669228 &  6292 $\pm$ 16 &   4.1  &  -2.44 $\pm$ 0.07 &   0 \\
 % 18000206 &  265.125283 & -53.651426 &  6203 $\pm$ 11 &  3.88  &  -2.23 $\pm$ 0.04 &   0 \\
 %     9198 &  265.197767 & -53.660686 &  6452 $\pm$ 18 &  4.07  &  -2.16 $\pm$ 0.08 &   0 \\
 %    14557 &  265.164978 & -53.658134 &  5711 $\pm$ 19 &  3.49  &  -2.36 $\pm$ 0.05 &   0 \\
 %    11484 &  265.159105 & -53.661042 &  6380 $\pm$ 13 &  4.06  &  -2.65 $\pm$ 0.06 &   0 \\
 %    14833 &  265.156598 & -53.655488 &  5831 $\pm$ 13 &  3.68  &  -2.24 $\pm$ 0.03 &   0 \\
 % 18000049 &  265.122856 & -53.652274 &  5796 $\pm$ 11 &  3.58  &  -2.16 $\pm$ 0.03 &   0 \\
 %     1288 &  265.189702 & -53.688675 &  6373 $\pm$ 16 &  4.12  &  -2.57 $\pm$ 0.07 &   0 \\
 %     9211 &  265.197235 & -53.670853 &  6405 $\pm$ 21 &  4.01  &  -2.16 $\pm$ 0.09 &   0 \\
 %    11943 &  265.149150 & -53.662584 &  6275 $\pm$ 14 &   4  &  -2.49 $\pm$ 0.06 &   0 \\
 %     1921 &  265.173309 & -53.691853 &  6433 $\pm$ 16 &  4.11  &  -2.28 $\pm$ 0.07 &   0 \\
 %    11813 &  265.152161 & -53.669430 &  6327 $\pm$ 18 &  4.14  &  -2.43 $\pm$ 0.09 &   0 \\
 % 16000266 &  265.169746 & -53.636677 &  6318 $\pm$ 13 &  3.98  &  -2.25 $\pm$ 0.05 &   0 \\
 %     8071 &  265.126276 & -53.682098 &  6486 $\pm$ 23 &  4.14  &  -2.46 $\pm$ 0.12 &   0 \\
 %     9769 &  265.186096 & -53.669746 &  6380 $\pm$ 16 &   4.1  &  -2.29 $\pm$ 0.07 &   0 \\
 %     8571 &  265.213531 & -53.669235 &  5928 $\pm$ 14 &   3.7  &  -2.31 $\pm$ 0.04 &   0 \\
 %     4668 &  265.191727 & -53.679771 &  6346 $\pm$ 15 &  4.07  &  -2.34 $\pm$ 0.06 &   0 \\
 % 13000050 &  265.181294 & -53.711740 &  6360 $\pm$ 14 &  4.17  &  -2.44 $\pm$ 0.07 &   0 \\
 %     4642 &  265.192322 & -53.684902 &  6376 $\pm$ 14 &  4.04  &  -2.54 $\pm$ 0.07 &   0 \\
 %    10869 &  265.170131 & -53.663402 &  5646 $\pm$ 17 &  3.62  &  -1.96 $\pm$ 0.03 &   0 \\
 %    10113 &  265.180359 & -53.671135 &  6367 $\pm$ 16 &  4.15  &  -2.55 $\pm$ 0.08 &   0 \\
 %     6220 &  265.169891 & -53.674862 &  5324 $\pm$ 11 &  2.06  &  -2.58 $\pm$ 0.02 &   0 \\
 %     2095 &  265.168274 & -53.697445 &  5644 $\pm$ 13 &  3.49  &  -2.17 $\pm$ 0.03 &   0 \\
 %    11106 &  265.165802 & -53.667366 &  6358 $\pm$ 26 &  4.17  &  -2.48 $\pm$ 0.11 &   0 \\
 %     4659 &  265.191620 & -53.683132 &  6435 $\pm$ 15 &  4.13  &  -2.43 $\pm$ 0.08 &   0 \\
 %     3109 &  265.136785 & -53.690044 &  6383 $\pm$ 13 &  4.09  &  -2.26 $\pm$ 0.05 &   0 \\
 %     5002 &  265.186017 & -53.676847 &  6449 $\pm$ 26 &   4.2  &   -2.09 $\pm$ 0.1 &   0 \\
 %    11687 &  265.154419 & -53.670368 &  6410 $\pm$ 20 &  4.19  &   -2.4 $\pm$ 0.09 &   0 \\
 % 15000371 &  265.198754 & -53.639292 &  6185 $\pm$ 17 &  3.93  &  -2.25 $\pm$ 0.06 &   0 \\
 %     5854 &  265.174988 & -53.676373 &  6357 $\pm$ 24 &  4.06  &   -2.6 $\pm$ 0.11 &   0 \\
 % 24000069 &  265.201089 & -53.632018 &  5587 $\pm$ 11 &  3.34  &  -2.26 $\pm$ 0.02 &   0 \\
 %     6677 &  265.162240 & -53.680163 &  6310 $\pm$ 15 &  4.13  &  -2.52 $\pm$ 0.07 &   0 \\
 %    10738 &  265.172184 & -53.660407 &  6283 $\pm$ 23 &  4.03  &  -2.18 $\pm$ 0.09 &   0 \\
 % 12000127 &  265.153054 & -53.723531 &  5866 $\pm$ 10 &   3.6  &   -2.1 $\pm$ 0.02 &   0 \\
 %     5373 &  265.180115 & -53.683445 &  6453 $\pm$ 17 &  4.16  &  -2.63 $\pm$ 0.09 &   0 \\
 %     9385 &  265.193665 & -53.669792 &  5362 $\pm$ 10 &  2.63  &  -2.43 $\pm$ 0.02 &   0 \\
 %     6692 &  265.162076 & -53.682601 &   5021 $\pm$ 4 &  1.22  &  -1.85 $\pm$ 0.01 &   0 \\
 %     5587 &  265.177673 & -53.675041 &  6390 $\pm$ 23 &  4.05  &  -2.91 $\pm$ 0.12 &   0 \\
 % 21000286 &  265.243416 & -53.676769 &  5713 $\pm$ 29 &  3.46  &  -2.33 $\pm$ 0.07 &   0 \\
 %      796 &  265.206879 & -53.690481 &  6305 $\pm$ 16 &  4.03  &  -2.36 $\pm$ 0.07 &   0 \\
 %     4524 &  265.194763 & -53.685608 &  6349 $\pm$ 14 &  4.04  &  -2.49 $\pm$ 0.06 &   0 \\
 %     5616 &  265.177091 & -53.680240 &  6400 $\pm$ 16 &  4.14  &  -2.43 $\pm$ 0.07 &   0 \\
 %     3168 &  265.238754 & -53.681660 &  5647 $\pm$ 11 &   3.4  &  -2.15 $\pm$ 0.02 &   0 \\
 %     5692 &  265.176501 & -53.674819 &  6315 $\pm$ 47 &  4.17  &  -2.31 $\pm$ 0.16 &   0 \\
 %     5159 &  265.183014 & -53.681065 &  6334 $\pm$ 14 &  3.97  &  -2.57 $\pm$ 0.07 &   0 \\
 %     9159 &  265.199043 & -53.662589 &   5057 $\pm$ 2 &  1.55  &  -2.01 $\pm$ 0.01 &   0 \\
 % 15000079 &  265.212352 & -53.642677 &  6299 $\pm$ 12 &  4.02  &  -2.23 $\pm$ 0.04 &   0 \\
 %    11758 &  265.152898 & -53.666746 &   5162 $\pm$ 7 &  2.13  &  -2.16 $\pm$ 0.01 &   0 \\
 %     6910 &  265.158709 & -53.676260 &  6359 $\pm$ 16 &  4.02  &  -2.29 $\pm$ 0.07 &   0 \\
 %     9100 &  265.200098 & -53.666301 &  6368 $\pm$ 23 &  4.18  &  -2.01 $\pm$ 0.08 &   0 \\
 %     5148 &  265.183655 & -53.674080 &  6148 $\pm$ 14 &  3.85  &  -2.26 $\pm$ 0.05 &   0 \\
 %    12004 &  265.147308 & -53.666454 &  5401 $\pm$ 10 &  2.79  &  -2.22 $\pm$ 0.02 &   0 \\
 %     5159 &  265.183007 & -53.681064 &  6283 $\pm$ 16 &  3.97  &  -2.45 $\pm$ 0.07 &   0 \\
 %     7840 &  265.135223 & -53.675148 &  5899 $\pm$ 13 &  3.74  &  -2.37 $\pm$ 0.04 &   0 \\
 %      390 &  265.157330 & -53.712941 &  6406 $\pm$ 14 &  4.05  &  -2.33 $\pm$ 0.07 &   0 \\
 %     7212 &  265.151680 & -53.678459 &  5741 $\pm$ 12 &  3.56  &  -2.19 $\pm$ 0.03 &   0 \\
 %     4758 &  265.190491 & -53.674477 &  5667 $\pm$ 21 &   3.6  &  -2.12 $\pm$ 0.04 &   0 \\
 %     2747 &  265.150940 & -53.695572 &   5131 $\pm$ 8 &  2.05  &  -2.13 $\pm$ 0.02 &   0 \\
 %     6039 &  265.172760 & -53.675331 &  6261 $\pm$ 14 &  3.97  &  -2.46 $\pm$ 0.06 &   0 \\
 % 15000624 &  265.209155 & -53.638802 &  6410 $\pm$ 14 &  4.15  &  -2.38 $\pm$ 0.07 &   0 \\
 % 13000313 &  265.174565 & -53.715814 &  6409 $\pm$ 16 &   4.1  &   -3  &   1 \\
 %     5235 &  265.181915 & -53.686775 &  6037 $\pm$ 12 &  3.76  &  -2.33 $\pm$ 0.04 &   0 \\
 %     7155 &  265.152496 & -53.676430 &  5667 $\pm$ 12 &  3.49  &  -2.09 $\pm$ 0.03 &   0 \\
 % 22000224 &  265.234430 & -53.664508 &  6357 $\pm$ 12 &  4.09  &  -2.54 $\pm$ 0.05 &   0 \\
 %    10937 &  265.168976 & -53.667912 &  6284 $\pm$ 12 &  3.93  &  -2.48 $\pm$ 0.05 &   0 \\
 %    14479 &  265.167389 & -53.658169 &  6393 $\pm$ 28 &  4.05  &  -2.81 $\pm$ 0.15 &   0 \\
 % 19000177 &  265.107920 & -53.660443 &   5219 $\pm$ 9 &  2.37  &  -2.07 $\pm$ 0.01 &   0 \\
 %     4525 &  265.194744 & -53.685242 &  6123 $\pm$ 14 &   3.9  &   -2.4 $\pm$ 0.05 &   0 \\
 %    11011 &  265.167747 & -53.661634 &   5360 $\pm$ 8 &  2.75  &  -2.15 $\pm$ 0.01 &   0 \\
 %    12514 &  265.130066 & -53.669952 &  6398 $\pm$ 16 &  4.08  &  -2.58 $\pm$ 0.08 &   0 \\
 %     1261 &  265.190100 & -53.691071 &  6384 $\pm$ 18 &  4.19  &  -2.01 $\pm$ 0.06 &   1 \\
 %     8296 &  265.223012 & -53.665779 &  6306 $\pm$ 11 &  3.99  &  -2.35 $\pm$ 0.04 &   0 \\
 %     6398 &  265.167053 & -53.679577 &  5658 $\pm$ 14 &  3.44  &  -2.25 $\pm$ 0.03 &   0 \\
 %     7444 &  265.144954 & -53.684000 &   5513 $\pm$ 9 &  3.03  &  -2.13 $\pm$ 0.02 &   0 \\
 %     6632 &  265.163483 & -53.673927 &  6330 $\pm$ 13 &  4.04  &  -2.63 $\pm$ 0.06 &   0 \\
 %     5310 &  265.181462 & -53.677019 &  6258 $\pm$ 24 &  4.07  &  -2.49 $\pm$ 0.09 &   0 \\
 %     5314 &  265.181091 & -53.676579 &  5161 $\pm$ 10 &  2.08  &  -2.17 $\pm$ 0.02 &   0 \\
 % 19000119 &  265.105249 & -53.660587 &  5924 $\pm$ 10 &  3.68  &  -2.23 $\pm$ 0.03 &   0 \\
 %    10608 &  265.173599 & -53.665670 &  5378 $\pm$ 15 &   2.7  &  -2.19 $\pm$ 0.03 &   0 \\
 % 12000069 &  265.157768 & -53.719790 &  6410 $\pm$ 13 &  4.18  &  -2.36 $\pm$ 0.06 &   0 \\
 %     1982 &  265.171265 & -53.690681 &  5377 $\pm$ 10 &  2.56  &  -2.25 $\pm$ 0.02 &   0 \\
 %    13452 &  265.196694 & -53.647500 &  5511 $\pm$ 10 &  3.17  &  -2.08 $\pm$ 0.02 &   0 \\
 %    15801 &  265.184951 & -53.635443 &  6374 $\pm$ 10 &  3.87  &  -2.26 $\pm$ 0.04 &   0 \\
 % 11000016 &  265.130635 & -53.690050 &  6432 $\pm$ 11 &  4.11  &  -2.45 $\pm$ 0.06 &   0 \\
 %     5863 &  265.174896 & -53.674515 &  6175 $\pm$ 13 &  3.86  &  -2.44 $\pm$ 0.05 &   0 \\
 %     3855 &  265.212891 & -53.679085 &  5931 $\pm$ 13 &  3.73  &   -2.6 $\pm$ 0.05 &   0 \\
 %    14763 &  265.159127 & -53.656366 &  6334 $\pm$ 18 &  4.08  &  -2.54 $\pm$ 0.08 &   0 \\
 %    10062 &  265.181152 & -53.664360 &  6346 $\pm$ 13 &  4.06  &  -2.57 $\pm$ 0.07 &   0 \\
 %    10052 &  265.181152 & -53.669495 &  6335 $\pm$ 12 &  4.02  &  -2.49 $\pm$ 0.06 &   0 \\
 %     7729 &  265.137512 & -53.681061 &  6279 $\pm$ 12 &  3.96  &  -2.68 $\pm$ 0.06 &   0 \\
 %    11517 &  265.157654 & -53.670082 &  6383 $\pm$ 18 &  3.93  &   -2.72 $\pm$ 0.1 &   0 \\
 % 23000210 &  265.213271 & -53.657419 &  6405 $\pm$ 12 &  4.13  &  -2.39 $\pm$ 0.06 &   0 \\
 %    11801 &  265.152360 & -53.660112 &  6186 $\pm$ 13 &  3.84  &  -2.33 $\pm$ 0.05 &   0 \\
 %     8448 &  265.216785 & -53.664644 &  6328 $\pm$ 12 &  4.15  &  -2.39 $\pm$ 0.05 &   0 \\
 %    11052 &  265.166504 & -53.673489 &  5327 $\pm$ 10 &  2.52  &   -2.2 $\pm$ 0.02 &   0 \\
 %     6676 &  265.162637 & -53.680517 &  6186 $\pm$ 15 &  3.89  &  -2.52 $\pm$ 0.07 &   0 \\
 %    11035 &  265.166979 & -53.667865 &  6046 $\pm$ 22 &  3.85  &  -2.16 $\pm$ 0.06 &   0 \\
 %     5796 &  265.175507 & -53.678024 &  6431 $\pm$ 34 &  4.15  &   -1.74 $\pm$ 0.1 &   0 \\
 %     6757 &  265.160796 & -53.683337 &   5285 $\pm$ 8 &  2.58  &  -2.12 $\pm$ 0.01 &   0 \\
 %    14166 &  265.175873 & -53.646362 &  6352 $\pm$ 16 &  4.09  &   -2.7 $\pm$ 0.08 &   0 \\
 %     9267 &  265.195740 & -53.670483 &  5749 $\pm$ 13 &   3.6  &  -2.29 $\pm$ 0.03 &   0 \\
 %      172 &  265.168480 & -53.704306 &  6279 $\pm$ 16 &  4.05  &  -2.38 $\pm$ 0.06 &   0 \\
 %    11919 &  265.149658 & -53.662357 &  5444 $\pm$ 13 &  2.95  &  -2.17 $\pm$ 0.02 &   0 \\
 % 15000108 &  265.199795 & -53.637100 &  6068 $\pm$ 11 &  3.82  &  -2.21 $\pm$ 0.03 &   0 \\
 %     8769 &  265.208015 & -53.665508 &   5477 $\pm$ 9 &  2.97  &  -2.14 $\pm$ 0.02 &   0 \\
 %     5970 &  265.173370 & -53.682537 &   5109 $\pm$ 7 &  1.86  &  -2.18 $\pm$ 0.02 &   0 \\
 %     4868 &  265.188293 & -53.686333 &  6388 $\pm$ 16 &  4.18  &  -2.79 $\pm$ 0.08 &   0 \\
 %     6904 &  265.158140 & -53.678204 &  6032 $\pm$ 13 &  3.79  &  -2.29 $\pm$ 0.04 &   0 \\
 %     4649 &  265.192200 & -53.677902 &  6022 $\pm$ 13 &  3.77  &  -2.38 $\pm$ 0.04 &   0 \\
 %     2726 &  265.151550 & -53.696537 &  5782 $\pm$ 16 &   4.1  &  -1.94 $\pm$ 0.03 &   0 \\
 %    11478 &  265.159180 & -53.664024 &  6288 $\pm$ 24 &  4.14  &   -2.47 $\pm$ 0.1 &   0 \\
 % 18000168 &  265.124372 & -53.648964 &  6352 $\pm$ 11 &  4.05  &  -2.44 $\pm$ 0.05 &   0 \\
 %     5095 &  265.184214 & -53.681936 &  5782 $\pm$ 13 &  3.58  &  -2.23 $\pm$ 0.03 &   0 \\
 %     5901 &  265.173994 & -53.676812 &  6352 $\pm$ 16 &  4.11  &  -2.42 $\pm$ 0.07 &   0 \\
 %     6478 &  265.166138 & -53.680286 &  5705 $\pm$ 19 &  3.48  &   -2.2 $\pm$ 0.04 &   0 \\
 %      918 &  265.201111 & -53.690125 &  5907 $\pm$ 13 &  3.72  &  -2.35 $\pm$ 0.04 &   0 \\
 % 16000068 &  265.167867 & -53.638003 &  6417 $\pm$ 14 &  4.16  &  -2.33 $\pm$ 0.06 &   0 \\
 %    11616 &  265.155225 & -53.672744 &  6129 $\pm$ 14 &  3.81  &  -2.29 $\pm$ 0.05 &   0 \\
 % 15000140 &  265.209770 & -53.652177 &  5389 $\pm$ 13 &  2.83  &   -2.1 $\pm$ 0.02 &   0 \\
 %    12506 &  265.130676 & -53.668633 &  6260 $\pm$ 14 &  3.88  &  -2.48 $\pm$ 0.06 &   0 \\
 %    10869 &  265.170135 & -53.663403 &  5469 $\pm$ 26 &  3.62  &  -1.81 $\pm$ 0.04 &   0 \\
 %     9142 &  265.198761 & -53.672020 &  6909 $\pm$ 12 &  3.97  &  -2.32 $\pm$ 0.07 &   0 \\
 %     5241 &  265.181824 & -53.684921 &  6453 $\pm$ 16 &  3.94  &  -2.42 $\pm$ 0.08 &   0 \\
 % 22000118 &  265.238752 & -53.675961 &   5463 $\pm$ 9 &  2.97  &  -2.08 $\pm$ 0.02 &   0 \\
 %     7194 &  265.151414 & -53.687237 &  6361 $\pm$ 13 &   4  &  -2.06 $\pm$ 0.05 &   0 \\
 %     4740 &  265.190557 & -53.682697 &  5755 $\pm$ 13 &  3.57  &  -2.08 $\pm$ 0.03 &   0 \\
 %    11233 &  265.163879 & -53.664394 &  6323 $\pm$ 24 &  4.11  &   -2.6 $\pm$ 0.12 &   1 \\
 %    10575 &  265.174469 & -53.665222 &  6279 $\pm$ 12 &  4.06  &  -2.47 $\pm$ 0.05 &   1 \\
 %      163 &  265.169067 & -53.702396 &  6037 $\pm$ 13 &   3.8  &  -2.61 $\pm$ 0.05 &   0 \\
 % 13000413 &  265.171515 & -53.713823 &  6382 $\pm$ 15 &  4.16  &  -2.51 $\pm$ 0.07 &   0 \\
 %    14788 &  265.157623 & -53.658451 &  5344 $\pm$ 13 &  2.62  &  -2.17 $\pm$ 0.02 &   0 \\
 %    13544 &  265.192810 & -53.659836 &  5458 $\pm$ 10 &  2.89  &  -2.15 $\pm$ 0.02 &   0 \\
 %     4874 &  265.188271 & -53.683131 &  6448 $\pm$ 24 &  4.19  &  -2.55 $\pm$ 0.11 &   0 \\
 %     8933 &  265.203497 & -53.669406 &  6450 $\pm$ 15 &  4.08  &  -2.23 $\pm$ 0.06 &   0 \\
 %     5998 &  265.172913 & -53.674603 &  6353 $\pm$ 19 &  4.04  &   -2.53 $\pm$ 0.1 &   0 \\
 %     7682 &  265.138763 & -53.685333 &  6389 $\pm$ 15 &  4.06  &   -2.7 $\pm$ 0.08 &   0 \\
 %    13679 &  265.189697 & -53.653400 &  5611 $\pm$ 11 &  3.43  &  -2.22 $\pm$ 0.02 &   0 \\
 %     5702 &  265.176418 & -53.673765 &  6146 $\pm$ 37 &  3.82  &  -2.16 $\pm$ 0.12 &   0 \\
 %     6375 &  265.167816 & -53.675564 &  5397 $\pm$ 11 &  2.75  &  -2.26 $\pm$ 0.02 &   0 \\
 % 24000306 &  265.208433 & -53.628295 &  5727 $\pm$ 19 &  3.65  &  -2.09 $\pm$ 0.04 &   0 \\
 % 13000156 &  265.188000 & -53.706135 &  5674 $\pm$ 11 &  3.47  &  -2.06 $\pm$ 0.02 &   0 \\
 %     9035 &  265.201385 & -53.664234 &  6270 $\pm$ 12 &   4  &  -2.37 $\pm$ 0.05 &   1 \\
 %    11985 &  265.147705 & -53.666481 &  6455 $\pm$ 25 &  4.18  &  -2.47 $\pm$ 0.12 &   0 \\
 %     5668 &  265.176361 & -53.678139 &  5763 $\pm$ 12 &  3.59  &  -2.27 $\pm$ 0.03 &   0 \\
 %     9125 &  265.199708 & -53.665143 &  6425 $\pm$ 19 &  4.19  &  -2.51 $\pm$ 0.09 &   0 \\
 %    13275 &  265.202882 & -53.648764 &  6335 $\pm$ 13 &  4.04  &  -2.39 $\pm$ 0.06 &   0 \\
 %    14699 &  265.161295 & -53.650404 &  6430 $\pm$ 12 &  4.15  &  -2.41 $\pm$ 0.06 &   0 \\
 %    10348 &  265.176910 & -53.661034 &  6280 $\pm$ 25 &  3.99  &  -2.46 $\pm$ 0.12 &   0 \\
 %     9739 &  265.186432 & -53.665001 &  5676 $\pm$ 15 &   3.5  &  -2.13 $\pm$ 0.03 &   0 \\
 %     6113 &  265.171051 & -53.680111 &  6100 $\pm$ 11 &  3.83  &  -2.63 $\pm$ 0.05 &   0 \\
 %    14185 &  265.175537 & -53.651440 &  6388 $\pm$ 14 &  4.06  &  -2.75 $\pm$ 0.08 &   0 \\
 %     7037 &  265.155426 & -53.674274 &  6404 $\pm$ 14 &  4.06  &  -2.57 $\pm$ 0.07 &   0 \\
 %    11631 &  265.155726 & -53.664920 &  6002 $\pm$ 13 &  3.75  &  -2.39 $\pm$ 0.04 &   0 \\
 %     4976 &  265.186188 & -53.684731 &  6454 $\pm$ 19 &  4.06  &   -2.48 $\pm$ 0.1 &   0 \\
 % 13000139 &  265.173294 & -53.709481 &  6224 $\pm$ 10 &  3.85  &  -2.26 $\pm$ 0.04 &   0 \\
 % 15000199 &  265.200961 & -53.642600 &  6411 $\pm$ 13 &  4.18  &  -2.52 $\pm$ 0.06 &   0 \\
 %     6692 &  265.162079 & -53.682602 &   5032 $\pm$ 4 &  1.22  &  -1.92 $\pm$ 0.01 &   0 \\
 %     5747 &  265.175751 & -53.677837 &  5930 $\pm$ 13 &  3.65  &  -2.26 $\pm$ 0.04 &   0 \\
 %     9208 &  265.196943 & -53.671489 &  5464 $\pm$ 10 &  3.08  &  -2.11 $\pm$ 0.02 &   0 \\
 %     8592 &  265.212646 & -53.666870 &  6298 $\pm$ 14 &  3.97  &  -2.54 $\pm$ 0.07 &   0 \\
 %     6299 &  265.168884 & -53.675793 &  6424 $\pm$ 17 &  4.11  &   -2.6 $\pm$ 0.09 &   0 \\
 %    11943 &  265.149139 & -53.662582 &  6244 $\pm$ 22 &   4  &  -2.42 $\pm$ 0.09 &   0 \\
 %    10284 &  265.177612 & -53.670395 &  6194 $\pm$ 11 &  3.86  &   -2.4 $\pm$ 0.05 &   0 \\
 %    13006 &  265.111516 & -53.670505 &  6072 $\pm$ 11 &  3.78  &  -2.19 $\pm$ 0.03 &   0 \\
 %     6546 &  265.165100 & -53.680508 &  6375 $\pm$ 15 &  4.14  &  -2.85 $\pm$ 0.08 &   0 \\
 % 16000016 &  265.170834 & -53.636902 &  6264 $\pm$ 23 &  4.11  &  -2.25 $\pm$ 0.09 &   0 \\
 %    13650 &  265.190247 & -53.657993 &  5384 $\pm$ 10 &  2.76  &  -2.23 $\pm$ 0.02 &   0 \\
 %    15130 &  265.146701 & -53.658349 &   5208 $\pm$ 8 &  2.34  &  -2.15 $\pm$ 0.01 &   0 \\
 % 19000101 &  265.092476 & -53.662170 &  6326 $\pm$ 11 &  3.98  &  -2.32 $\pm$ 0.05 &   0 \\
 %     2273 &  265.163757 & -53.696049 &  6371 $\pm$ 15 &  3.99  &  -2.56 $\pm$ 0.08 &   0 \\
 %     1957 &  265.171722 & -53.695831 &  6108 $\pm$ 15 &   3.8  &  -2.47 $\pm$ 0.06 &   0 \\
 %     9900 &  265.183472 & -53.667072 &  6466 $\pm$ 15 &  4.06  &  -2.46 $\pm$ 0.08 &   0 \\
 % 12000243 &  265.171355 & -53.716409 &  6344 $\pm$ 18 &   4  &  -2.49 $\pm$ 0.08 &   0 \\
 %     5313 &  265.181548 & -53.676688 &  5448 $\pm$ 14 &  3.06  &  -2.18 $\pm$ 0.03 &   0 \\
 %    10745 &  265.171600 & -53.672592 &  5543 $\pm$ 13 &  3.31  &  -2.17 $\pm$ 0.03 &   0 \\
 %     9364 &  265.194338 & -53.665417 &  6346 $\pm$ 15 &  4.12  &  -2.25 $\pm$ 0.06 &   0 \\
 %     7547 &  265.142601 & -53.676848 &  5531 $\pm$ 11 &  3.29  &  -2.13 $\pm$ 0.02 &   0 \\
 %     4213 &  265.202517 & -53.687387 &  6268 $\pm$ 35 &  4.03  &   -2.9 $\pm$ 0.16 &   0 \\
 %     6653 &  265.163025 & -53.676964 &  5705 $\pm$ 31 &  3.35  &   -2.2 $\pm$ 0.07 &   0 \\
 %     8933 &  265.203491 & -53.669407 &  6412 $\pm$ 14 &  4.08  &  -2.39 $\pm$ 0.06 &   0 \\
 %     4731 &  265.190704 & -53.686974 &  6223 $\pm$ 13 &  3.93  &   -2.4 $\pm$ 0.05 &   0 \\
 %     4971 &  265.186646 & -53.676441 &  6235 $\pm$ 12 &  3.88  &  -2.27 $\pm$ 0.05 &   0 \\
 %    14744 &  265.159905 & -53.647626 &  6145 $\pm$ 10 &  3.85  &  -2.31 $\pm$ 0.04 &   1 \\
 %    13196 &  265.206099 & -53.651106 &  5689 $\pm$ 18 &  3.53  &   -2.2 $\pm$ 0.04 &   0 \\
 %     2443 &  265.159559 & -53.688153 &  6263 $\pm$ 13 &  3.94  &  -2.34 $\pm$ 0.06 &   0 \\
 %     7617 &  265.140839 & -53.674408 &  6367 $\pm$ 20 &  4.16  &   -2.3 $\pm$ 0.09 &   0 \\
 %    10662 &  265.172607 & -53.673679 &  6394 $\pm$ 13 &  4.09  &  -2.53 $\pm$ 0.07 &   0 \\
 %     2344 &  265.161652 & -53.697311 &  5907 $\pm$ 15 &  3.71  &  -2.32 $\pm$ 0.04 &   0 \\
 %    13787 &  265.186096 & -53.658619 &  6369 $\pm$ 14 &  4.03  &  -2.36 $\pm$ 0.06 &   0 \\
 %     7116 &  265.153340 & -53.682576 &  6389 $\pm$ 14 &  4.11  &   -2.1 $\pm$ 0.05 &   0 \\
 %     5566 &  265.177490 & -53.679703 &  5746 $\pm$ 14 &  3.54  &  -2.26 $\pm$ 0.03 &   0 \\
 %     4352 &  265.199448 & -53.675118 &  5401 $\pm$ 14 &  2.58  &   -2.1 $\pm$ 0.02 &   0 \\
 %     8571 &  265.213516 & -53.669237 &  5921 $\pm$ 14 &   3.7  &  -2.18 $\pm$ 0.04 &   0 \\
 %     9604 &  265.188691 & -53.667871 &  5668 $\pm$ 11 &  3.42  &   -2.1 $\pm$ 0.02 &   0 \\
 %     6752 &  265.160859 & -53.686480 &  5570 $\pm$ 12 &  3.26  &  -2.04 $\pm$ 0.02 &   0 \\
 %     6536 &  265.164978 & -53.682312 &  6327 $\pm$ 15 &  4.01  &  -2.56 $\pm$ 0.07 &   0 \\
 % 21000186 &  265.264140 & -53.687504 &  6418 $\pm$ 13 &  4.19  &  -2.33 $\pm$ 0.06 &   0 \\
 %    11435 &  265.159851 & -53.670071 &  6213 $\pm$ 24 &  3.85  &   -2.46 $\pm$ 0.1 &   0 \\
 %     4931 &  265.187333 & -53.682685 &  6413 $\pm$ 15 &   4.1  &  -2.59 $\pm$ 0.08 &   0 \\
 %    11313 &  265.162014 & -53.667226 &  5473 $\pm$ 10 &  3.04  &  -2.06 $\pm$ 0.02 &   0 \\
 %     7945 &  265.131488 & -53.676944 &  6248 $\pm$ 36 &  4.19  &  -2.16 $\pm$ 0.11 &   0 \\
 % 15000108 &  265.199795 & -53.637100 &  6099 $\pm$ 15 &  3.82  &  -2.45 $\pm$ 0.06 &   0 \\
 %    12431 &  265.133575 & -53.666115 &  6359 $\pm$ 15 &  4.09  &  -2.74 $\pm$ 0.07 &   0 \\
 %    13848 &  265.184479 & -53.648861 &  6288 $\pm$ 13 &  4.03  &  -2.62 $\pm$ 0.06 &   0 \\
 %    10452 &  265.176046 & -53.661685 &  6441 $\pm$ 19 &  4.08  &  -2.78 $\pm$ 0.11 &   0 \\
 %     1264 &  265.190186 & -53.690491 &  6375 $\pm$ 14 &  4.14  &  -2.51 $\pm$ 0.07 &   0 \\
 %     7656 &  265.139862 & -53.677479 &  6361 $\pm$ 14 &   4  &  -2.73 $\pm$ 0.07 &   0 \\
 %      893 &  265.202387 & -53.688395 &  6575 $\pm$ 25 &  4.18  &  -1.93 $\pm$ 0.09 &   0 \\
 %     4917 &  265.187531 & -53.681068 &  6181 $\pm$ 14 &  3.84  &  -2.41 $\pm$ 0.06 &   0 \\
 %     4931 &  265.187347 & -53.682686 &  6407 $\pm$ 13 &   4.1  &  -2.66 $\pm$ 0.07 &   0 \\
 %     4352 &  265.199463 & -53.675117 &  5338 $\pm$ 10 &  2.58  &  -2.21 $\pm$ 0.02 &   0 \\
 %     1669 &  265.179377 & -53.687901 &  5861 $\pm$ 13 &  3.68  &  -2.24 $\pm$ 0.04 &   0 \\
 %     5687 &  265.176804 & -53.675321 &  6017 $\pm$ 36 &  4.19  &   -3  &   0 \\
 %     6015 &  265.172424 & -53.681454 &  6341 $\pm$ 13 &  4.06  &  -2.97 $\pm$ 0.07 &   0 \\
 %     1733 &  265.177734 & -53.695805 &  6491 $\pm$ 18 &  4.14  &   -2.1 $\pm$ 0.08 &   0 \\
 %     4950 &  265.187164 & -53.673817 &  6344 $\pm$ 12 &  4.02  &  -2.64 $\pm$ 0.06 &   0 \\
 %     5233 &  265.182159 & -53.674217 &  6371 $\pm$ 15 &  4.16  &  -2.81 $\pm$ 0.08 &   0 \\
 %     3200 &  265.236424 & -53.681483 &  6303 $\pm$ 11 &  3.93  &  -2.38 $\pm$ 0.05 &   0 \\
 %     5092 &  265.184387 & -53.683075 &  5900 $\pm$ 14 &  3.66  &   -2.3 $\pm$ 0.04 &   0 \\
 %     4758 &  265.190499 & -53.674478 &  5624 $\pm$ 26 &   3.6  &  -1.93 $\pm$ 0.05 &   0 \\
 %     5159 &  265.183007 & -53.681064 &  6343 $\pm$ 26 &  3.97  &  -2.13 $\pm$ 0.09 &   0 \\
 % 22000223 &  265.228724 & -53.664707 &  5973 $\pm$ 28 &  4.13  &  -2.16 $\pm$ 0.07 &   0 \\
 %    15609 &  265.195753 & -53.641891 &  6007 $\pm$ 24 &  3.82  &  -2.32 $\pm$ 0.08 &   0 \\
 %    15659 &  265.192068 & -53.639713 &  6364 $\pm$ 13 &  4.04  &   -2 $\pm$ 0.05 &   0 \\
 % 13000026 &  265.175620 & -53.716023 &  6368 $\pm$ 12 &  4.01  &  -2.31 $\pm$ 0.05 &   1 \\
 % 17000118 &  265.136123 & -53.642813 &  6372 $\pm$ 10 &  4.04  &  -2.36 $\pm$ 0.04 &   0 \\
 %     9830 &  265.184662 & -53.669460 &  6316 $\pm$ 45 &  3.99  &  -2.33 $\pm$ 0.18 &   0 \\
 %     1052 &  265.196116 & -53.698486 &  5633 $\pm$ 12 &  3.55  &  -2.09 $\pm$ 0.02 &   0 \\
 % 23000172 &  265.224145 & -53.664033 &  6392 $\pm$ 11 &   4.1  &  -2.55 $\pm$ 0.06 &   0 \\
 %     6662 &  265.163239 & -53.674366 &  5524 $\pm$ 11 &  3.18  &  -2.23 $\pm$ 0.02 &   0 \\
 %     6168 &  265.170685 & -53.676765 &  6130 $\pm$ 13 &  3.84  &  -2.49 $\pm$ 0.05 &   0 \\
 % 19000179 &  265.085836 & -53.658881 &  6364 $\pm$ 12 &  4.13  &  -2.19 $\pm$ 0.05 &   0 \\
 %     2462 &  265.158966 & -53.691471 &  6529 $\pm$ 18 &  4.16  &   -2.47 $\pm$ 0.1 &   0 \\
 %     6484 &  265.166229 & -53.677643 &  5246 $\pm$ 11 &  2.29  &  -2.24 $\pm$ 0.02 &   0 \\
 % 20000167 &  265.106954 & -53.680753 &  6422 $\pm$ 13 &  4.16  &  -2.45 $\pm$ 0.06 &   0 \\
 %      771 &  265.208466 & -53.688618 &  5911 $\pm$ 13 &  3.71  &  -2.44 $\pm$ 0.04 &   0 \\
 % 15000097 &  265.193993 & -53.639818 &   5525 $\pm$ 9 &  3.26  &  -2.02 $\pm$ 0.02 &   0 \\
 % 22000200 &  265.241278 & -53.667763 &  6358 $\pm$ 13 &  4.07  &   -2.3 $\pm$ 0.05 &   0 \\
 %    14672 &  265.161719 & -53.655114 &  6327 $\pm$ 18 &  4.17  &  -1.98 $\pm$ 0.05 &   0 \\
 %    14758 &  265.159149 & -53.658676 &  6487 $\pm$ 24 &  4.15  &  -2.73 $\pm$ 0.13 &   0 \\
 % 17000120 &  265.147361 & -53.642559 &  5638 $\pm$ 11 &  3.49  &  -2.14 $\pm$ 0.02 &   0 \\
 %     1552 &  265.182355 & -53.690693 &  6366 $\pm$ 17 &  4.16  &  -2.45 $\pm$ 0.08 &   0 \\
 %     1542 &  265.182709 & -53.694763 &  6133 $\pm$ 13 &  3.82  &   -2.6 $\pm$ 0.05 &   0 \\
 %     5648 &  265.176788 & -53.683189 &  5513 $\pm$ 13 &  2.97  &   -2.1 $\pm$ 0.02 &   0 \\
 %     5031 &  265.185638 & -53.679897 &   5404 $\pm$ 9 &  2.35  &  -2.28 $\pm$ 0.02 &   0 \\
 %     9865 &  265.184082 & -53.667587 &  6315 $\pm$ 16 &  3.96  &  -2.59 $\pm$ 0.08 &   0 \\
 %    13610 &  265.191803 & -53.648533 &  5508 $\pm$ 11 &  3.26  &  -2.12 $\pm$ 0.02 &   0 \\
 % 15000015 &  265.207431 & -53.641613 &  6335 $\pm$ 11 &  4.07  &  -2.45 $\pm$ 0.05 &   1 \\
 %    14557 &  265.164966 & -53.658136 &  5647 $\pm$ 12 &  3.49  &  -2.13 $\pm$ 0.02 &   0 \\
 %      907 &  265.201039 & -53.697104 &  6207 $\pm$ 24 &  3.93  &  -2.35 $\pm$ 0.09 &   0 \\
 %    11951 &  265.148376 & -53.671555 &  6393 $\pm$ 17 &  4.17  &  -2.64 $\pm$ 0.09 &   0 \\
 %    12630 &  265.125946 & -53.673428 &  6386 $\pm$ 15 &  4.02  &  -2.58 $\pm$ 0.07 &   1 \\
 %    11085 &  265.166779 & -53.661701 &  5639 $\pm$ 16 &  3.43  &  -2.19 $\pm$ 0.03 &   0 \\
 %     5451 &  265.179260 & -53.674465 &  6411 $\pm$ 16 &  4.07  &  -2.56 $\pm$ 0.08 &   0 \\
 %     8324 &  265.221258 & -53.671606 &  5804 $\pm$ 11 &  3.62  &  -2.07 $\pm$ 0.03 &   0 \\
 %     4860 &  265.188666 & -53.674692 &  5464 $\pm$ 11 &  3.06  &  -2.11 $\pm$ 0.02 &   0 \\
 %     5894 &  265.174530 & -53.678032 &  6406 $\pm$ 14 &  4.17  &  -2.55 $\pm$ 0.07 &   0 \\
 %    10552 &  265.175099 & -53.660033 &  6150 $\pm$ 14 &  3.86  &  -2.32 $\pm$ 0.05 &   0 \\
 %     9281 &  265.196189 & -53.665148 &  6380 $\pm$ 16 &  4.16  &  -2.19 $\pm$ 0.06 &   0 \\
 %     1824 &  265.175903 & -53.689728 &   5064 $\pm$ 7 &  1.35  &  -1.92 $\pm$ 0.03 &   0 \\
 % 23000132 &  265.225492 & -53.650551 &  6399 $\pm$ 12 &  4.13  &  -2.24 $\pm$ 0.05 &   0 \\
 % 12000301 &  265.164234 & -53.717599 &  6408 $\pm$ 13 &  4.09  &  -2.31 $\pm$ 0.06 &   0 \\
 %     9281 &  265.196198 & -53.665150 &  6339 $\pm$ 15 &  4.16  &  -2.28 $\pm$ 0.06 &   0 \\
 %    14319 &  265.171997 & -53.655952 &  5934 $\pm$ 15 &   3.7  &  -2.31 $\pm$ 0.04 &   0 \\
 %     7037 &  265.155425 & -53.674275 &  6346 $\pm$ 14 &  4.06  &  -2.11 $\pm$ 0.05 &   0 \\
 %     9001 &  265.201693 & -53.670300 &  6401 $\pm$ 15 &  4.09  &  -2.18 $\pm$ 0.06 &   0 \\
 %    15679 &  265.190820 & -53.638268 &  6243 $\pm$ 10 &  3.94  &  -2.32 $\pm$ 0.04 &   0 \\
 %     7312 &  265.148399 & -53.679637 &  6417 $\pm$ 17 &  4.18  &  -2.38 $\pm$ 0.08 &   0 \\
 %    11934 &  265.148895 & -53.668503 &  6363 $\pm$ 15 &  4.09  &  -2.15 $\pm$ 0.06 &   0 \\
 %     5853 &  265.175110 & -53.676308 &  6412 $\pm$ 25 &  4.17  &  -2.72 $\pm$ 0.13 &   0 \\
 %     6110 &  265.171295 & -53.680965 &  5954 $\pm$ 12 &  3.72  &  -2.26 $\pm$ 0.04 &   0 \\
 %    14323 &  265.171844 & -53.652218 &  5573 $\pm$ 12 &  3.15  &  -2.25 $\pm$ 0.03 &   1 \\
 % 14000389 &  265.196533 & -53.705808 &  6359 $\pm$ 20 &  4.19  &  -2.46 $\pm$ 0.09 &   0 \\
 %     4547 &  265.194897 & -53.674662 &  5971 $\pm$ 20 &  3.77  &   -2.3 $\pm$ 0.06 &   0 \\
 %     5214 &  265.182433 & -53.678490 &  6243 $\pm$ 27 &  3.94  &  -2.32 $\pm$ 0.11 &   0 \\
 %     4213 &  265.202515 & -53.687386 &  6525 $\pm$ 27 &  4.03  &  -2.73 $\pm$ 0.16 &   0 \\
 % 13000099 &  265.182060 & -53.707163 &  6341 $\pm$ 12 &  4.02  &   -2.2 $\pm$ 0.04 &   0 \\
 %     2577 &  265.156311 & -53.691967 &  5504 $\pm$ 11 &  3.09  &  -2.27 $\pm$ 0.02 &   0 \\
 %     3529 &  265.222931 & -53.675701 &  6372 $\pm$ 20 &  4.19  &   -2.49 $\pm$ 0.1 &   0 \\
 %    13420 &  265.197357 & -53.658669 &  6346 $\pm$ 15 &  3.96  &  -2.48 $\pm$ 0.07 &   0 \\
 %    10313 &  265.177094 & -53.673367 &  6360 $\pm$ 23 &  4.18  &  -2.43 $\pm$ 0.11 &   0 \\
 %     3842 &  265.213287 & -53.674812 &  5529 $\pm$ 11 &   3.2  &  -2.19 $\pm$ 0.02 &   0 \\
 %     8532 &  265.214966 & -53.669373 &  6371 $\pm$ 17 &  4.05  &  -2.45 $\pm$ 0.09 &   0 \\
 % 19000159 &  265.099080 & -53.667350 &  6098 $\pm$ 11 &  3.81  &  -2.19 $\pm$ 0.03 &   0 \\
 %     8402 &  265.218648 & -53.666415 &  6377 $\pm$ 20 &  4.09  &  -2.34 $\pm$ 0.09 &   0 \\
 %     4649 &  265.192188 & -53.677902 &  5990 $\pm$ 14 &  3.77  &  -2.26 $\pm$ 0.04 &   0 \\
 %     9088 &  265.199870 & -53.672362 &  6255 $\pm$ 16 &  4.09  &  -2.28 $\pm$ 0.06 &   0 \\
 %     4886 &  265.188049 & -53.678982 &  6412 $\pm$ 17 &  4.14  &  -2.85 $\pm$ 0.09 &   0 \\
 %    12171 &  265.141876 & -53.670399 &  6386 $\pm$ 16 &  4.19  &  -2.39 $\pm$ 0.08 &   0 \\
 %     2887 &  265.145942 & -53.691632 &  6366 $\pm$ 15 &  4.06  &  -2.32 $\pm$ 0.06 &   0 \\
 %    11484 &  265.159119 & -53.661041 &  6397 $\pm$ 22 &  4.06  &  -2.97 $\pm$ 0.11 &   0 \\
 %    12011 &  265.146606 & -53.670616 &   5166 $\pm$ 9 &  2.02  &  -2.21 $\pm$ 0.02 &   0 \\
 %      204 &  265.166748 & -53.702652 &  6408 $\pm$ 15 &  4.04  &  -2.61 $\pm$ 0.08 &   0 \\
 %    12441 &  265.133331 & -53.669807 &  6432 $\pm$ 15 &  4.02  &  -2.55 $\pm$ 0.07 &   0 \\
 %     5627 &  265.177429 & -53.675980 &  6468 $\pm$ 15 &  4.18  &  -2.49 $\pm$ 0.08 &   0 \\
 %     3633 &  265.219543 & -53.675983 &  5606 $\pm$ 12 &  3.34  &  -2.16 $\pm$ 0.03 &   0 \\
 %     6606 &  265.163483 & -53.681686 &  6204 $\pm$ 13 &  3.91  &  -2.41 $\pm$ 0.05 &   0 \\
 %     6622 &  265.163788 & -53.676689 &  6187 $\pm$ 18 &  3.93  &  -2.43 $\pm$ 0.08 &   0 \\
 %     6752 &  265.160858 & -53.686481 &  5612 $\pm$ 12 &  3.26  &  -2.19 $\pm$ 0.03 &   0 \\
 %     6210 &  265.170044 & -53.678066 &  6382 $\pm$ 12 &  4.05  &  -2.53 $\pm$ 0.06 &   0 \\
 %     7444 &  265.144958 & -53.683998 &  5500 $\pm$ 11 &  3.03  &  -2.17 $\pm$ 0.02 &   0 \\
 %    10478 &  265.175598 & -53.669235 &  5640 $\pm$ 12 &  3.44  &   -2.2 $\pm$ 0.03 &   0 \\
 %     7806 &  265.135435 & -53.682370 &  6414 $\pm$ 14 &  4.19  &  -2.25 $\pm$ 0.06 &   0 \\
 %     6295 &  265.168854 & -53.676655 &  6338 $\pm$ 11 &  3.98  &  -2.74 $\pm$ 0.06 &   0 \\
 %     8335 &  265.221052 & -53.667487 &  6379 $\pm$ 16 &  4.06  &  -2.25 $\pm$ 0.07 &   0 \\
 %     2025 &  265.169891 & -53.694489 &  6261 $\pm$ 16 &  3.92  &  -2.66 $\pm$ 0.08 &   0 \\
 %     4871 &  265.188477 & -53.685417 &  5253 $\pm$ 10 &  2.25  &  -2.29 $\pm$ 0.02 &   0 \\
 %     4740 &  265.190552 & -53.682697 &  5779 $\pm$ 14 &  3.57  &  -2.18 $\pm$ 0.03 &   0 \\
 %    10817 &  265.170685 & -53.664383 &  6073 $\pm$ 24 &  4.02  &  -2.13 $\pm$ 0.07 &   0 \\
 %     6949 &  265.157166 & -53.680588 &  5574 $\pm$ 13 &  3.18  &  -2.13 $\pm$ 0.02 &   0 \\
 % 15000092 &  265.196038 & -53.640376 &  5256 $\pm$ 11 &   2.5  &  -2.11 $\pm$ 0.02 &   0 \\
 %    10452 &  265.176056 & -53.661686 &  6435 $\pm$ 35 &  4.08  &   -2 $\pm$ 0.13 &   0 \\
 % 24000163 &  265.179433 & -53.628944 &  6324 $\pm$ 11 &  4.05  &  -2.22 $\pm$ 0.04 &   1 \\
 % 12000071 &  265.168404 & -53.719501 &  6218 $\pm$ 16 &  4.13  &  -2.34 $\pm$ 0.06 &   0 \\
 %     6942 &  265.157471 & -53.686035 &  6504 $\pm$ 17 &  4.19  &  -2.42 $\pm$ 0.09 &   0 \\
 %     8671 &  265.210716 & -53.662482 &  6337 $\pm$ 18 &  4.17  &  -2.28 $\pm$ 0.07 &   0 \\
 %     5385 &  265.180145 & -53.680252 &  5421 $\pm$ 11 &  2.79  &  -2.21 $\pm$ 0.02 &   0 \\
 %     9636 &  265.188324 & -53.668964 &  6045 $\pm$ 13 &  3.75  &  -2.13 $\pm$ 0.04 &   0 \\
 %     4917 &  265.187544 & -53.681068 &  6193 $\pm$ 17 &  3.84  &  -2.23 $\pm$ 0.06 &   0 \\
 %     6460 &  265.165863 & -53.687069 &  6348 $\pm$ 14 &  3.97  &  -2.39 $\pm$ 0.06 &   0 \\
 %     7945 &  265.131500 & -53.676945 &  6433 $\pm$ 16 &  4.19  &  -2.58 $\pm$ 0.09 &   0 \\
 %    11253 &  265.163269 & -53.670921 &  5720 $\pm$ 12 &  3.55  &  -2.28 $\pm$ 0.03 &   0 \\
 %    11250 &  265.163361 & -53.671310 &  6468 $\pm$ 19 &  4.18  &   -2.58 $\pm$ 0.1 &   0 \\
 %     7221 &  265.151062 & -53.687435 &  6203 $\pm$ 13 &  3.91  &  -2.56 $\pm$ 0.06 &   0 \\
 %    15330 &  265.137831 & -53.658055 &  5619 $\pm$ 10 &  3.36  &  -2.05 $\pm$ 0.02 &   1 \\
 %     4685 &  265.191895 & -53.674614 &  6412 $\pm$ 18 &  4.11  &  -2.66 $\pm$ 0.09 &   0 \\
 % 19000142 &  265.108627 & -53.656963 &  6424 $\pm$ 13 &  4.04  &  -2.37 $\pm$ 0.06 &   0 \\
 %     2772 &  265.150459 & -53.691305 &  5686 $\pm$ 12 &  3.54  &  -2.19 $\pm$ 0.03 &   0 \\
 %     3593 &  265.220337 & -53.682880 &  6075 $\pm$ 14 &  3.79  &  -2.41 $\pm$ 0.05 &   0 \\
 %    15359 &  265.135918 & -53.659561 &  6048 $\pm$ 11 &  3.79  &  -2.18 $\pm$ 0.03 &   0 \\
 %     4040 &  265.207733 & -53.680126 &  6098 $\pm$ 13 &  3.81  &  -2.51 $\pm$ 0.05 &   0 \\
 %     4305 &  265.200199 & -53.686759 &  6393 $\pm$ 16 &  4.08  &  -2.27 $\pm$ 0.07 &   0 \\
 %     7155 &  265.152491 & -53.676429 &  5541 $\pm$ 13 &  3.49  &  -2.14 $\pm$ 0.02 &   0 \\
 %     7115 &  265.153412 & -53.683228 &  6310 $\pm$ 13 &  3.96  &  -2.49 $\pm$ 0.06 &   0 \\
 %     4033 &  265.207916 & -53.682972 &  5929 $\pm$ 14 &  3.73  &  -2.46 $\pm$ 0.04 &   0 \\
 %     5645 &  265.176605 & -53.685051 &  5470 $\pm$ 12 &  2.93  &  -2.33 $\pm$ 0.03 &   0 \\
 % 16000098 &  265.164346 & -53.632010 &  6444 $\pm$ 16 &  4.03  &   -2.3 $\pm$ 0.08 &   0 \\
 %     3844 &  265.212738 & -53.687195 &  5480 $\pm$ 11 &  2.95  &  -2.24 $\pm$ 0.02 &   0 \\
 %     4918 &  265.188019 & -53.680889 &  6314 $\pm$ 14 &  4.03  &  -2.69 $\pm$ 0.07 &   0 \\
 %     8476 &  265.216483 & -53.663987 &  6278 $\pm$ 13 &  3.94  &  -2.38 $\pm$ 0.05 &   0 \\
 %    15130 &  265.146698 & -53.658348 &  5241 $\pm$ 13 &  2.34  &  -2.19 $\pm$ 0.02 &   0 \\
 %    15452 &  265.131067 & -53.657403 &  6274 $\pm$ 10 &  3.97  &   -2.3 $\pm$ 0.04 &   0 \\
 %     6948 &  265.157076 & -53.682215 &  5877 $\pm$ 12 &  3.64  &  -2.13 $\pm$ 0.03 &   0 \\
 %    10638 &  265.173248 & -53.672359 &  5516 $\pm$ 10 &  2.77  &  -2.17 $\pm$ 0.02 &   0 \\
 %     1824 &  265.175903 & -53.689728 &   5048 $\pm$ 3 &  1.35  &  -2.03 $\pm$ 0.01 &   0 \\
 %    11313 &  265.162018 & -53.667225 &  5545 $\pm$ 13 &  3.04  &  -2.12 $\pm$ 0.03 &   0 \\
 %     3752 &  265.215576 & -53.681152 &  6413 $\pm$ 14 &  4.06  &  -2.26 $\pm$ 0.06 &   0 \\
 % 13000456 &  265.194562 & -53.710755 &  6294 $\pm$ 15 &   4.2  &  -1.97 $\pm$ 0.04 &   0 \\
 %     1348 &  265.187469 & -53.690804 &  6386 $\pm$ 14 &  4.07  &  -2.79 $\pm$ 0.07 &   0 \\
 %     7597 &  265.141640 & -53.676436 &  5900 $\pm$ 18 &  3.69  &   -2.5 $\pm$ 0.06 &   1 \\
 %     1299 &  265.188782 & -53.696644 &  6369 $\pm$ 14 &  4.01  &  -2.67 $\pm$ 0.07 &   0 \\
 %     1201 &  265.191559 & -53.689850 &  6150 $\pm$ 12 &  3.87  &  -2.29 $\pm$ 0.04 &   0 \\
 %    12941 &  265.114552 & -53.666550 &  6436 $\pm$ 13 &  4.19  &  -2.42 $\pm$ 0.06 &   0 \\
 %     7729 &  265.137526 & -53.681063 &  6250 $\pm$ 12 &  3.96  &  -2.18 $\pm$ 0.04 &   0 \\
 %    11553 &  265.157374 & -53.661269 &  5689 $\pm$ 12 &  3.54  &  -2.14 $\pm$ 0.03 &   0 \\
 %     5214 &  265.182434 & -53.678490 &  6129 $\pm$ 21 &  3.94  &  -2.41 $\pm$ 0.08 &   0 \\
 %     1105 &  265.194519 & -53.689709 &  5654 $\pm$ 14 &  3.45  &  -2.12 $\pm$ 0.03 &   0 \\
 %     1626 &  265.180481 & -53.688190 &  6379 $\pm$ 16 &  4.16  &  -2.25 $\pm$ 0.06 &   0 \\
 %    11480 &  265.158927 & -53.662959 &  6222 $\pm$ 13 &  3.93  &  -2.44 $\pm$ 0.06 &   0 \\
 % 15000003 &  265.209691 & -53.649073 &  5640 $\pm$ 11 &  3.43  &  -2.03 $\pm$ 0.02 &   0 \\
 %    13200 &  265.205294 & -53.659263 &  6292 $\pm$ 16 &  3.96  &  -2.46 $\pm$ 0.07 &   0 \\
 %      742 &  265.209563 & -53.693212 &  6139 $\pm$ 12 &  3.87  &  -2.22 $\pm$ 0.04 &   0 \\
 %     6933 &  265.157623 & -53.676872 &  6424 $\pm$ 16 &  4.15  &   -2.7 $\pm$ 0.08 &   0 \\
 %     8855 &  265.205837 & -53.665401 &  6128 $\pm$ 13 &  3.89  &  -2.13 $\pm$ 0.04 &   0 \\
 %    14699 &  265.161295 & -53.650404 &  6322 $\pm$ 22 &  4.15  &   -2.54 $\pm$ 0.1 &   0 \\
 %    10829 &  265.170449 & -53.661191 &  6408 $\pm$ 15 &  4.08  &  -2.44 $\pm$ 0.08 &   0 \\
 %     8571 &  265.213531 & -53.669235 &  5872 $\pm$ 19 &   3.7  &  -2.36 $\pm$ 0.05 &   0 \\
 %    10445 &  265.175903 & -53.664577 &  5218 $\pm$ 11 &  2.27  &  -2.21 $\pm$ 0.02 &   0 \\
 %     4868 &  265.188294 & -53.686333 &  6344 $\pm$ 19 &  4.18  &  -2.48 $\pm$ 0.09 &   0 \\
 %      813 &  265.205655 & -53.692708 &  6013 $\pm$ 18 &  3.82  &  -2.05 $\pm$ 0.05 &   1 \\
 %     9769 &  265.186089 & -53.669746 &  6402 $\pm$ 20 &   4.1  &   -2.6 $\pm$ 0.11 &   0 \\
 %     5854 &  265.174975 & -53.676371 &  6403 $\pm$ 36 &  4.06  &  -2.73 $\pm$ 0.18 &   0 \\
 %     4947 &  265.187375 & -53.675672 &  6259 $\pm$ 25 &  3.99  &  -2.51 $\pm$ 0.11 &   0 \\
 % 22000171 &  265.248662 & -53.672180 &  6160 $\pm$ 11 &  3.85  &   -2.3 $\pm$ 0.04 &   1 \\
 %     1776 &  265.177200 & -53.687768 &  6370 $\pm$ 19 &  4.17  &  -2.29 $\pm$ 0.08 &   0 \\
 % 15000624 &  265.209155 & -53.638802 &  6347 $\pm$ 16 &  4.15  &  -2.43 $\pm$ 0.07 &   0 \\
 %     6698 &  265.162097 & -53.679176 &   5107 $\pm$ 5 &  1.94  &  -2.13 $\pm$ 0.01 &   0 \\
 % 22000060 &  265.248787 & -53.672602 &  6220 $\pm$ 11 &  3.92  &  -2.26 $\pm$ 0.04 &   0 \\
 % 18000210 &  265.126339 & -53.649891 &  6417 $\pm$ 13 &  4.14  &  -2.32 $\pm$ 0.06 &   0 \\
 %    11392 &  265.161001 & -53.665448 &  6128 $\pm$ 14 &  3.85  &  -2.26 $\pm$ 0.05 &   0 \\
 %     4503 &  265.195412 & -53.681124 &  6162 $\pm$ 13 &   3.8  &  -2.17 $\pm$ 0.04 &   0 \\
 %    11887 &  265.149963 & -53.664322 &  6019 $\pm$ 20 &  3.77  &  -2.49 $\pm$ 0.07 &   0 \\
 %    11887 &  265.149964 & -53.664321 &  6040 $\pm$ 13 &  3.77  &  -2.19 $\pm$ 0.04 &   0 \\
 %     7885 &  265.133282 & -53.686441 &  6399 $\pm$ 12 &  4.16  &   -2.4 $\pm$ 0.05 &   0 \\
 %    14917 &  265.154621 & -53.650098 &  6423 $\pm$ 12 &  4.08  &  -2.23 $\pm$ 0.05 &   0 \\
 %     3252 &  265.233700 & -53.683827 &  6384 $\pm$ 16 &  4.16  &  -2.26 $\pm$ 0.07 &   0 \\
 %    15359 &  265.135925 & -53.659561 &  6110 $\pm$ 19 &  3.79  &  -2.39 $\pm$ 0.07 &   0 \\
 % 13000392 &  265.189285 & -53.715244 &  6398 $\pm$ 14 &  4.09  &  -2.39 $\pm$ 0.07 &   0 \\
 %     4860 &  265.188660 & -53.674694 &  5552 $\pm$ 11 &  3.06  &  -2.13 $\pm$ 0.02 &   0 \\
 % 16000525 &  265.152823 & -53.634134 &  6377 $\pm$ 21 &  3.99  &   -2.54 $\pm$ 0.1 &   0 \\
 % 15000319 &  265.201134 & -53.635640 &  6401 $\pm$ 12 &  4.15  &  -2.25 $\pm$ 0.05 &   0 \\
 % 22000099 &  265.224602 & -53.666099 &  6246 $\pm$ 14 &  3.57  &   -2.2 $\pm$ 0.05 &   0 \\
 % 16000164 &  265.161968 & -53.640610 &  6405 $\pm$ 11 &  4.02  &  -2.21 $\pm$ 0.05 &   0 \\
 %     9663 &  265.187653 & -53.668842 &  5390 $\pm$ 11 &   2.7  &  -2.22 $\pm$ 0.02 &   0 \\
 %     4527 &  265.195007 & -53.684174 &  5698 $\pm$ 14 &  3.51  &  -2.32 $\pm$ 0.03 &   0 \\
 % 20000246 &  265.104455 & -53.681175 &  6395 $\pm$ 13 &  4.08  &  -2.31 $\pm$ 0.06 &   0 \\
 %     7427 &  265.145264 & -53.682121 &  6399 $\pm$ 17 &  4.19  &  -2.32 $\pm$ 0.07 &   0 \\
 %     9149 &  265.198997 & -53.670389 &  6284 $\pm$ 14 &  4.06  &  -2.39 $\pm$ 0.06 &   0 \\
 %     3003 &  265.141296 & -53.689243 &   5092 $\pm$ 5 &  1.81  &   -2.1 $\pm$ 0.01 &   0 \\
 %    12268 &  265.138977 & -53.666992 &  6495 $\pm$ 17 &  4.12  &  -2.64 $\pm$ 0.08 &   0 \\
 %    10742 &  265.171387 & -53.673599 &  6260 $\pm$ 16 &  3.99  &  -2.74 $\pm$ 0.07 &   0 \\
 %     5882 &  265.174262 & -53.681493 &  5842 $\pm$ 14 &  3.64  &  -2.03 $\pm$ 0.03 &   0 \\
 %     6638 &  265.163083 & -53.683799 &  6307 $\pm$ 14 &  4.09  &  -2.13 $\pm$ 0.05 &   0 \\
 %    14589 &  265.164518 & -53.653340 &  6287 $\pm$ 14 &  3.93  &  -2.24 $\pm$ 0.05 &   0 \\
 %     7133 &  265.152479 & -53.685322 &  6076 $\pm$ 14 &  3.82  &  -2.35 $\pm$ 0.05 &   0 \\
 %     5136 &  265.183868 & -53.678543 &  5594 $\pm$ 12 &  3.33  &  -2.12 $\pm$ 0.02 &   0 \\
 %     7558 &  265.141815 & -53.683517 &  6313 $\pm$ 14 &  4.13  &  -2.23 $\pm$ 0.06 &   1 \\
 %     4525 &  265.194733 & -53.685242 &  6216 $\pm$ 15 &   3.9  &  -2.39 $\pm$ 0.06 &   0 \\
 %     1237 &  265.190665 & -53.690884 &  6404 $\pm$ 16 &  4.09  &  -2.47 $\pm$ 0.07 &   0 \\
 %     4593 &  265.193512 & -53.679569 &  6303 $\pm$ 13 &  3.97  &  -2.76 $\pm$ 0.07 &   0 \\
 %     7092 &  265.153870 & -53.683815 &  5559 $\pm$ 12 &  3.17  &  -2.22 $\pm$ 0.03 &   0 \\
 % 23000060 &  265.230672 & -53.661259 &  5516 $\pm$ 11 &  3.25  &  -2.06 $\pm$ 0.02 &   0 \\
 %    10593 &  265.173889 & -53.670017 &  6456 $\pm$ 13 &  4.16  &  -2.65 $\pm$ 0.07 &   0 \\
 %     4760 &  265.190430 & -53.674252 &  5155 $\pm$ 12 &  2.04  &  -2.14 $\pm$ 0.02 &   0 \\
 %     5188 &  265.182702 & -53.685309 &  6437 $\pm$ 18 &  4.14  &  -2.42 $\pm$ 0.09 &   0 \\
 %    15700 &  265.189310 & -53.640135 &  6429 $\pm$ 22 &  4.06  &  -2.13 $\pm$ 0.09 &   0 \\
 %     7250 &  265.150055 & -53.678036 &  6418 $\pm$ 14 &  4.08  &  -2.74 $\pm$ 0.08 &   0 \\
 %     5387 &  265.180328 & -53.679045 &  6290 $\pm$ 16 &  4.08  &  -2.22 $\pm$ 0.06 &   0 \\
 %     5437 &  265.179474 & -53.677334 &  5756 $\pm$ 18 &  3.46  &  -2.17 $\pm$ 0.04 &   0 \\
 %    13275 &  265.202882 & -53.648764 &  6280 $\pm$ 11 &  4.04  &  -2.14 $\pm$ 0.04 &   0 \\
 %     5016 &  265.185555 & -53.684874 &  6133 $\pm$ 13 &  3.82  &  -2.23 $\pm$ 0.04 &   0 \\
 %     4503 &  265.195404 & -53.681126 &  6127 $\pm$ 13 &   3.8  &   -2.5 $\pm$ 0.05 &   0 \\
 % 24000204 &  265.206413 & -53.632771 &  5959 $\pm$ 11 &  3.78  &  -2.25 $\pm$ 0.03 &   0 \\
 %    10415 &  265.175964 & -53.672146 &  5668 $\pm$ 19 &  3.26  &  -2.06 $\pm$ 0.04 &   0 \\
 %     5651 &  265.176815 & -53.682589 &  5423 $\pm$ 10 &  3.04  &  -2.22 $\pm$ 0.02 &   0 \\
 %    10734 &  265.171692 & -53.663116 &  5873 $\pm$ 21 &  4.13  &  -1.77 $\pm$ 0.04 &   0 \\
 %    11645 &  265.154948 & -53.672991 &  5753 $\pm$ 13 &  3.59  &  -2.13 $\pm$ 0.03 &   0 \\
 %     1776 &  265.177185 & -53.687767 &  6335 $\pm$ 17 &  4.17  &  -2.45 $\pm$ 0.07 &   0 \\
 % 12000110 &  265.163334 & -53.712289 &   5507 $\pm$ 9 &  3.08  &  -2.02 $\pm$ 0.02 &   0 \\
 %     5694 &  265.176575 & -53.674728 &  6496 $\pm$ 28 &  4.16  &   -2.5 $\pm$ 0.15 &   0 \\
 %     8904 &  265.203979 & -53.672169 &  5542 $\pm$ 11 &  3.16  &   -2.2 $\pm$ 0.02 &   0 \\
 %    11264 &  265.163086 & -53.661160 &  6242 $\pm$ 20 &  3.91  &  -2.41 $\pm$ 0.08 &   0 \\
 %     5233 &  265.182171 & -53.674218 &  6287 $\pm$ 21 &  4.16  &   -2.1 $\pm$ 0.07 &   0 \\
 %     1552 &  265.182343 & -53.690693 &  6346 $\pm$ 15 &  4.16  &  -2.68 $\pm$ 0.08 &   0 \\
 %    11758 &  265.152893 & -53.666744 &  5170 $\pm$ 11 &  2.13  &   -2.2 $\pm$ 0.02 &   0 \\
 %     5848 &  265.175049 & -53.677467 &  6383 $\pm$ 13 &  4.05  &  -2.54 $\pm$ 0.06 &   0 \\
 %      727 &  265.210846 & -53.687946 &  6166 $\pm$ 13 &  3.84  &  -2.45 $\pm$ 0.05 &   0 \\
 %     7133 &  265.152466 & -53.685322 &  6142 $\pm$ 13 &  3.82  &  -2.48 $\pm$ 0.05 &   0 \\
 % 21000098 &  265.262501 & -53.684574 &  6408 $\pm$ 12 &  4.17  &  -2.35 $\pm$ 0.05 &   0 \\
 %    15700 &  265.189310 & -53.640135 &  6433 $\pm$ 24 &  4.06  &   -2.12 $\pm$ 0.1 &   0 \\
 %     9229 &  265.197325 & -53.663482 &   5036 $\pm$ 3 &  1.29  &  -1.89 $\pm$ 0.01 &   0 \\
 %     2568 &  265.156250 & -53.698799 &  6462 $\pm$ 14 &  4.06  &  -2.61 $\pm$ 0.08 &   0 \\
 %      376 &  265.158173 & -53.703709 &  6313 $\pm$ 14 &  3.95  &  -2.58 $\pm$ 0.07 &   0 \\
 %    12457 &  265.132660 & -53.666351 &  6469 $\pm$ 16 &  4.17  &   -2.9 $\pm$ 0.08 &   0 \\
 %     7522 &  265.143372 & -53.680595 &  6420 $\pm$ 14 &  4.13  &   -2.3 $\pm$ 0.06 &   0 \\
 % 16000085 &  265.164276 & -53.633916 &  6401 $\pm$ 11 &   4  &  -2.34 $\pm$ 0.05 &   1 \\
 %    12330 &  265.137329 & -53.662270 &   5468 $\pm$ 9 &  2.71  &  -2.19 $\pm$ 0.02 &   0 \\
 %    14464 &  265.167532 & -53.652156 &  6290 $\pm$ 21 &  4.13  &  -2.17 $\pm$ 0.07 &   0 \\
 %     6466 &  265.166313 & -53.685444 &  6913 $\pm$ 24 &  4.17  &  -2.24 $\pm$ 0.12 &   0 \\
 %     4886 &  265.188038 & -53.678982 &  6414 $\pm$ 22 &  4.14  &   -2.41 $\pm$ 0.1 &   0 \\
 %     1602 &  265.181152 & -53.690845 &  5865 $\pm$ 14 &  3.66  &  -2.11 $\pm$ 0.03 &   0 \\
 %     5235 &  265.181924 & -53.686777 &  5946 $\pm$ 13 &  3.76  &  -2.06 $\pm$ 0.03 &   0 \\
 %     8764 &  265.208510 & -53.669359 &  6292 $\pm$ 17 &  4.05  &  -2.37 $\pm$ 0.07 &   0 \\
 %     8904 &  265.203989 & -53.672169 &  5513 $\pm$ 10 &  3.16  &  -2.08 $\pm$ 0.02 &   0 \\
 %    11631 &  265.155731 & -53.664921 &  5998 $\pm$ 18 &  3.75  &  -2.48 $\pm$ 0.06 &   0 \\
 %    14667 &  265.161896 & -53.657009 &  5250 $\pm$ 12 &  2.27  &  -2.27 $\pm$ 0.02 &   0 \\
 % 24000034 &  265.200638 & -53.622814 &  6362 $\pm$ 12 &  4.17  &  -2.35 $\pm$ 0.05 &   0 \\
 %     6174 &  265.170441 & -53.675945 &  6296 $\pm$ 10 &  4.01  &  -2.48 $\pm$ 0.05 &   1 \\
 %    14942 &  265.152954 & -53.658352 &  6428 $\pm$ 21 &  3.98  &  -2.55 $\pm$ 0.11 &   0 \\
 %     3648 &  265.219086 & -53.679459 &  6392 $\pm$ 17 &   4.1  &  -2.45 $\pm$ 0.08 &   0 \\
 %     3650 &  265.218964 & -53.678642 &  6381 $\pm$ 18 &  4.09  &  -2.82 $\pm$ 0.09 &   0 \\
 %    11835 &  265.151611 & -53.671761 &  6469 $\pm$ 15 &  4.13  &  -2.65 $\pm$ 0.08 &   0 \\
 %     3669 &  265.218384 & -53.679573 &  6437 $\pm$ 17 &  4.14  &  -2.78 $\pm$ 0.09 &   0 \\
 %     8553 &  265.214339 & -53.668133 &  6276 $\pm$ 21 &  3.86  &  -2.19 $\pm$ 0.08 &   0 \\
 % 24000035 &  265.196431 & -53.621968 &  6418 $\pm$ 12 &  4.17  &  -2.28 $\pm$ 0.05 &   0 \\
 %     2772 &  265.150452 & -53.691303 &  5822 $\pm$ 40 &  3.54  &  -1.96 $\pm$ 0.08 &   0 \\
 % 14000072 &  265.215094 & -53.699558 &  6146 $\pm$ 12 &  3.82  &  -2.24 $\pm$ 0.04 &   0 \\
 % 24000074 &  265.182654 & -53.631390 &  5768 $\pm$ 12 &   3.6  &   -2.1 $\pm$ 0.03 &   1 \\
 %     9459 &  265.191864 & -53.670437 &  6339 $\pm$ 14 &  3.98  &   -2.5 $\pm$ 0.06 &   0 \\
 %     7558 &  265.141819 & -53.683518 &  6318 $\pm$ 16 &  4.13  &  -2.11 $\pm$ 0.06 &   1 \\
 %     5385 &  265.180139 & -53.680252 &   5377 $\pm$ 9 &  2.79  &  -2.16 $\pm$ 0.02 &   0 \\
 %     1261 &  265.190094 & -53.691071 &  6400 $\pm$ 18 &  4.19  &  -2.41 $\pm$ 0.08 &   1 \\
 %     5872 &  265.174042 & -53.686821 &  6496 $\pm$ 15 &  4.18  &  -2.17 $\pm$ 0.07 &   0 \\
 %     7326 &  265.147661 & -53.685907 &  6459 $\pm$ 15 &  4.11  &  -2.11 $\pm$ 0.06 &   0 \\
 %     7079 &  265.154236 & -53.676991 &  6382 $\pm$ 14 &  4.11  &  -2.51 $\pm$ 0.07 &   0 \\
 %     8592 &  265.212648 & -53.666871 &  6191 $\pm$ 15 &  3.97  &  -2.26 $\pm$ 0.05 &   0 \\
 %     7806 &  265.135437 & -53.682369 &  6405 $\pm$ 22 &  4.19  &   -2.38 $\pm$ 0.1 &   0 \\
 %     8677 &  265.209930 & -53.672134 &  6203 $\pm$ 24 &  3.98  &  -2.52 $\pm$ 0.09 &   0 \\
 %     6048 &  265.172577 & -53.674446 &  5588 $\pm$ 19 &  3.48  &  -2.34 $\pm$ 0.04 &   0 \\
 %    13975 &  265.180634 & -53.659817 &  6343 $\pm$ 15 &   4.1  &  -2.28 $\pm$ 0.06 &   0 \\
 %     8774 &  265.208462 & -53.662146 &  6356 $\pm$ 19 &  4.15  &  -2.36 $\pm$ 0.08 &   0 \\
 %     9272 &  265.195910 & -53.668190 &  5594 $\pm$ 11 &  3.32  &  -2.12 $\pm$ 0.02 &   0 \\
 %     6749 &  265.161530 & -53.674294 &  5860 $\pm$ 15 &  3.69  &  -2.33 $\pm$ 0.04 &   0 \\
 %     1447 &  265.185150 & -53.690697 &  6428 $\pm$ 15 &  4.19  &  -2.56 $\pm$ 0.07 &   0 \\
 %     2887 &  265.145942 & -53.691632 &  6442 $\pm$ 16 &  4.06  &  -2.37 $\pm$ 0.08 &   0 \\
 %    10475 &  265.175629 & -53.670525 &  6404 $\pm$ 18 &  4.17  &  -2.85 $\pm$ 0.09 &   0 \\
 %     7117 &  265.153412 & -53.681854 &  5163 $\pm$ 10 &  2.09  &  -2.19 $\pm$ 0.02 &   0 \\
 %     1846 &  265.175568 & -53.688515 &  6198 $\pm$ 14 &  3.94  &  -2.35 $\pm$ 0.05 &   0 \\
 %    15832 &  265.182991 & -53.639145 &  6279 $\pm$ 19 &   4  &  -2.02 $\pm$ 0.06 &   0 \\
 %     9001 &  265.201691 & -53.670300 &  6349 $\pm$ 14 &  4.09  &  -2.45 $\pm$ 0.06 &   0 \\
 % 18000213 &  265.115752 & -53.648888 &  6394 $\pm$ 13 &  4.18  &  -2.44 $\pm$ 0.06 &   0 \\
 %     4668 &  265.191711 & -53.679771 &  6439 $\pm$ 16 &  4.07  &  -2.54 $\pm$ 0.08 &   0 \\
 %     6201 &  265.169952 & -53.680412 &  6485 $\pm$ 12 &  4.15  &  -2.65 $\pm$ 0.06 &   0 \\
 %      160 &  265.168976 & -53.704178 &  6494 $\pm$ 19 &  4.11  &   -2.92 $\pm$ 0.1 &   0 \\
 %     5637 &  265.177342 & -53.674664 &  6456 $\pm$ 25 &  4.08  &  -2.53 $\pm$ 0.13 &   0 \\
 %     5148 &  265.183655 & -53.674080 &  6169 $\pm$ 12 &  3.85  &  -2.42 $\pm$ 0.05 &   0 \\
 %    15861 &  265.180664 & -53.645386 &  5462 $\pm$ 11 &  2.98  &  -2.18 $\pm$ 0.02 &   0 \\
 % 15000140 &  265.209770 & -53.652177 &  5436 $\pm$ 13 &  2.83  &  -2.14 $\pm$ 0.02 &   0 \\
 %     3577 &  265.221039 & -53.684647 &  5901 $\pm$ 14 &  3.66  &  -2.28 $\pm$ 0.04 &   0 \\
 %    13228 &  265.204814 & -53.653103 &  5946 $\pm$ 29 &  3.82  &   -2 $\pm$ 0.07 &   1 \\
 %    11804 &  265.152022 & -53.673068 &  5594 $\pm$ 13 &  3.49  &  -2.08 $\pm$ 0.02 &   0 \\
 %     5414 &  265.179657 & -53.685543 &   5150 $\pm$ 9 &  2.07  &  -2.22 $\pm$ 0.02 &   0 \\
 %     8093 &  265.125488 & -53.673969 &  5810 $\pm$ 29 &  3.64  &  -2.23 $\pm$ 0.07 &   0 \\
 %     8310 &  265.221649 & -53.673115 &  6503 $\pm$ 21 &  4.19  &   -3  &   0 \\
 %     9159 &  265.199036 & -53.662590 &   5070 $\pm$ 4 &  1.55  &  -2.08 $\pm$ 0.01 &   0 \\
 %     7806 &  265.135435 & -53.682370 &  6350 $\pm$ 20 &  4.19  &   -3  &   0 \\
 %     4731 &  265.190709 & -53.686973 &  6231 $\pm$ 13 &  3.93  &  -2.51 $\pm$ 0.06 &   0 \\
 %    11059 &  265.166840 & -53.671803 &  6421 $\pm$ 13 &  4.03  &  -2.39 $\pm$ 0.06 &   0 \\
 % 13000150 &  265.185832 & -53.707391 &  6410 $\pm$ 14 &  4.06  &  -2.14 $\pm$ 0.05 &   0 \\
 %     7547 &  265.142609 & -53.676849 &  5502 $\pm$ 20 &  3.29  &  -2.23 $\pm$ 0.04 &   0 \\
 %    12617 &  265.126495 & -53.673447 &  6202 $\pm$ 15 &  3.96  &  -2.52 $\pm$ 0.06 &   0 \\
 %     3696 &  265.217712 & -53.675362 &  6287 $\pm$ 14 &  3.95  &  -2.77 $\pm$ 0.07 &   0 \\
 %     4030 &  265.207855 & -53.685963 &   5149 $\pm$ 8 &  1.76  &  -2.29 $\pm$ 0.02 &   0 \\
 %     5353 &  265.180497 & -53.678521 &  6331 $\pm$ 17 &  4.19  &  -2.45 $\pm$ 0.08 &   0 \\
 %     5696 &  265.176880 & -53.674389 &  6369 $\pm$ 17 &  4.02  &  -2.12 $\pm$ 0.06 &   0 \\
 %    11682 &  265.154358 & -53.671890 &  5467 $\pm$ 12 &  2.99  &  -2.24 $\pm$ 0.02 &   0 \\
 %    12617 &  265.126507 & -53.673447 &  6250 $\pm$ 13 &  3.96  &  -2.38 $\pm$ 0.05 &   0 \\
 % 14000101 &  265.207936 & -53.709055 &  6453 $\pm$ 17 &  4.11  &  -2.61 $\pm$ 0.09 &   0 \\
 %     6430 &  265.166443 & -53.682907 &  6471 $\pm$ 15 &  4.17  &  -2.28 $\pm$ 0.07 &   0 \\
 %     5811 &  265.175659 & -53.674599 &  5578 $\pm$ 85 &  4.13  &  -1.85 $\pm$ 0.13 &   0 \\
 %    12692 &  265.124599 & -53.662088 &  6382 $\pm$ 12 &  4.15  &  -2.55 $\pm$ 0.06 &   0 \\
 %    12364 &  265.136017 & -53.662071 &  6295 $\pm$ 13 &  3.92  &  -2.67 $\pm$ 0.06 &   0 \\
 %     9913 &  265.183502 & -53.662167 &  6497 $\pm$ 18 &  4.18  &   -2.83 $\pm$ 0.1 &   0 \\
 %    11174 &  265.165161 & -53.663345 &  5614 $\pm$ 16 &  3.34  &  -2.23 $\pm$ 0.04 &   0 \\
 %     3003 &  265.141296 & -53.689243 &   5078 $\pm$ 5 &  1.81  &  -2.13 $\pm$ 0.02 &   0 \\
 %    14955 &  265.152527 & -53.658707 &  6500 $\pm$ 25 &  4.19  &  -1.92 $\pm$ 0.08 &   0 \\
 %    11480 &  265.158936 & -53.662960 &  6282 $\pm$ 19 &  3.93  &  -2.43 $\pm$ 0.09 &   0 \\
 %     9594 &  265.189107 & -53.672558 &  6315 $\pm$ 25 &  4.05  &  -2.54 $\pm$ 0.11 &   0 \\
 %     2209 &  265.165466 & -53.696266 &  5864 $\pm$ 14 &  3.68  &  -2.31 $\pm$ 0.04 &   0 \\
 %     6106 &  265.171539 & -53.682434 &  5661 $\pm$ 12 &   3.4  &  -2.32 $\pm$ 0.03 &   0 \\
 %     4760 &  265.190429 & -53.674252 &   5138 $\pm$ 7 &  2.04  &  -2.15 $\pm$ 0.01 &   0 \\
 %     9385 &  265.193664 & -53.669792 &   5344 $\pm$ 8 &  2.63  &  -2.27 $\pm$ 0.01 &   0 \\
 %    11514 &  265.157990 & -53.673103 &  6330 $\pm$ 17 &  4.17  &  -2.54 $\pm$ 0.08 &   0 \\
 %    14280 &  265.173035 & -53.647682 &  5506 $\pm$ 11 &   3.1  &  -2.14 $\pm$ 0.02 &   0 \\
 %    10196 &  265.178772 & -53.672180 &  6365 $\pm$ 14 &  4.15  &  -2.75 $\pm$ 0.07 &   0 \\
 %     5603 &  265.177036 & -53.685938 &  6367 $\pm$ 15 &  4.07  &   -2.3 $\pm$ 0.06 &   0 \\
 %    11922 &  265.149738 & -53.660301 &  6302 $\pm$ 14 &  4.03  &  -2.59 $\pm$ 0.07 &   0 \\
 %     7656 &  265.139862 & -53.677479 &  6381 $\pm$ 14 &   4  &   -2.5 $\pm$ 0.07 &   0 \\
 %     6343 &  265.167603 & -53.683117 &  5489 $\pm$ 11 &  3.14  &  -2.22 $\pm$ 0.02 &   0 \\
 %     4157 &  265.204315 & -53.681290 &  6424 $\pm$ 16 &  4.07  &  -2.77 $\pm$ 0.09 &   0 \\
 %    13897 &  265.183075 & -53.650597 &  6405 $\pm$ 15 &  4.13  &  -2.52 $\pm$ 0.08 &   0 \\
 %     6758 &  265.161036 & -53.682844 &  6160 $\pm$ 14 &  4.02  &  -2.21 $\pm$ 0.05 &   0 \\
 %     2418 &  265.160004 & -53.693348 &  5802 $\pm$ 13 &  3.59  &   -2.2 $\pm$ 0.03 &   0 \\
 %     9313 &  265.195179 & -53.660651 &  6414 $\pm$ 17 &  4.15  &  -2.29 $\pm$ 0.07 &   0 \\
 %    11127 &  265.165192 & -53.673302 &  6403 $\pm$ 16 &  4.18  &   -2.6 $\pm$ 0.08 &   0 \\
 %     6727 &  265.161250 & -53.681218 &  6263 $\pm$ 14 &  3.96  &  -2.31 $\pm$ 0.05 &   0 \\
 %     9871 &  265.184357 & -53.665966 &  6409 $\pm$ 17 &  4.19  &  -2.35 $\pm$ 0.08 &   0 \\
 %     7773 &  265.136505 & -53.675388 &   5092 $\pm$ 4 &  1.75  &   -2.2 $\pm$ 0.01 &   0 \\
 %     1830 &  265.175262 & -53.699490 &  5536 $\pm$ 11 &  3.14  &  -2.15 $\pm$ 0.02 &   0 \\
 %    13071 &  265.108096 & -53.663425 &  6469 $\pm$ 12 &  4.18  &  -2.45 $\pm$ 0.06 &   0 \\
 %      868 &  265.203583 & -53.687782 &   5069 $\pm$ 4 &  1.61  &  -2.09 $\pm$ 0.01 &   0 \\
 %     6727 &  265.161255 & -53.681217 &  6284 $\pm$ 12 &  3.96  &  -2.47 $\pm$ 0.05 &   0 \\
 %     7212 &  265.151672 & -53.678459 &  5722 $\pm$ 13 &  3.56  &  -2.25 $\pm$ 0.03 &   0 \\
 %     5783 &  265.175590 & -53.682886 &  6355 $\pm$ 18 &  4.13  &  -2.12 $\pm$ 0.07 &   0 \\
 %     6808 &  265.159973 & -53.676121 &  6203 $\pm$ 14 &  3.99  &  -2.29 $\pm$ 0.05 &   0 \\
 %    10153 &  265.179565 & -53.671848 &  6443 $\pm$ 15 &  4.03  &  -2.48 $\pm$ 0.07 &   0 \\
 %     6872 &  265.158875 & -53.676601 &  5634 $\pm$ 13 &  3.39  &  -2.23 $\pm$ 0.03 &   0 \\
 %    14726 &  265.160688 & -53.646169 &  5989 $\pm$ 12 &  3.75  &  -2.28 $\pm$ 0.03 &   0 \\
 %    11085 &  265.166785 & -53.661702 &  5624 $\pm$ 12 &  3.43  &  -2.26 $\pm$ 0.03 &   0 \\
 %     5016 &  265.185547 & -53.684875 &  6133 $\pm$ 12 &  3.82  &  -2.38 $\pm$ 0.05 &   0 \\
 % 23000287 &  265.225025 & -53.657512 &   5122 $\pm$ 7 &  1.93  &  -2.11 $\pm$ 0.01 &   0 \\
 %     1626 &  265.180496 & -53.688189 &  6271 $\pm$ 18 &  4.16  &  -2.18 $\pm$ 0.06 &   0 \\
 %     1828 &  265.175323 & -53.700596 &  6220 $\pm$ 13 &  3.85  &  -2.62 $\pm$ 0.06 &   0 \\
 %     7653 &  265.139595 & -53.678882 &   5203 $\pm$ 8 &  2.35  &  -2.09 $\pm$ 0.01 &   0 \\
 %     7682 &  265.138763 & -53.685332 &  6398 $\pm$ 11 &  4.06  &  -2.47 $\pm$ 0.05 &   0 \\
 %     2443 &  265.159546 & -53.688152 &  6255 $\pm$ 13 &  3.94  &  -2.66 $\pm$ 0.06 &   0 \\
 %     9636 &  265.188324 & -53.668964 &  6039 $\pm$ 13 &  3.75  &  -2.31 $\pm$ 0.04 &   0 \\
 %     6002 &  265.173065 & -53.674000 &  5490 $\pm$ 11 &  2.98  &  -2.25 $\pm$ 0.02 &   0 \\
 %     1542 &  265.182698 & -53.694765 &  6151 $\pm$ 13 &  3.82  &  -2.33 $\pm$ 0.05 &   0 \\
 % 12000104 &  265.143574 & -53.714040 &  6273 $\pm$ 12 &  3.92  &  -2.35 $\pm$ 0.05 &   0 \\
 % 12000201 &  265.142074 & -53.713401 &  5708 $\pm$ 15 &   3.5  &  -2.08 $\pm$ 0.03 &   0 \\
 %    11615 &  265.155427 & -53.672950 &  5903 $\pm$ 15 &  3.71  &  -2.29 $\pm$ 0.04 &   0 \\
 % 18000136 &  265.134105 & -53.652706 &   5425 $\pm$ 9 &  2.88  &  -2.08 $\pm$ 0.02 &   0 \\
 %     5848 &  265.175059 & -53.677467 &  6330 $\pm$ 17 &  4.05  &  -2.39 $\pm$ 0.08 &   0 \\
 % 11000133 &  265.113285 & -53.690057 &  6305 $\pm$ 14 &  4.08  &  -2.28 $\pm$ 0.05 &   0 \\
 %     9313 &  265.195190 & -53.660652 &  6379 $\pm$ 15 &  4.15  &  -2.69 $\pm$ 0.08 &   0 \\
 % 14000325 &  265.212764 & -53.708033 &  5306 $\pm$ 26 &  2.97  &  -2.11 $\pm$ 0.04 &   0 \\
 %    14479 &  265.167380 & -53.658167 &  6365 $\pm$ 17 &  4.05  &  -1.97 $\pm$ 0.06 &   0 \\
 %     5783 &  265.175598 & -53.682884 &  6335 $\pm$ 13 &  4.13  &  -2.39 $\pm$ 0.06 &   0 \\
 %     5687 &  265.176819 & -53.675320 &  6532 $\pm$ 17 &  4.19  &  -2.52 $\pm$ 0.09 &   0 \\
 %     5914 &  265.174408 & -53.674953 &  6408 $\pm$ 16 &  4.15  &   -2.3 $\pm$ 0.07 &   0 \\
 %     7519 &  265.143447 & -53.682959 &  6391 $\pm$ 18 &   4.1  &  -2.38 $\pm$ 0.08 &   0 \\
 % 17000261 &  265.146127 & -53.640482 &  6355 $\pm$ 11 &  4.12  &  -2.33 $\pm$ 0.05 &   0 \\
 %    11578 &  265.156372 & -53.664536 &  6171 $\pm$ 20 &  3.89  &  -2.31 $\pm$ 0.07 &   0 \\
 % 23000068 &  265.231292 & -53.660342 &  6350 $\pm$ 13 &  4.16  &  -2.14 $\pm$ 0.05 &   0 \\
 %     1620 &  265.180786 & -53.692657 &  6406 $\pm$ 14 &  4.02  &  -2.49 $\pm$ 0.07 &   0 \\
 %     1447 &  265.185162 & -53.690697 &  6326 $\pm$ 19 &  4.19  &  -2.56 $\pm$ 0.08 &   0 \\
 %     8562 &  265.213831 & -53.662367 &  5753 $\pm$ 11 &  3.56  &  -2.09 $\pm$ 0.02 &   0 \\
 %    11189 &  265.164459 & -53.672012 &  5795 $\pm$ 12 &   3.6  &   -2.3 $\pm$ 0.03 &   0 \\
 %     6677 &  265.162231 & -53.680164 &  6382 $\pm$ 14 &  4.13  &  -2.55 $\pm$ 0.07 &   0 \\
 %    15280 &  265.140316 & -53.657349 &  6381 $\pm$ 12 &  4.12  &  -2.52 $\pm$ 0.06 &   0 \\
 %    10047 &  265.181488 & -53.670273 &  6121 $\pm$ 13 &  3.83  &  -2.44 $\pm$ 0.05 &   0 \\
 %    14798 &  265.157867 & -53.652046 &  6654 $\pm$ 24 &  4.13  &  -2.35 $\pm$ 0.13 &   0 \\
 %    10903 &  265.169497 & -53.666780 &   5351 $\pm$ 9 &  2.68  &  -2.08 $\pm$ 0.01 &   0 \\
 % 12000066 &  265.163137 & -53.720221 &  6426 $\pm$ 13 &  4.14  &  -2.34 $\pm$ 0.06 &   0 \\
 %    11759 &  265.153206 & -53.666210 &  6301 $\pm$ 14 &  3.99  &  -2.52 $\pm$ 0.06 &   0 \\
 % 23000360 &  265.228222 & -53.646959 &  5704 $\pm$ 49 &  3.43  &  -1.48 $\pm$ 0.07 &   0 \\
 %     5136 &  265.183860 & -53.678543 &  5589 $\pm$ 11 &  3.33  &  -2.14 $\pm$ 0.02 &   0 \\
 %     5693 &  265.176605 & -53.674515 &  6369 $\pm$ 18 &  4.03  &  -2.58 $\pm$ 0.09 &   0 \\
 %     6546 &  265.165100 & -53.680508 &  6354 $\pm$ 14 &  4.14  &  -2.59 $\pm$ 0.07 &   0 \\
 %    15892 &  265.178284 & -53.645935 &  6409 $\pm$ 27 &  4.07  &   -2.16 $\pm$ 0.1 &   0 \\
 %     1299 &  265.188770 & -53.696642 &  6251 $\pm$ 17 &  4.01  &  -2.33 $\pm$ 0.06 &   0 \\
 %     5648 &  265.176788 & -53.683189 &  5496 $\pm$ 12 &  2.97  &  -2.25 $\pm$ 0.02 &   0 \\
 %    11514 &  265.157990 & -53.673103 &  6344 $\pm$ 17 &  4.17  &  -2.69 $\pm$ 0.09 &   0 \\
 % 13000055 &  265.167467 & -53.710464 &  6354 $\pm$ 12 &  4.04  &  -2.55 $\pm$ 0.06 &   0 \\
 %     9188 &  265.197648 & -53.666774 &  6446 $\pm$ 16 &  4.18  &  -2.07 $\pm$ 0.06 &   0 \\
 %    10764 &  265.171295 & -53.668694 &  6455 $\pm$ 14 &  4.13  &  -2.87 $\pm$ 0.07 &   0 \\
 %     4700 &  265.191244 & -53.683919 &  6456 $\pm$ 19 &  4.19  &   -2.53 $\pm$ 0.1 &   0 \\
 %    10966 &  265.168213 & -53.669121 &  6376 $\pm$ 15 &  4.17  &  -2.48 $\pm$ 0.07 &   0 \\
 %      706 &  265.211168 & -53.693711 &  6543 $\pm$ 16 &  4.17  &  -2.32 $\pm$ 0.08 &   0 \\
 %     5562 &  265.178031 & -53.680340 &  5863 $\pm$ 15 &  3.62  &  -2.17 $\pm$ 0.04 &   0 \\
 %    13113 &  265.212865 & -53.659674 &  5542 $\pm$ 11 &  3.21  &  -2.04 $\pm$ 0.02 &   0 \\
 %     3887 &  265.211517 & -53.684158 &  6397 $\pm$ 17 &  4.16  &  -2.94 $\pm$ 0.09 &   0 \\
 % 24000102 &  265.189406 & -53.628418 &  5822 $\pm$ 11 &  3.71  &  -2.15 $\pm$ 0.03 &   0 \\
 % 20000142 &  265.106481 & -53.674969 &  6386 $\pm$ 14 &  4.17  &  -2.34 $\pm$ 0.06 &   0 \\
 %     4967 &  265.186371 & -53.679169 &  6171 $\pm$ 13 &  3.85  &  -2.44 $\pm$ 0.05 &   0 \\
 %     5934 &  265.173737 & -53.678432 &  5626 $\pm$ 12 &  3.41  &  -2.17 $\pm$ 0.03 &   0 \\
 %     5894 &  265.174532 & -53.678031 &  6291 $\pm$ 16 &  4.17  &  -2.18 $\pm$ 0.06 &   0 \\
 %     4758 &  265.190499 & -53.674478 &  5747 $\pm$ 22 &   3.6  &  -2.24 $\pm$ 0.05 &   0 \\
 % 16000170 &  265.164599 & -53.639161 &  6368 $\pm$ 15 &  3.97  &  -2.25 $\pm$ 0.06 &   0 \\
 %     5002 &  265.186005 & -53.676846 &  6552 $\pm$ 20 &   4.2  &  -2.65 $\pm$ 0.11 &   0 \\
 %    10348 &  265.176910 & -53.661034 &  6224 $\pm$ 14 &  3.99  &  -2.49 $\pm$ 0.06 &   0 \\
 % 23000102 &  265.214955 & -53.655367 &  5882 $\pm$ 11 &  3.65  &  -2.08 $\pm$ 0.02 &   0 \\
 %     3352 &  265.230152 & -53.677457 &  6361 $\pm$ 12 &  4.05  &  -2.35 $\pm$ 0.05 &   0 \\
 %     5018 &  265.185487 & -53.682857 &  5836 $\pm$ 13 &  3.61  &  -2.13 $\pm$ 0.03 &   0 \\
 %     7067 &  265.154144 & -53.684746 &  6302 $\pm$ 12 &  3.97  &  -2.72 $\pm$ 0.06 &   0 \\
 %      845 &  265.204076 & -53.694903 &  6386 $\pm$ 14 &  4.15  &  -2.43 $\pm$ 0.06 &   0 \\
 %    15194 &  265.144257 & -53.659607 &  5584 $\pm$ 17 &  3.26  &  -2.24 $\pm$ 0.04 &   0 \\
 %    11361 &  265.161163 & -53.662884 &  5782 $\pm$ 20 &  3.55  &   -2.2 $\pm$ 0.05 &   0 \\
 %     5414 &  265.179672 & -53.685542 &   5137 $\pm$ 7 &  2.07  &  -2.16 $\pm$ 0.01 &   0 \\
 % 15000015 &  265.207431 & -53.641613 &  6346 $\pm$ 13 &  4.07  &  -2.42 $\pm$ 0.06 &   1 \\
 %     4316 &  265.200226 & -53.680672 &   5147 $\pm$ 8 &  2.03  &  -2.17 $\pm$ 0.02 &   0 \\
 %     1520 &  265.182824 & -53.689607 &  6341 $\pm$ 21 &  4.15  &  -2.24 $\pm$ 0.08 &   0 \\
 %    10925 &  265.169128 & -53.671364 &  5897 $\pm$ 17 &  3.69  &  -2.16 $\pm$ 0.04 &   0 \\
 %    10737 &  265.171661 & -53.660423 &  5617 $\pm$ 15 &  3.32  &  -2.13 $\pm$ 0.03 &   0 \\
 %     9880 &  265.183929 & -53.663269 &  5469 $\pm$ 11 &  2.91  &  -2.16 $\pm$ 0.02 &   0 \\
 % 14000393 &  265.217547 & -53.700649 &   5363 $\pm$ 9 &  2.76  &  -2.11 $\pm$ 0.02 &   0 \\
 %    11151 &  265.164673 & -53.673550 &  5624 $\pm$ 12 &  3.41  &  -2.22 $\pm$ 0.03 &   0 \\
 %    11745 &  265.153200 & -53.673069 &  6146 $\pm$ 14 &  3.94  &  -2.15 $\pm$ 0.04 &   0 \\
 %     9414 &  265.193115 & -53.667793 &  5320 $\pm$ 11 &  2.52  &  -2.17 $\pm$ 0.02 &   0 \\
 % 13000113 &  265.181954 & -53.716464 &  5443 $\pm$ 12 &  2.91  &  -2.13 $\pm$ 0.02 &   0 \\
 %    12409 &  265.134766 & -53.663342 &  6341 $\pm$ 14 &  4.02  &  -2.45 $\pm$ 0.06 &   0 \\
 %    13452 &  265.196694 & -53.647500 &  5552 $\pm$ 11 &  3.17  &   -2.1 $\pm$ 0.02 &   0 \\
 %     5783 &  265.175590 & -53.682886 &  6374 $\pm$ 20 &  4.13  &  -2.39 $\pm$ 0.09 &   0 \\
 %    11919 &  265.149658 & -53.662358 &   5456 $\pm$ 8 &  2.95  &   -2.1 $\pm$ 0.01 &   0 \\
 % 18000121 &  265.122706 & -53.654953 &  5823 $\pm$ 11 &  3.63  &  -2.21 $\pm$ 0.03 &   0 \\
 %     3267 &  265.233156 & -53.684427 &  6308 $\pm$ 25 &  4.11  &  -2.21 $\pm$ 0.09 &   0 \\
 %     6478 &  265.166138 & -53.680286 &  5674 $\pm$ 13 &  3.48  &  -2.16 $\pm$ 0.03 &   0 \\
 %     2887 &  265.145935 & -53.691631 &  6339 $\pm$ 13 &  4.06  &  -2.48 $\pm$ 0.06 &   0 \\
 %     8855 &  265.205841 & -53.665401 &  6196 $\pm$ 14 &  3.89  &  -2.42 $\pm$ 0.06 &   0 \\
 % 14000114 &  265.212516 & -53.699679 &  5801 $\pm$ 12 &  3.64  &  -2.22 $\pm$ 0.03 &   1 \\
 %    11361 &  265.161155 & -53.662882 &  5716 $\pm$ 14 &  3.55  &  -2.25 $\pm$ 0.03 &   0 \\
 %    15194 &  265.144257 & -53.659607 &  5548 $\pm$ 15 &  3.26  &  -2.24 $\pm$ 0.03 &   0 \\
 %     6546 &  265.165098 & -53.680507 &  6316 $\pm$ 20 &  4.14  &  -2.31 $\pm$ 0.08 &   0 \\
 % 22000004 &  265.237963 & -53.676140 &  5240 $\pm$ 10 &   2.4  &  -2.15 $\pm$ 0.01 &   0 \\
 %     1220 &  265.191406 & -53.690350 &  6319 $\pm$ 13 &  4.05  &   -2.5 $\pm$ 0.06 &   0 \\
 %     4305 &  265.200195 & -53.686760 &  6379 $\pm$ 15 &  4.08  &  -2.51 $\pm$ 0.07 &   0 \\
 %    14762 &  265.158997 & -53.656525 &  6539 $\pm$ 32 &  4.19  &  -2.51 $\pm$ 0.18 &   0 \\
 %     3003 &  265.141296 & -53.689243 &  5104 $\pm$ 33 &  1.81  &  -2.21 $\pm$ 0.09 &   8 \\
 % 22000170 &  265.233247 & -53.672536 &  6275 $\pm$ 11 &   3.9  &  -2.23 $\pm$ 0.04 &   1 \\
 %     5054 &  265.185150 & -53.675152 &  5486 $\pm$ 11 &  2.97  &  -2.17 $\pm$ 0.02 &   0 \\
 %    11384 &  265.160706 & -53.669060 &  6327 $\pm$ 24 &  4.07  &  -2.53 $\pm$ 0.12 &   0 \\
 % 19000244 &  265.100968 & -53.662155 &  6427 $\pm$ 12 &   4.1  &  -2.26 $\pm$ 0.05 &   0 \\
 %    10308 &  265.177826 & -53.659927 &  6314 $\pm$ 17 &  4.14  &  -2.41 $\pm$ 0.07 &   0 \\
 %     5353 &  265.180511 & -53.678520 &  6384 $\pm$ 14 &  4.19  &  -2.52 $\pm$ 0.07 &   0 \\
 % 21000155 &  265.242583 & -53.687856 &  6399 $\pm$ 14 &   4.1  &  -2.31 $\pm$ 0.06 &   1 \\
 %     6126 &  265.171539 & -53.676720 &  6428 $\pm$ 14 &  4.13  &  -2.31 $\pm$ 0.06 &   0 \\
 %     2872 &  265.146667 & -53.689835 &  6375 $\pm$ 16 &  4.06  &  -2.71 $\pm$ 0.08 &   0 \\
 %     4896 &  265.188110 & -53.676949 &  6325 $\pm$ 12 &  3.95  &  -2.68 $\pm$ 0.06 &   0 \\
 %     4055 &  265.207062 & -53.677555 &  6392 $\pm$ 14 &  4.06  &  -2.64 $\pm$ 0.07 &   0 \\
 %    10817 &  265.170680 & -53.664383 &  6247 $\pm$ 14 &  4.02  &  -2.16 $\pm$ 0.05 &   0 \\
 %     4648 &  265.192620 & -53.678527 &  6308 $\pm$ 21 &  4.05  &   -2.55 $\pm$ 0.1 &   0 \\
 %     6430 &  265.166450 & -53.682908 &  6428 $\pm$ 19 &  4.17  &  -2.15 $\pm$ 0.08 &   0 \\
 %    10425 &  265.176239 & -53.671051 &  6022 $\pm$ 14 &  3.76  &  -2.26 $\pm$ 0.04 &   0 \\
 %     2553 &  265.156494 & -53.692963 &  6757 $\pm$ 16 &   4  &  -2.32 $\pm$ 0.08 &   1 \\
 % 15000102 &  265.204025 & -53.638992 &  6394 $\pm$ 13 &  4.12  &  -2.24 $\pm$ 0.05 &   0 \\
 %     1120 &  265.194470 & -53.691684 &  6338 $\pm$ 17 &  4.09  &  -2.44 $\pm$ 0.07 &   0 \\
 %     6139 &  265.170471 & -53.686638 &  5442 $\pm$ 16 &  2.72  &   -2.2 $\pm$ 0.03 &   0 \\
 %     6948 &  265.157074 & -53.682213 &  5847 $\pm$ 13 &  3.64  &  -2.29 $\pm$ 0.04 &   0 \\
 %    14667 &  265.161880 & -53.657008 &   5201 $\pm$ 8 &  2.27  &  -2.13 $\pm$ 0.01 &   0 \\
 %     6509 &  265.165283 & -53.680187 &  5988 $\pm$ 16 &  3.74  &  -2.41 $\pm$ 0.05 &   0 \\
 %     4747 &  265.190735 & -53.680973 &  6111 $\pm$ 12 &   3.8  &  -2.43 $\pm$ 0.05 &   0 \\
 %     7437 &  265.145050 & -53.687302 &  5475 $\pm$ 11 &   3  &  -2.26 $\pm$ 0.02 &   0 \\
 %     7644 &  265.139825 & -53.682989 &  6372 $\pm$ 16 &  4.13  &  -2.21 $\pm$ 0.07 &   0 \\
 %    10172 &  265.179260 & -53.668476 &  6468 $\pm$ 13 &  4.07  &  -2.45 $\pm$ 0.07 &   0 \\
 %     3300 &  265.231865 & -53.681414 &  5373 $\pm$ 10 &  2.74  &  -2.08 $\pm$ 0.02 &   1 \\
 %    10714 &  265.171661 & -53.670345 &  5373 $\pm$ 11 &  2.58  &  -2.22 $\pm$ 0.02 &   0 \\
 %     9267 &  265.195744 & -53.670481 &  5801 $\pm$ 12 &   3.6  &  -2.12 $\pm$ 0.03 &   0 \\
 %     4885 &  265.188299 & -53.679142 &  6433 $\pm$ 18 &  4.05  &  -2.25 $\pm$ 0.07 &   0 \\
 %    16011 &  265.168299 & -53.645333 &  6358 $\pm$ 12 &  4.11  &  -2.32 $\pm$ 0.06 &   0 \\
 %    14860 &  265.155994 & -53.650554 &  6351 $\pm$ 12 &  4.08  &  -2.39 $\pm$ 0.05 &   0 \\
 % 15000061 &  265.217097 & -53.644767 &   5368 $\pm$ 9 &  2.72  &  -2.09 $\pm$ 0.02 &   0 \\
 %     4971 &  265.186650 & -53.676440 &  6189 $\pm$ 14 &  3.88  &  -2.15 $\pm$ 0.05 &   0 \\
 %    10090 &  265.180542 & -53.666668 &  6143 $\pm$ 15 &  3.82  &  -2.43 $\pm$ 0.06 &   0 \\
 %     5110 &  265.184404 & -53.675556 &  5597 $\pm$ 13 &  3.39  &   -2.1 $\pm$ 0.03 &   0 \\
 %    10502 &  265.175537 & -53.662743 &  6375 $\pm$ 20 &  3.88  &  -2.59 $\pm$ 0.11 &   0 \\
 %     1213 &  265.191473 & -53.695849 &  6086 $\pm$ 28 &  3.88  &  -2.09 $\pm$ 0.08 &   0 \\
 %     6536 &  265.164992 & -53.682312 &  6398 $\pm$ 19 &  4.01  &   -2.1 $\pm$ 0.07 &   0 \\
 %      930 &  265.200934 & -53.695801 &  6283 $\pm$ 19 &  4.16  &  -2.28 $\pm$ 0.07 &   0 \\
 %     8447 &  265.217068 & -53.665411 &  6381 $\pm$ 14 &  4.19  &  -2.71 $\pm$ 0.07 &   0 \\
 %     9050 &  265.200481 & -53.671457 &  4785 $\pm$ 16 &  1.08  &  -2.03 $\pm$ 0.02 &   0 \\
 %    13827 &  265.184723 & -53.649769 &  6008 $\pm$ 12 &  3.77  &  -2.43 $\pm$ 0.04 &   0 \\
 %     3257 &  265.233191 & -53.678920 &  5390 $\pm$ 11 &  2.77  &   -2.2 $\pm$ 0.02 &   0 \\
 % 12000199 &  265.143301 & -53.713435 &  5869 $\pm$ 11 &  3.65  &  -2.08 $\pm$ 0.03 &   0 \\
 %     2035 &  265.170013 & -53.688454 &  6358 $\pm$ 14 &  4.03  &  -2.58 $\pm$ 0.07 &   1 \\
 %    11553 &  265.157379 & -53.661270 &  5646 $\pm$ 18 &  3.54  &  -2.26 $\pm$ 0.04 &   0 \\
 %     8817 &  265.207031 & -53.665207 &  6126 $\pm$ 13 &  3.86  &  -2.52 $\pm$ 0.05 &   0 \\
 %    15761 &  265.186461 & -53.639336 &  5780 $\pm$ 13 &  3.59  &  -2.17 $\pm$ 0.03 &   0 \\
 %    12971 &  265.113492 & -53.666747 &  6322 $\pm$ 12 &  4.03  &  -2.38 $\pm$ 0.05 &   0 \\
 %     4746 &  265.190521 & -53.681263 &  6318 $\pm$ 27 &  4.16  &   -3  &   0 \\
 %     7994 &  265.129782 & -53.681862 &   5358 $\pm$ 9 &  2.73  &  -2.15 $\pm$ 0.01 &   0 \\
 %     5901 &  265.173981 & -53.676811 &  6351 $\pm$ 13 &  4.11  &  -2.63 $\pm$ 0.06 &   0 \\
 %      796 &  265.206879 & -53.690479 &  6348 $\pm$ 15 &  4.03  &  -2.69 $\pm$ 0.08 &   0 \\
 %    11911 &  265.149811 & -53.667088 &  6451 $\pm$ 22 &  4.19  &  -2.49 $\pm$ 0.11 &   0 \\
 %    10663 &  265.172577 & -53.673168 &  6108 $\pm$ 16 &  3.81  &  -2.45 $\pm$ 0.06 &   0 \\
 %     6949 &  265.157153 & -53.680588 &  5499 $\pm$ 12 &  3.18  &  -2.11 $\pm$ 0.02 &   0 \\
 %     6994 &  265.156144 & -53.683284 &  6447 $\pm$ 17 &  4.16  &  -2.33 $\pm$ 0.07 &   0 \\
 %     9198 &  265.197754 & -53.660686 &  6359 $\pm$ 17 &  4.07  &  -2.59 $\pm$ 0.09 &   0 \\
 %    14464 &  265.167542 & -53.652157 &  6429 $\pm$ 26 &  4.13  &  -2.34 $\pm$ 0.13 &   0 \\
 %     6872 &  265.158883 & -53.676600 &  5629 $\pm$ 11 &  3.39  &  -2.16 $\pm$ 0.02 &   0 \\
 % 16000070 &  265.174558 & -53.636676 &  6368 $\pm$ 11 &  4.06  &  -2.22 $\pm$ 0.05 &   0 \\
 %      747 &  265.209503 & -53.689465 &  6214 $\pm$ 13 &   3.9  &  -2.42 $\pm$ 0.05 &   0 \\
 %     7312 &  265.148407 & -53.679638 &  6479 $\pm$ 16 &  4.18  &  -2.47 $\pm$ 0.08 &   0 \\
 %      918 &  265.201101 & -53.690126 &  5898 $\pm$ 14 &  3.72  &   -2.2 $\pm$ 0.04 &   0 \\
 %    10326 &  265.177063 & -53.670273 &  6519 $\pm$ 13 &  4.16  &  -2.52 $\pm$ 0.07 &   0 \\
 %     3643 &  265.218597 & -53.682400 &  5551 $\pm$ 12 &  3.24  &   -2.1 $\pm$ 0.02 &   0 \\
 %     5648 &  265.176796 & -53.683190 &  5454 $\pm$ 10 &  2.97  &  -2.12 $\pm$ 0.02 &   0 \\
 %     9920 &  265.183746 & -53.660198 &  6354 $\pm$ 16 &  4.07  &  -2.42 $\pm$ 0.07 &   0 \\
 %    14699 &  265.161285 & -53.650406 &  6494 $\pm$ 31 &  4.15  &   -2.6 $\pm$ 0.19 &   0 \\
 % 22000300 &  265.238879 & -53.677084 &  5917 $\pm$ 11 &   3.7  &  -2.23 $\pm$ 0.03 &   0 \\
 % 12000310 &  265.150738 & -53.710449 &  6419 $\pm$ 21 &  4.16  &  -1.93 $\pm$ 0.07 &   0 \\
 %     1662 &  265.179504 & -53.691994 &  5768 $\pm$ 14 &  3.62  &  -2.47 $\pm$ 0.04 &   0 \\
 %     4967 &  265.186366 & -53.679169 &  6074 $\pm$ 17 &  3.85  &  -2.44 $\pm$ 0.06 &   0 \\
 %     5054 &  265.185156 & -53.675153 &  5439 $\pm$ 10 &  2.97  &  -2.04 $\pm$ 0.02 &   0 \\
 %    11173 &  265.164795 & -53.664001 &  5955 $\pm$ 22 &  3.73  &  -2.36 $\pm$ 0.07 &   0 \\
 % 15000104 &  265.209703 & -53.638638 &  6007 $\pm$ 10 &  3.77  &  -2.24 $\pm$ 0.03 &   0 \\
 %     4524 &  265.194774 & -53.685609 &  6404 $\pm$ 15 &  4.04  &  -2.28 $\pm$ 0.06 &   0 \\
 % 19000149 &  265.096737 & -53.655224 &   5145 $\pm$ 8 &  2.08  &  -2.09 $\pm$ 0.01 &   0 \\
 % 14000103 &  265.198567 & -53.707440 &  5460 $\pm$ 10 &   3  &   -2.1 $\pm$ 0.02 &   1 \\
 %     9291 &  265.195127 & -53.671155 &  6109 $\pm$ 19 &  3.84  &   -2.4 $\pm$ 0.07 &   0 \\
 % 12000100 &  265.163019 & -53.715112 &  5320 $\pm$ 10 &  2.58  &   -2.1 $\pm$ 0.02 &   0 \\
 %    10897 &  265.169434 & -53.669418 &  6513 $\pm$ 22 &  4.18  &  -2.76 $\pm$ 0.12 &   0 \\
 %     7326 &  265.147675 & -53.685905 &  6372 $\pm$ 15 &  4.11  &  -2.63 $\pm$ 0.08 &   0 \\
 %     4886 &  265.188049 & -53.678982 &  6382 $\pm$ 17 &  4.14  &  -2.54 $\pm$ 0.09 &   0 \\
 %     1628 &  265.180145 & -53.699974 &  6374 $\pm$ 20 &  4.17  &   -2.86 $\pm$ 0.1 &   0 \\
 % 11000217 &  265.124255 & -53.685754 &  6397 $\pm$ 11 &  4.07  &  -2.24 $\pm$ 0.05 &   0 \\
 %      796 &  265.206879 & -53.690481 &  6236 $\pm$ 26 &  4.03  &  -2.88 $\pm$ 0.12 &   0 \\
 %     7310 &  265.148407 & -53.681149 &  5577 $\pm$ 12 &  3.32  &  -2.23 $\pm$ 0.03 &   0 \\
 %     5580 &  265.177979 & -53.676403 &  5461 $\pm$ 11 &   3  &  -2.25 $\pm$ 0.02 &   0 \\
 %     5792 &  265.175598 & -53.680157 &  6430 $\pm$ 14 &  4.08  &   -2.4 $\pm$ 0.07 &   0 \\
 %    12209 &  265.140869 & -53.671249 &  6412 $\pm$ 17 &  4.18  &  -2.07 $\pm$ 0.07 &   0 \\
 %     9022 &  265.201111 & -53.671013 &  6115 $\pm$ 12 &  3.98  &  -1.93 $\pm$ 0.03 &   0 \\
 %     4944 &  265.186958 & -53.677928 &  6419 $\pm$ 16 &  4.07  &   -2.8 $\pm$ 0.08 &   0 \\
 %    10796 &  265.170563 & -53.672157 &  6391 $\pm$ 13 &  4.15  &  -2.65 $\pm$ 0.07 &   0 \\
 %    10126 &  265.180206 & -53.668213 &  6176 $\pm$ 32 &  3.89  &  -2.51 $\pm$ 0.13 &   0 \\
 %     8532 &  265.214968 & -53.669373 &  6370 $\pm$ 22 &  4.05  &   -2.31 $\pm$ 0.1 &   0 \\
 % 18000058 &  265.133393 & -53.650686 &   5509 $\pm$ 9 &  3.04  &  -2.08 $\pm$ 0.02 &   0 \\
 % 19000055 &  265.094993 & -53.669514 &  5597 $\pm$ 10 &  3.26  &  -2.17 $\pm$ 0.02 &   0 \\
 %    10608 &  265.173584 & -53.665668 &  5403 $\pm$ 11 &   2.7  &  -2.24 $\pm$ 0.02 &   0 \\
 % 15000097 &  265.193993 & -53.639818 &  5505 $\pm$ 11 &  3.26  &  -2.11 $\pm$ 0.02 &   0 \\
 %     1119 &  265.194391 & -53.692094 &   5400 $\pm$ 9 &  2.83  &  -2.13 $\pm$ 0.01 &   0 \\
 % 13000122 &  265.188172 & -53.713722 &  6447 $\pm$ 12 &  4.09  &  -2.62 $\pm$ 0.06 &   0 \\
 % 16000090 &  265.174130 & -53.633404 &  5950 $\pm$ 10 &  3.68  &  -2.21 $\pm$ 0.03 &   0 \\
 %     6693 &  265.162028 & -53.681977 &  6214 $\pm$ 17 &  4.15  &  -2.07 $\pm$ 0.05 &   0 \\
 %     1176 &  265.192300 & -53.690091 &   5142 $\pm$ 7 &  2.09  &  -2.15 $\pm$ 0.01 &   0 \\
 %     4967 &  265.186366 & -53.679169 &  6017 $\pm$ 18 &  3.85  &  -2.39 $\pm$ 0.06 &   0 \\
 % 24000197 &  265.201012 & -53.633753 &  5982 $\pm$ 11 &  3.75  &  -2.13 $\pm$ 0.03 &   0 \\
 %     2872 &  265.146665 & -53.689833 &  6359 $\pm$ 15 &  4.06  &  -2.45 $\pm$ 0.07 &   0 \\
 %     1264 &  265.190183 & -53.690490 &  6423 $\pm$ 17 &  4.14  &  -2.39 $\pm$ 0.08 &   0 \\
 %     2124 &  265.168030 & -53.690353 &  6279 $\pm$ 14 &  3.96  &  -2.45 $\pm$ 0.06 &   0 \\
 %     8634 &  265.211546 & -53.667426 &  6210 $\pm$ 13 &  3.94  &  -2.39 $\pm$ 0.05 &   0 \\
 %    11419 &  265.160197 & -53.665183 &  6053 $\pm$ 13 &  3.79  &  -2.25 $\pm$ 0.04 &   0 \\
 %    11230 &  265.163956 & -53.667604 &   5390 $\pm$ 9 &  2.75  &  -2.13 $\pm$ 0.02 &   0 \\
 %     9769 &  265.186096 & -53.669746 &  6464 $\pm$ 14 &   4.1  &  -2.59 $\pm$ 0.07 &   0 \\
 % 15000064 &  265.224300 & -53.644599 &  6290 $\pm$ 13 &  4.01  &  -2.43 $\pm$ 0.05 &   0 \\
 %    10584 &  265.173676 & -53.673710 &  6353 $\pm$ 16 &  4.12  &  -2.65 $\pm$ 0.08 &   0 \\
 % 15000319 &  265.201134 & -53.635640 &  6229 $\pm$ 42 &  4.15  &  -2.21 $\pm$ 0.14 &   0 \\
 %     9604 &  265.188690 & -53.667870 &  5611 $\pm$ 12 &  3.42  &   -2.2 $\pm$ 0.03 &   0 \\
 %     7816 &  265.135712 & -53.676826 &  5864 $\pm$ 12 &  3.65  &  -2.23 $\pm$ 0.03 &   0 \\
 % 23000056 &  265.228026 & -53.661609 &   5488 $\pm$ 9 &   3  &  -2.07 $\pm$ 0.02 &   0 \\
 %    13751 &  265.186951 & -53.651955 &  6372 $\pm$ 17 &  4.18  &  -2.48 $\pm$ 0.08 &   0 \\
 %     5758 &  265.175745 & -53.676296 &  6388 $\pm$ 17 &  4.03  &  -2.85 $\pm$ 0.09 &   0 \\
 %     5648 &  265.176796 & -53.683190 &  5436 $\pm$ 12 &  2.97  &  -2.03 $\pm$ 0.02 &   0 \\
 % 13000047 &  265.187732 & -53.711968 &  6349 $\pm$ 12 &  3.96  &  -2.32 $\pm$ 0.05 &   0 \\
 %    10447 &  265.175933 & -53.664280 &  6325 $\pm$ 25 &  3.95  &   -2.24 $\pm$ 0.1 &   0 \\
 %      975 &  265.198914 & -53.692123 &  5546 $\pm$ 12 &   3.2  &   -2.2 $\pm$ 0.02 &   0 \\
 %    11627 &  265.155346 & -53.667296 &  6437 $\pm$ 15 &  4.11  &  -2.59 $\pm$ 0.08 &   0 \\
 %     4885 &  265.188293 & -53.679142 &  6417 $\pm$ 16 &  4.05  &  -2.53 $\pm$ 0.08 &   0 \\
 %     7653 &  265.139587 & -53.678883 &  5275 $\pm$ 12 &  2.35  &  -2.15 $\pm$ 0.02 &   0 \\
 %    11140 &  265.165183 & -53.665771 &  6231 $\pm$ 13 &  3.91  &  -2.57 $\pm$ 0.06 &   0 \\
 %    14429 &  265.168290 & -53.655037 &  6475 $\pm$ 11 &  3.79  &  -2.11 $\pm$ 0.04 &   0 \\
 %     5651 &  265.176819 & -53.682590 &  5489 $\pm$ 10 &  3.04  &  -2.28 $\pm$ 0.02 &   1 \\
 %     4896 &  265.188125 & -53.676949 &  6290 $\pm$ 15 &  3.95  &  -2.24 $\pm$ 0.06 &   0 \\
 % 11000201 &  265.114885 & -53.687294 &  6339 $\pm$ 13 &  4.16  &  -2.45 $\pm$ 0.06 &   0 \\
 %     1439 &  265.185242 & -53.694637 &  6287 $\pm$ 13 &  3.97  &  -2.49 $\pm$ 0.06 &   0 \\
 %     1205 &  265.191956 & -53.687775 &  5793 $\pm$ 14 &  3.62  &  -2.13 $\pm$ 0.03 &   0 \\
 %     4202 &  265.202972 & -53.679337 &  6378 $\pm$ 16 &  4.18  &  -2.33 $\pm$ 0.07 &   0 \\
 %    12232 &  265.140198 & -53.670540 &  5264 $\pm$ 10 &  2.28  &  -2.21 $\pm$ 0.02 &   0 \\
 %    11185 &  265.164520 & -53.673107 &  6229 $\pm$ 13 &  3.94  &   -2.4 $\pm$ 0.05 &   1 \\
 %     6808 &  265.159961 & -53.676121 &  6298 $\pm$ 13 &  3.99  &   -2.2 $\pm$ 0.05 &   0 \\
 %     7250 &  265.150053 & -53.678037 &  6307 $\pm$ 16 &  4.08  &  -2.31 $\pm$ 0.06 &   0 \\
 %    12619 &  265.126648 & -53.670902 &  5476 $\pm$ 11 &  2.93  &  -2.15 $\pm$ 0.02 &   0 \\
 % 15000079 &  265.212352 & -53.642677 &  6352 $\pm$ 11 &  4.02  &  -2.29 $\pm$ 0.04 &   0 \\
 %     4874 &  265.188263 & -53.683132 &  6377 $\pm$ 17 &  4.19  &  -2.95 $\pm$ 0.09 &   0 \\
 %     2024 &  265.170166 & -53.694378 &  6248 $\pm$ 17 &  3.98  &  -2.48 $\pm$ 0.07 &   0 \\
 %     1520 &  265.182831 & -53.689606 &  6383 $\pm$ 17 &  4.15  &  -2.65 $\pm$ 0.08 &   0 \\
 %     4760 &  265.190430 & -53.674252 &   5150 $\pm$ 9 &  2.04  &   -2.2 $\pm$ 0.02 &   0 \\
 % 19000135 &  265.087021 & -53.658230 &  6355 $\pm$ 13 &  4.12  &  -2.28 $\pm$ 0.05 &   0 \\
 %    12020 &  265.146790 & -53.661911 &   5105 $\pm$ 6 &  1.66  &  -2.18 $\pm$ 0.01 &   0 \\
 %     6757 &  265.160797 & -53.683338 &  5375 $\pm$ 10 &  2.58  &  -2.19 $\pm$ 0.02 &   0 \\
 %     2311 &  265.163391 & -53.694386 &  5689 $\pm$ 13 &  3.51  &  -2.17 $\pm$ 0.03 &   0 \\
 %    15990 &  265.170868 & -53.643384 &  6427 $\pm$ 12 &  4.14  &  -2.29 $\pm$ 0.05 &   0 \\
 % 17000172 &  265.146994 & -53.637589 &  5600 $\pm$ 17 &  3.23  &  -2.15 $\pm$ 0.03 &   0 \\
 % 19000066 &  265.101404 & -53.666882 &  6440 $\pm$ 12 &  4.14  &  -2.29 $\pm$ 0.05 &   0 \\
 %     3803 &  265.214203 & -53.687233 &  6466 $\pm$ 24 &  4.15  &  -2.22 $\pm$ 0.11 &   0 \\
 %     8135 &  265.123373 & -53.676979 &  6405 $\pm$ 18 &  4.05  &  -2.22 $\pm$ 0.07 &   1 \\
 %     5201 &  265.182465 & -53.681622 &  5948 $\pm$ 15 &  3.75  &  -2.42 $\pm$ 0.05 &   1 \\
 %     5095 &  265.184204 & -53.681934 &  5784 $\pm$ 13 &  3.58  &  -2.37 $\pm$ 0.04 &   0 \\
 %     5032 &  265.185333 & -53.679729 &  5943 $\pm$ 28 &  3.84  &  -2.49 $\pm$ 0.08 &   0 \\
 %     5188 &  265.182709 & -53.685310 &  6554 $\pm$ 15 &  4.14  &  -2.86 $\pm$ 0.08 &   0 \\
 %      802 &  265.206343 & -53.692537 &  6451 $\pm$ 14 &  4.17  &  -2.43 $\pm$ 0.07 &   0 \\
 %    11547 &  265.157318 & -53.665916 &   5050 $\pm$ 4 &  1.46  &  -1.92 $\pm$ 0.01 &   0 \\
 %     6466 &  265.166321 & -53.685444 &  6466 $\pm$ 18 &  4.17  &  -2.72 $\pm$ 0.11 &   0 \\
 %     2223 &  265.165253 & -53.689110 &  6341 $\pm$ 15 &  4.08  &  -2.75 $\pm$ 0.08 &   0 \\
 %     7427 &  265.145273 & -53.682122 &  6449 $\pm$ 16 &  4.19  &  -1.84 $\pm$ 0.05 &   0 \\
 %    15194 &  265.144259 & -53.659607 &  5542 $\pm$ 12 &  3.26  &  -2.14 $\pm$ 0.02 &   0 \\
 %     9542 &  265.189819 & -53.668709 &  5787 $\pm$ 28 &  3.87  &  -2.16 $\pm$ 0.06 &   0 \\
 %     2474 &  265.158173 & -53.697002 &  6458 $\pm$ 19 &  4.18  &   -2.65 $\pm$ 0.1 &   0 \\
 % 22000322 &  265.242225 & -53.664347 &  6407 $\pm$ 14 &   4.1  &  -2.51 $\pm$ 0.07 &   0 \\
 % 20000043 &  265.107962 & -53.683647 &  6410 $\pm$ 14 &  4.16  &  -2.28 $\pm$ 0.06 &   0 \\
 %    11391 &  265.160651 & -53.666261 &  5578 $\pm$ 11 &  3.26  &  -2.04 $\pm$ 0.02 &   0 \\
 %     7289 &  265.149191 & -53.678189 &  6446 $\pm$ 15 &  4.17  &  -2.31 $\pm$ 0.07 &   0 \\
 %     8228 &  265.228736 & -53.670628 &  6341 $\pm$ 10 &  4.01  &  -2.28 $\pm$ 0.04 &   0 \\
 %     9594 &  265.189117 & -53.672558 &  6333 $\pm$ 17 &  4.05  &   -2.5 $\pm$ 0.08 &   0 \\
 %     9280 &  265.195740 & -53.665638 &   5133 $\pm$ 9 &  2.03  &  -2.26 $\pm$ 0.02 &   0 \\
 %     5702 &  265.176422 & -53.673763 &  6055 $\pm$ 25 &  3.82  &   -2.1 $\pm$ 0.07 &   0 \\
 % 16000290 &  265.152430 & -53.634225 &  5950 $\pm$ 21 &  3.73  &  -2.18 $\pm$ 0.06 &   0 \\
 %    15407 &  265.133814 & -53.654333 &  6394 $\pm$ 14 &  4.18  &   -2.3 $\pm$ 0.06 &   1 \\
 %     5994 &  265.172974 & -53.675014 &  6366 $\pm$ 12 &  4.08  &  -2.69 $\pm$ 0.06 &   1 \\
 %     7608 &  265.141023 & -53.683695 &   5295 $\pm$ 9 &   2.6  &  -2.12 $\pm$ 0.01 &   0 \\
 %     5748 &  265.175910 & -53.676901 &  6323 $\pm$ 18 &   4.2  &  -2.29 $\pm$ 0.07 &   1 \\
 %     8622 &  265.212142 & -53.662021 &  5963 $\pm$ 10 &  3.72  &   -2.2 $\pm$ 0.03 &   0 \\
 % 17000235 &  265.140721 & -53.645459 &  6264 $\pm$ 11 &   4  &  -2.22 $\pm$ 0.04 &   0 \\
 %    15610 &  265.195143 & -53.645002 &  6473 $\pm$ 14 &   4.2  &  -2.35 $\pm$ 0.06 &   0 \\
 %     4700 &  265.191254 & -53.683918 &  6432 $\pm$ 17 &  4.19  &  -2.24 $\pm$ 0.07 &   0 \\
 %     4352 &  265.199463 & -53.675117 &  5371 $\pm$ 21 &  2.58  &  -2.15 $\pm$ 0.04 &   0 \\
 %    11804 &  265.152008 & -53.673069 &  5692 $\pm$ 13 &  3.49  &  -2.11 $\pm$ 0.03 &   0 \\
 %     6676 &  265.162628 & -53.680515 &  6229 $\pm$ 15 &  3.89  &  -2.39 $\pm$ 0.06 &   0 \\
 % 19000143 &  265.098993 & -53.656813 &  5727 $\pm$ 11 &  3.53  &  -2.13 $\pm$ 0.02 &   0 \\
 % 22000112 &  265.235195 & -53.661234 &  6351 $\pm$ 10 &  4.02  &  -2.27 $\pm$ 0.04 &   0 \\
 %    12627 &  265.126726 & -53.661985 &  6404 $\pm$ 13 &  4.17  &   -2.2 $\pm$ 0.05 &   0 \\
 % 20000240 &  265.118720 & -53.683849 &   5165 $\pm$ 7 &  2.11  &  -2.12 $\pm$ 0.01 &   0 \\
 %     7644 &  265.139832 & -53.682991 &  6458 $\pm$ 15 &  4.13  &  -2.37 $\pm$ 0.08 &   0 \\
 %     8269 &  265.224413 & -53.671025 &  6415 $\pm$ 15 &  4.17  &  -2.31 $\pm$ 0.07 &   0 \\
 %     5939 &  265.173645 & -53.677296 &  5998 $\pm$ 14 &  3.76  &   -2.4 $\pm$ 0.04 &   0 \\
 % 15000140 &  265.209770 & -53.652177 &  5412 $\pm$ 10 &  2.83  &   -2.1 $\pm$ 0.02 &   0 \\
 %     9459 &  265.191873 & -53.670436 &  6258 $\pm$ 14 &  3.98  &  -2.33 $\pm$ 0.06 &   0 \\
 %     4760 &  265.190429 & -53.674252 &   5125 $\pm$ 8 &  2.04  &  -2.17 $\pm$ 0.01 &   0 \\
 %    13228 &  265.204814 & -53.653103 &  5994 $\pm$ 12 &  3.82  &  -2.31 $\pm$ 0.04 &   1 \\
 %    11517 &  265.157649 & -53.670082 &  6227 $\pm$ 13 &  3.93  &  -2.19 $\pm$ 0.05 &   0 \\
 % 12000038 &  265.153780 & -53.725666 &  6393 $\pm$ 13 &  4.17  &  -2.52 $\pm$ 0.06 &   0 \\
 % 16000087 &  265.175032 & -53.633729 &  6268 $\pm$ 10 &  3.91  &  -2.26 $\pm$ 0.04 &   0 \\
 % 19000180 &  265.109741 & -53.658004 &  6355 $\pm$ 13 &  4.14  &  -2.28 $\pm$ 0.05 &   0 \\
 %    12823 &  265.118545 & -53.670505 &  6400 $\pm$ 15 &  4.14  &   -2.3 $\pm$ 0.07 &   0 \\
 %     9125 &  265.199707 & -53.665142 &  6412 $\pm$ 16 &  4.19  &  -2.56 $\pm$ 0.08 &   0 \\
 %     6509 &  265.165278 & -53.680188 &  5974 $\pm$ 21 &  3.74  &  -2.06 $\pm$ 0.06 &   0 \\
 %    16086 &  265.158604 & -53.644957 &  6331 $\pm$ 12 &  4.08  &  -2.58 $\pm$ 0.05 &   0 \\
 % 15000092 &  265.196038 & -53.640376 &   5296 $\pm$ 9 &   2.5  &  -2.11 $\pm$ 0.01 &   0 \\
 %    14401 &  265.169800 & -53.647457 &  5377 $\pm$ 11 &  2.67  &  -2.24 $\pm$ 0.02 &   0 \\
 %     5241 &  265.181830 & -53.684920 &  6242 $\pm$ 20 &  3.94  &  -2.26 $\pm$ 0.07 &   0 \\
 %    12406 &  265.134827 & -53.664463 &  6241 $\pm$ 24 &  3.97  &  -2.33 $\pm$ 0.09 &   0 \\
 %    12020 &  265.146786 & -53.661912 &   5069 $\pm$ 3 &  1.66  &  -2.03 $\pm$ 0.01 &   0 \\
 %      154 &  265.168914 & -53.709157 &  5991 $\pm$ 14 &  3.78  &  -2.24 $\pm$ 0.04 &   0 \\
 %     9900 &  265.183481 & -53.667071 &  6211 $\pm$ 23 &  4.06  &   -2.98 $\pm$ 0.1 &   0 \\
 %     1846 &  265.175582 & -53.688516 &  6227 $\pm$ 14 &  3.94  &  -2.23 $\pm$ 0.05 &   0 \\
 %     5366 &  265.180700 & -53.674237 &  6027 $\pm$ 20 &  3.71  &  -2.05 $\pm$ 0.05 &   0 \\
 %     5031 &  265.185635 & -53.679897 &   5312 $\pm$ 9 &  2.35  &  -2.17 $\pm$ 0.01 &   0 \\
 %     7660 &  265.139435 & -53.675140 &  5500 $\pm$ 10 &  3.01  &  -2.19 $\pm$ 0.02 &   0 \\
 %     3979 &  265.209534 & -53.675743 &  6398 $\pm$ 32 &  4.19  &  -2.19 $\pm$ 0.13 &   0 \\
 %    15648 &  265.192616 & -53.641792 &  6348 $\pm$ 27 &  4.12  &   -2.3 $\pm$ 0.11 &   0 \\
 %     1963 &  265.171783 & -53.689514 &  5656 $\pm$ 13 &  3.48  &  -2.23 $\pm$ 0.03 &   0 \\
 %    14968 &  265.152285 & -53.650825 &  6281 $\pm$ 10 &  3.94  &  -2.22 $\pm$ 0.04 &   0 \\
 % 11000340 &  265.125417 & -53.689967 &  6112 $\pm$ 12 &   3.8  &  -2.15 $\pm$ 0.04 &   0 \\
 %    11011 &  265.167755 & -53.661633 &  5402 $\pm$ 12 &  2.75  &   -2.2 $\pm$ 0.02 &   0 \\
 %    15994 &  265.170180 & -53.645725 &  6274 $\pm$ 12 &  4.01  &  -2.31 $\pm$ 0.05 &   0 \\
 %     9880 &  265.183939 & -53.663271 &   5409 $\pm$ 9 &  2.91  &   -2.1 $\pm$ 0.02 &   0 \\
 %     4695 &  265.191193 & -53.685570 &  6328 $\pm$ 15 &  4.05  &  -2.51 $\pm$ 0.07 &   0 \\
 %     9871 &  265.184362 & -53.665967 &  6446 $\pm$ 19 &  4.19  &  -2.28 $\pm$ 0.09 &   0 \\
 %     9149 &  265.199005 & -53.670391 &  6315 $\pm$ 14 &  4.06  &  -2.51 $\pm$ 0.06 &   0 \\
 % 21000185 &  265.246203 & -53.687587 &  6305 $\pm$ 11 &  3.97  &  -2.51 $\pm$ 0.05 &   0 \\
 %    10591 &  265.173462 & -53.671070 &  6148 $\pm$ 12 &  3.83  &  -2.43 $\pm$ 0.05 &   0 \\
 %     5627 &  265.177418 & -53.675978 &  6384 $\pm$ 21 &  4.18  &  -2.29 $\pm$ 0.09 &   0 \\
 %    14107 &  265.177399 & -53.657707 &  5919 $\pm$ 14 &  3.75  &  -2.49 $\pm$ 0.05 &   0 \\
 % 15000007 &  265.202091 & -53.644879 &  6387 $\pm$ 14 &  4.17  &  -2.36 $\pm$ 0.06 &   0 \\
 %     5748 &  265.175903 & -53.676903 &  6375 $\pm$ 16 &   4.2  &  -2.41 $\pm$ 0.07 &   1 \\
 % 22000017 &  265.234556 & -53.672099 &  6344 $\pm$ 12 &  4.08  &  -2.38 $\pm$ 0.05 &   0 \\
 %    11224 &  265.163452 & -53.670502 &  5968 $\pm$ 11 &  3.73  &  -2.31 $\pm$ 0.03 &   0 \\
 %     6638 &  265.163086 & -53.683800 &  6341 $\pm$ 14 &  4.09  &  -2.45 $\pm$ 0.07 &   0 \\
 % 12000122 &  265.152377 & -53.726071 &  5841 $\pm$ 11 &  3.62  &  -2.21 $\pm$ 0.03 &   0 \\
 %     7656 &  265.139852 & -53.677480 &  6395 $\pm$ 15 &   4  &  -2.22 $\pm$ 0.06 &   0 \\
 % 22000081 &  265.230971 & -53.669612 &  5622 $\pm$ 10 &  3.27  &  -2.08 $\pm$ 0.02 &   0 \\
 %     6572 &  265.164386 & -53.682900 &  5807 $\pm$ 19 &  3.59  &  -2.18 $\pm$ 0.05 &   0 \\
 %     2772 &  265.150452 & -53.691303 &  5710 $\pm$ 14 &  3.54  &  -2.24 $\pm$ 0.03 &   0 \\
 %    11386 &  265.160919 & -53.668404 &  5860 $\pm$ 19 &  3.64  &  -2.33 $\pm$ 0.05 &   0 \\
 %    14182 &  265.175598 & -53.653450 &  6344 $\pm$ 14 &  4.05  &  -2.35 $\pm$ 0.07 &   0 \\
 %     1288 &  265.189697 & -53.688675 &  6366 $\pm$ 14 &  4.12  &  -2.57 $\pm$ 0.07 &   0 \\
 %     5166 &  265.182831 & -53.679150 &  6385 $\pm$ 16 &  4.15  &  -2.56 $\pm$ 0.08 &   0 \\
 % 19000095 &  265.097141 & -53.663352 &  5594 $\pm$ 10 &  3.38  &   -2.1 $\pm$ 0.02 &   0 \\
 % 13000068 &  265.193038 & -53.708358 &  6434 $\pm$ 14 &  4.18  &  -2.36 $\pm$ 0.06 &   0 \\
 %    12916 &  265.115482 & -53.664866 &  6401 $\pm$ 12 &  4.14  &  -2.14 $\pm$ 0.05 &   0 \\
 % 19000081 &  265.096680 & -53.665327 &  6337 $\pm$ 13 &  4.18  &  -2.39 $\pm$ 0.06 &   0 \\
 % 16000131 &  265.171445 & -53.630661 &  5700 $\pm$ 11 &  3.46  &  -2.12 $\pm$ 0.02 &   0 \\
 %     6509 &  265.165283 & -53.680187 &  5993 $\pm$ 13 &  3.74  &  -2.48 $\pm$ 0.05 &   0 \\
 %    10847 &  265.170044 & -53.668991 &  6320 $\pm$ 14 &  3.94  &  -2.62 $\pm$ 0.06 &   0 \\
 %    12020 &  265.146790 & -53.661911 &   5096 $\pm$ 5 &  1.66  &  -2.15 $\pm$ 0.01 &   0 \\
 %     5661 &  265.176414 & -53.679142 &  6383 $\pm$ 34 &  4.12  &  -2.01 $\pm$ 0.11 &   0 \\
 %    11433 &  265.159632 & -53.670355 &  6417 $\pm$ 32 &  4.15  &  -1.72 $\pm$ 0.08 &   0 \\
 %     6063 &  265.171783 & -53.681339 &  6425 $\pm$ 17 &  4.09  &  -2.79 $\pm$ 0.09 &   0 \\
 % 13000098 &  265.184811 & -53.708192 &  6370 $\pm$ 15 &  4.18  &  -2.22 $\pm$ 0.06 &   0 \\
 %     7547 &  265.142609 & -53.676849 &  5646 $\pm$ 12 &  3.29  &  -2.21 $\pm$ 0.03 &   0 \\
 %    11549 &  265.157074 & -53.664093 &  6334 $\pm$ 24 &  3.98  &  -2.34 $\pm$ 0.11 &   0 \\
 %    14319 &  265.171994 & -53.655952 &  5858 $\pm$ 16 &   3.7  &  -2.24 $\pm$ 0.04 &   0 \\
 %     4121 &  265.205048 & -53.676937 &  6427 $\pm$ 15 &  4.06  &  -2.56 $\pm$ 0.08 &   0 \\
 %     7209 &  265.151221 & -53.679475 &  6399 $\pm$ 22 &  4.16  &  -2.51 $\pm$ 0.11 &   0 \\
 %     4620 &  265.192932 & -53.682777 &  6216 $\pm$ 13 &  3.88  &  -2.26 $\pm$ 0.05 &   0 \\
 %    10829 &  265.170441 & -53.661190 &  6424 $\pm$ 27 &  4.08  &  -2.92 $\pm$ 0.14 &   0 \\
 %    14830 &  265.156737 & -53.657208 &  6363 $\pm$ 16 &  4.15  &  -2.56 $\pm$ 0.07 &   0 \\
 % 23000575 &  265.225419 & -53.657770 &  6270 $\pm$ 22 &  3.85  &   -2.47 $\pm$ 0.1 &   0 \\
 % 17000661 &  265.146367 & -53.641082 &  6388 $\pm$ 13 &  4.18  &  -2.37 $\pm$ 0.05 &   0 \\
 %     7209 &  265.151215 & -53.679474 &  6317 $\pm$ 20 &  4.16  &   -2.79 $\pm$ 0.1 &   0 \\
 %     4440 &  265.197357 & -53.675968 &  5645 $\pm$ 14 &  3.42  &  -2.38 $\pm$ 0.04 &   0 \\
 %     4649 &  265.192200 & -53.677902 &  6098 $\pm$ 28 &  3.77  &  -2.17 $\pm$ 0.09 &   0 \\
 % 22000358 &  265.232225 & -53.681480 &  5107 $\pm$ 28 &   0  &  -2.65 $\pm$ 0.08 &   0 \\
 % 24000160 &  265.185694 & -53.631769 &  6407 $\pm$ 12 &  4.18  &  -2.56 $\pm$ 0.06 &   0 \\
 %     9612 &  265.189059 & -53.665136 &  6306 $\pm$ 14 &  3.95  &  -2.29 $\pm$ 0.06 &   0 \\
 %    11547 &  265.157325 & -53.665917 &   5045 $\pm$ 3 &  1.46  &  -1.87 $\pm$ 0.01 &   0 \\
 %      336 &  265.159882 & -53.704506 &  6142 $\pm$ 15 &  3.88  &  -2.51 $\pm$ 0.06 &   0 \\
 %     3816 &  265.214264 & -53.676525 &  6488 $\pm$ 15 &  4.11  &  -2.56 $\pm$ 0.08 &   0 \\
 %     5872 &  265.174043 & -53.686823 &  6292 $\pm$ 19 &  4.18  &  -2.47 $\pm$ 0.08 &   0 \\
 %     1662 &  265.179489 & -53.691995 &  5734 $\pm$ 12 &  3.62  &  -2.27 $\pm$ 0.03 &   0 \\
 %     7463 &  265.145203 & -53.673973 &  6475 $\pm$ 15 &  4.03  &  -2.91 $\pm$ 0.08 &   0 \\
 %    10747 &  265.171539 & -53.672127 &  5479 $\pm$ 10 &   3  &  -2.25 $\pm$ 0.02 &   0 \\
 %     5451 &  265.179256 & -53.674465 &  6407 $\pm$ 24 &  4.07  &  -2.02 $\pm$ 0.08 &   0 \\
 %    11282 &  265.162730 & -53.666175 &  6152 $\pm$ 13 &  3.94  &   -2.4 $\pm$ 0.05 &   0 \\
 %    14338 &  265.171478 & -53.652283 &  6581 $\pm$ 11 &  3.63  &   -2.5 $\pm$ 0.06 &   0 \\
 %     9900 &  265.183472 & -53.667072 &  6404 $\pm$ 16 &  4.06  &  -2.66 $\pm$ 0.09 &   0 \\
 % 11000060 &  265.125589 & -53.693856 &  6399 $\pm$ 14 &  4.11  &  -2.19 $\pm$ 0.06 &   0 \\
 %     9913 &  265.183512 & -53.662167 &  6473 $\pm$ 21 &  4.18  &   -2.1 $\pm$ 0.08 &   0 \\
 %     6565 &  265.164264 & -53.686089 &   5060 $\pm$ 3 &  1.66  &  -2.06 $\pm$ 0.01 &   0 \\
 %    11615 &  265.155426 & -53.672951 &  5903 $\pm$ 13 &  3.71  &  -2.27 $\pm$ 0.04 &   0 \\
 %    14830 &  265.156738 & -53.657207 &  6588 $\pm$ 25 &  4.15  &  -1.87 $\pm$ 0.08 &   0 \\
 % 17000019 &  265.144921 & -53.644539 &  6431 $\pm$ 12 &  4.16  &  -2.26 $\pm$ 0.05 &   0 \\
 %     9306 &  265.195432 & -53.663575 &  6050 $\pm$ 13 &  3.81  &  -2.17 $\pm$ 0.04 &   0 \\
 %     9364 &  265.194336 & -53.665417 &  6360 $\pm$ 15 &  4.12  &  -2.47 $\pm$ 0.07 &   0 \\
 % 14000278 &  265.217968 & -53.700392 &  6319 $\pm$ 18 &  4.03  &  -2.29 $\pm$ 0.08 &   0 \\
 % 13000038 &  265.182141 & -53.713544 &  6456 $\pm$ 12 &  4.08  &  -2.54 $\pm$ 0.06 &   0 \\
 %    14798 &  265.157876 & -53.652048 &  6320 $\pm$ 33 &  4.13  &  -2.53 $\pm$ 0.16 &   0 \\
 %     1205 &  265.191957 & -53.687775 &  5783 $\pm$ 13 &  3.62  &  -2.21 $\pm$ 0.03 &   0 \\
 %     8656 &  265.211165 & -53.662162 &  5584 $\pm$ 29 &  2.95  &  -1.68 $\pm$ 0.05 &   0 \\
 % 12000148 &  265.146355 & -53.721789 &  6041 $\pm$ 10 &  3.75  &  -2.25 $\pm$ 0.03 &   0 \\
 %    11801 &  265.152374 & -53.660110 &  6191 $\pm$ 20 &  3.84  &  -2.47 $\pm$ 0.08 &   0 \\
 %     2687 &  265.152466 & -53.694660 &  6392 $\pm$ 16 &   4.1  &  -2.43 $\pm$ 0.07 &   0 \\
 %    14319 &  265.171997 & -53.655952 &  5896 $\pm$ 25 &   3.7  &  -2.38 $\pm$ 0.08 &   0 \\
 %    10552 &  265.175110 & -53.660034 &  6096 $\pm$ 20 &  3.86  &  -2.23 $\pm$ 0.06 &   0 \\
 % 21000286 &  265.243416 & -53.676769 &  5687 $\pm$ 12 &  3.46  &  -2.13 $\pm$ 0.02 &   0 \\
 %     7747 &  265.136676 & -53.686569 &  6337 $\pm$ 19 &  4.12  &   -2.58 $\pm$ 0.1 &   0 \\
 %    10235 &  265.178589 & -53.672546 &  6419 $\pm$ 14 &  4.07  &  -2.69 $\pm$ 0.08 &   0 \\
 %    10325 &  265.177063 & -53.671066 &  6377 $\pm$ 14 &  4.14  &  -2.51 $\pm$ 0.07 &   0 \\
 %    10445 &  265.175897 & -53.664576 &   5201 $\pm$ 8 &  2.27  &  -2.11 $\pm$ 0.01 &   0 \\
 %     6606 &  265.163497 & -53.681687 &  6228 $\pm$ 13 &  3.91  &   -2.3 $\pm$ 0.05 &   0 \\
 %    15609 &  265.195753 & -53.641891 &  6045 $\pm$ 21 &  3.82  &  -1.98 $\pm$ 0.05 &   0 \\
 % 22000352 &  265.239035 & -53.663123 &   5019 $\pm$ 4 &  1.19  &  -1.87 $\pm$ 0.01 &   0 \\
 %     7522 &  265.143368 & -53.680594 &  6284 $\pm$ 17 &  4.13  &  -2.38 $\pm$ 0.06 &   0 \\
 % 19000340 &  265.104139 & -53.668243 &  6034 $\pm$ 12 &  3.74  &  -2.26 $\pm$ 0.04 &   0 \\
 % 15000003 &  265.209691 & -53.649073 &  5611 $\pm$ 12 &  3.43  &  -1.97 $\pm$ 0.02 &   0 \\
 % 14000488 &  265.196758 & -53.705647 &  6334 $\pm$ 22 &  4.19  &   -2.55 $\pm$ 0.1 &   0 \\
 %    14136 &  265.176544 & -53.651989 &  6324 $\pm$ 17 &  4.08  &  -2.47 $\pm$ 0.08 &   0 \\
 % 23000054 &  265.226678 & -53.661866 &  6321 $\pm$ 12 &  4.16  &  -2.11 $\pm$ 0.04 &   0 \\
 %    10348 &  265.176896 & -53.661035 &  6243 $\pm$ 16 &  3.99  &  -2.11 $\pm$ 0.05 &   0 \\
 %    11174 &  265.165149 & -53.663344 &  5576 $\pm$ 11 &  3.34  &   -2.2 $\pm$ 0.02 &   0 \\
 % 13000024 &  265.183015 & -53.716473 &  6363 $\pm$ 13 &  4.08  &  -2.31 $\pm$ 0.05 &   0 \\
 %     9594 &  265.189117 & -53.672558 &  6457 $\pm$ 22 &  4.05  &   -3  &   0 \\
 %     9548 &  265.190063 & -53.666218 &  6153 $\pm$ 12 &  3.86  &  -2.45 $\pm$ 0.05 &   0 \\
 %     7403 &  265.146088 & -53.681866 &  6431 $\pm$ 15 &  4.13  &  -2.49 $\pm$ 0.07 &   0 \\
 %     4958 &  265.186373 & -53.683294 &  6402 $\pm$ 13 &  4.03  &  -2.56 $\pm$ 0.07 &   0 \\
 %    14926 &  265.153881 & -53.654381 &  6280 $\pm$ 13 &  3.99  &  -2.28 $\pm$ 0.05 &   0 \\
 % 22000101 &  265.238285 & -53.665420 &  6206 $\pm$ 11 &   3.9  &  -2.24 $\pm$ 0.04 &   0 \\
 % 24000302 &  265.204354 & -53.630218 &  6122 $\pm$ 15 &  3.89  &  -2.19 $\pm$ 0.05 &   0 \\
 %     9910 &  265.183746 & -53.662735 &  5773 $\pm$ 15 &  3.61  &  -2.29 $\pm$ 0.04 &   0 \\
 %     7519 &  265.143433 & -53.682961 &  6372 $\pm$ 17 &   4.1  &  -2.63 $\pm$ 0.09 &   0 \\
 %     4648 &  265.192627 & -53.678528 &  6359 $\pm$ 19 &  4.05  &  -2.47 $\pm$ 0.09 &   0 \\
 %    11982 &  265.148163 & -53.667683 &  6314 $\pm$ 16 &  4.19  &  -2.69 $\pm$ 0.08 &   0 \\
 %    11745 &  265.153198 & -53.673069 &  6131 $\pm$ 23 &  3.94  &   -2.58 $\pm$ 0.1 &   0 \\
 %    14589 &  265.164520 & -53.653339 &  6192 $\pm$ 20 &  3.93  &  -2.39 $\pm$ 0.08 &   0 \\
 %    11682 &  265.154351 & -53.671889 &  5509 $\pm$ 12 &  2.99  &  -2.06 $\pm$ 0.02 &   0 \\
 %     9229 &  265.197327 & -53.663483 &   5046 $\pm$ 3 &  1.29  &  -1.96 $\pm$ 0.01 &   0 \\
 %     6698 &  265.162109 & -53.679176 &   5129 $\pm$ 9 &  1.94  &  -2.18 $\pm$ 0.02 &   0 \\
 %     1201 &  265.191567 & -53.689852 &  6179 $\pm$ 13 &  3.87  &  -2.26 $\pm$ 0.04 &   0 \\
 %     4778 &  265.190216 & -53.681446 &  6216 $\pm$ 13 &   3.9  &  -2.46 $\pm$ 0.05 &   0 \\
 %     1916 &  265.173065 & -53.697388 &  6261 $\pm$ 13 &  3.92  &  -2.24 $\pm$ 0.05 &   0 \\
 %     2097 &  265.168427 & -53.695866 &  6418 $\pm$ 16 &  4.11  &  -2.74 $\pm$ 0.08 &   0 \\
 % 11000211 &  265.124640 & -53.686619 &  6373 $\pm$ 10 &  4.04  &  -2.24 $\pm$ 0.04 &   0 \\
 % 14000020 &  265.201539 & -53.699970 &  6319 $\pm$ 12 &   4  &  -2.42 $\pm$ 0.06 &   0 \\
 %     1807 &  265.175751 & -53.695564 &  6459 $\pm$ 16 &  4.13  &   -3  &   0 \\
 %    14763 &  265.159119 & -53.656364 &  6467 $\pm$ 24 &  4.08  &  -2.31 $\pm$ 0.12 &   0 \\
 %     2338 &  265.162231 & -53.699383 &  5363 $\pm$ 10 &  2.63  &  -2.23 $\pm$ 0.02 &   0 \\
 %     3437 &  265.226257 & -53.676968 &  6214 $\pm$ 35 &  3.87  &  -2.32 $\pm$ 0.14 &   0 \\
 %     1105 &  265.194509 & -53.689708 &  5586 $\pm$ 14 &  3.45  &  -2.06 $\pm$ 0.03 &   0 \\
 %     5693 &  265.176608 & -53.674514 &  6422 $\pm$ 32 &  4.03  &  -2.64 $\pm$ 0.18 &   0 \\
 %    11514 &  265.157978 & -53.673105 &  6344 $\pm$ 22 &  4.17  &    -2.4 $\pm$ 0.1 &   1 \\
 %     8443 &  265.217224 & -53.669155 &  6409 $\pm$ 19 &  4.18  &  -2.51 $\pm$ 0.09 &   0 \\
 %    14758 &  265.159147 & -53.658677 &  6437 $\pm$ 16 &  4.15  &  -2.05 $\pm$ 0.06 &   0 \\
 %     6080 &  265.172058 & -53.676105 &  6194 $\pm$ 12 &  3.86  &  -2.48 $\pm$ 0.05 &   0 \\
 %     1330 &  265.188580 & -53.690542 &  6218 $\pm$ 17 &  3.91  &  -2.42 $\pm$ 0.07 &   0 \\
 %     5580 &  265.177989 & -53.676405 &  5496 $\pm$ 10 &   3  &  -2.21 $\pm$ 0.02 &   0 \\
 %    11687 &  265.154419 & -53.670368 &  6235 $\pm$ 37 &  4.19  &  -2.57 $\pm$ 0.17 &   0 \\
 %    15979 &  265.172329 & -53.639768 &  6325 $\pm$ 11 &  4.02  &  -2.25 $\pm$ 0.04 &   0 \\
 %    13475 &  265.195587 & -53.654587 &  6163 $\pm$ 16 &   4  &  -2.43 $\pm$ 0.06 &   1 \\
 %     1938 &  265.172699 & -53.696274 &  5977 $\pm$ 13 &  3.73  &  -2.47 $\pm$ 0.05 &   0 \\
 %    13196 &  265.206099 & -53.651106 &  5745 $\pm$ 17 &  3.53  &  -2.07 $\pm$ 0.04 &   0 \\
 %     3818 &  265.214233 & -53.675480 &   5141 $\pm$ 9 &  1.98  &  -2.11 $\pm$ 0.02 &   0 \\
 %     2582 &  265.155304 & -53.701107 &  6354 $\pm$ 15 &  3.95  &  -2.43 $\pm$ 0.07 &   0 \\
 % 22000209 &  265.238536 & -53.666474 &  5558 $\pm$ 10 &  3.12  &   -2.1 $\pm$ 0.02 &   0 \\
 %    15659 &  265.192068 & -53.639713 &  6326 $\pm$ 12 &  4.04  &  -2.32 $\pm$ 0.05 &   0 \\
 %     4947 &  265.187378 & -53.675671 &  6393 $\pm$ 18 &  3.99  &  -2.52 $\pm$ 0.09 &   0 \\
 %    13544 &  265.192809 & -53.659836 &   5427 $\pm$ 9 &  2.89  &  -2.08 $\pm$ 0.02 &   0 \\
 %    11419 &  265.160187 & -53.665184 &  6046 $\pm$ 19 &  3.79  &  -2.41 $\pm$ 0.07 &   0 \\
 % 13000130 &  265.192098 & -53.711394 &  6398 $\pm$ 13 &  4.16  &  -2.45 $\pm$ 0.06 &   0 \\
 %     4695 &  265.191193 & -53.685570 &  6374 $\pm$ 16 &  4.05  &  -2.28 $\pm$ 0.07 &   0 \\
 %     7141 &  265.152616 & -53.682696 &  6419 $\pm$ 14 &  4.14  &  -2.17 $\pm$ 0.06 &   0 \\
 %    10447 &  265.175934 & -53.664280 &  6687 $\pm$ 36 &  3.95  &   -3  &   0 \\
 %     9050 &  265.200470 & -53.671455 &   5020 $\pm$ 5 &  1.08  &  -1.89 $\pm$ 0.01 &   0 \\
 %      851 &  265.204097 & -53.689708 &  6416 $\pm$ 19 &  4.16  &  -2.31 $\pm$ 0.09 &   0 \\
 %    13420 &  265.197348 & -53.658670 &  6214 $\pm$ 19 &  3.96  &   -2.4 $\pm$ 0.08 &   0 \\
 %     8485 &  265.216344 & -53.660466 &   5434 $\pm$ 9 &   2.9  &  -2.11 $\pm$ 0.02 &   0 \\
 %     4846 &  265.189065 & -53.680961 &  5781 $\pm$ 12 &  3.59  &  -2.33 $\pm$ 0.03 &   0 \\
 %     1213 &  265.191467 & -53.695850 &  6161 $\pm$ 14 &  3.88  &  -2.68 $\pm$ 0.06 &   0 \\
 %     9753 &  265.185760 & -53.673630 &  6150 $\pm$ 12 &  3.85  &  -2.41 $\pm$ 0.04 &   0 \\
 % 20000133 &  265.116022 & -53.679976 &  5511 $\pm$ 10 &  3.11  &  -2.07 $\pm$ 0.02 &   0 \\
 %     8194 &  265.118368 & -53.676123 &  5604 $\pm$ 11 &  3.36  &  -2.16 $\pm$ 0.02 &   0 \\
 %     1119 &  265.194397 & -53.692093 &  5468 $\pm$ 11 &  2.83  &  -2.15 $\pm$ 0.02 &   0 \\
 %     6929 &  265.157916 & -53.678604 &  5662 $\pm$ 12 &   3.5  &  -2.18 $\pm$ 0.02 &   0 \\
 %     7092 &  265.153855 & -53.683814 &  5528 $\pm$ 10 &  3.17  &  -2.19 $\pm$ 0.02 &   0 \\
 %     9542 &  265.189815 & -53.668709 &  6212 $\pm$ 21 &  3.87  &  -2.25 $\pm$ 0.08 &   0 \\
 % 19000181 &  265.105288 & -53.657601 &  6061 $\pm$ 10 &  3.74  &  -2.22 $\pm$ 0.03 &   0 \\
 %     7202 &  265.151520 & -53.681282 &  6357 $\pm$ 13 &  4.03  &  -2.43 $\pm$ 0.06 &   0 \\
 %     3540 &  265.222137 & -53.679680 &  6327 $\pm$ 15 &  3.99  &  -2.54 $\pm$ 0.07 &   0 \\
 % 21000246 &  265.243127 & -53.688025 &  6301 $\pm$ 11 &  3.94  &  -2.32 $\pm$ 0.05 &   0 \\
 %     5166 &  265.182834 & -53.679151 &  6284 $\pm$ 18 &  4.15  &   -2.7 $\pm$ 0.09 &   0 \\
 % 15000319 &  265.201134 & -53.635640 &  6478 $\pm$ 23 &  4.15  &  -2.13 $\pm$ 0.09 &   0 \\
 %     6132 &  265.171143 & -53.675144 &  6403 $\pm$ 13 &  4.17  &  -2.49 $\pm$ 0.06 &   0 \\
 %    14798 &  265.157876 & -53.652048 &  6363 $\pm$ 18 &  4.13  &  -2.33 $\pm$ 0.08 &   0 \\
 %    10554 &  265.174072 & -53.673222 &  5326 $\pm$ 11 &  2.47  &  -2.14 $\pm$ 0.02 &   0 \\
 % 23000083 &  265.225445 & -53.658580 &  5582 $\pm$ 10 &  3.36  &  -2.16 $\pm$ 0.02 &   0 \\
 %     9035 &  265.201393 & -53.664233 &  6273 $\pm$ 12 &   4  &  -2.07 $\pm$ 0.04 &   1 \\
 %     9548 &  265.190052 & -53.666218 &  6233 $\pm$ 13 &  3.86  &  -2.23 $\pm$ 0.05 &   0 \\
 %     9253 &  265.196411 & -53.662556 &  5469 $\pm$ 11 &  2.95  &  -2.16 $\pm$ 0.02 &   0 \\
 %     7289 &  265.149200 & -53.678188 &  6430 $\pm$ 15 &  4.17  &  -2.79 $\pm$ 0.08 &   0 \\
 %    10062 &  265.181168 & -53.664361 &  6418 $\pm$ 15 &  4.06  &   -2.2 $\pm$ 0.06 &   0 \\
 %    11392 &  265.161011 & -53.665447 &  6171 $\pm$ 21 &  3.85  &  -2.52 $\pm$ 0.09 &   0 \\
 %    10307 &  265.178040 & -53.660362 &  6388 $\pm$ 27 &  4.14  &  -2.64 $\pm$ 0.13 &   0 \\
 % 22000044 &  265.239926 & -53.675102 &  5570 $\pm$ 11 &  3.31  &  -2.05 $\pm$ 0.02 &   1 \\
 %    14833 &  265.156586 & -53.655487 &  5927 $\pm$ 18 &  3.68  &   -2.2 $\pm$ 0.05 &   0 \\
 %     3167 &  265.238878 & -53.683047 &  5466 $\pm$ 10 &  3.09  &  -2.09 $\pm$ 0.02 &   0 \\
 %     6329 &  265.168365 & -53.676243 &  6428 $\pm$ 14 &  4.17  &  -2.55 $\pm$ 0.07 &   0 \\
 %     9024 &  265.201019 & -53.669941 &  6337 $\pm$ 14 &  4.02  &  -2.32 $\pm$ 0.06 &   0 \\
 %    14213 &  265.174469 & -53.659340 &  6245 $\pm$ 18 &  3.88  &  -2.42 $\pm$ 0.08 &   0 \\
 %     1220 &  265.191395 & -53.690348 &  6283 $\pm$ 14 &  4.05  &  -2.34 $\pm$ 0.06 &   0 \\
 %     5637 &  265.177338 & -53.674664 &  6393 $\pm$ 16 &  4.08  &  -2.34 $\pm$ 0.07 &   0 \\
 %    13728 &  265.187653 & -53.655983 &  6057 $\pm$ 13 &  3.81  &  -2.56 $\pm$ 0.05 &   0 \\
 % 21000154 &  265.238930 & -53.689277 &  6435 $\pm$ 13 &  4.15  &  -2.34 $\pm$ 0.06 &   0 \\
 %     6572 &  265.164398 & -53.682899 &  5757 $\pm$ 16 &  3.59  &  -2.38 $\pm$ 0.04 &   0 \\
 %     1893 &  265.173462 & -53.699589 &  5578 $\pm$ 12 &  3.31  &  -2.21 $\pm$ 0.03 &   0 \\
 %     5018 &  265.185486 & -53.682858 &  5931 $\pm$ 13 &  3.61  &  -2.24 $\pm$ 0.04 &   0 \\
 %     7597 &  265.141632 & -53.676437 &  5941 $\pm$ 14 &  3.69  &  -2.39 $\pm$ 0.04 &   1 \\
 %    11282 &  265.162720 & -53.666176 &  6266 $\pm$ 20 &  3.94  &   -2.69 $\pm$ 0.1 &   0 \\
 %    14429 &  265.168304 & -53.655037 &  6491 $\pm$ 17 &  3.79  &  -2.54 $\pm$ 0.09 &   0 \\
 %     8656 &  265.211151 & -53.662163 &  5755 $\pm$ 30 &  2.95  &  -2.19 $\pm$ 0.07 &   0 \\
 % 24000143 &  265.193294 & -53.620772 &  6354 $\pm$ 17 &  4.07  &  -2.25 $\pm$ 0.07 &   0 \\
 %     1049 &  265.196625 & -53.688007 &  6113 $\pm$ 15 &  3.84  &  -2.12 $\pm$ 0.04 &   0 \\
 %     6697 &  265.162002 & -53.679426 &  5332 $\pm$ 10 &  2.75  &  -2.17 $\pm$ 0.02 &   0 \\
 %     6482 &  265.165863 & -53.677986 &  6374 $\pm$ 19 &  4.05  &  -2.48 $\pm$ 0.11 &   0 \\
 %     5032 &  265.185333 & -53.679729 &  6103 $\pm$ 16 &  3.84  &  -2.35 $\pm$ 0.06 &   0 \\
 % 19000090 &  265.099013 & -53.663969 &  6383 $\pm$ 13 &  4.17  &  -2.36 $\pm$ 0.06 &   0 \\
 %     8817 &  265.207034 & -53.665206 &  6070 $\pm$ 14 &  3.86  &  -2.28 $\pm$ 0.04 &   0 \\
 %     7152 &  265.152679 & -53.678143 &   5585 $\pm$ 8 &  2.37  &  -2.46 $\pm$ 0.02 &   0 \\
 %    14882 &  265.155060 & -53.659479 &  6413 $\pm$ 14 &   4.1  &  -2.46 $\pm$ 0.07 &   0 \\
 % 19000213 &  265.087675 & -53.666981 &  5973 $\pm$ 22 &  3.71  &  -2.18 $\pm$ 0.06 &   0 \\
 %     5212 &  265.182587 & -53.678570 &  5486 $\pm$ 11 &  2.89  &   -2.2 $\pm$ 0.02 &   0 \\
 %     5562 &  265.178040 & -53.680340 &  5797 $\pm$ 13 &  3.62  &  -2.25 $\pm$ 0.03 &   0 \\
 %     9022 &  265.201099 & -53.671011 &  6175 $\pm$ 16 &  3.98  &   -2 $\pm$ 0.04 &   0 \\
 %     7034 &  265.155609 & -53.676289 &  5885 $\pm$ 13 &  3.74  &  -2.39 $\pm$ 0.04 &   0 \\
 % 19000077 &  265.093234 & -53.665803 &  5696 $\pm$ 11 &  3.52  &  -2.15 $\pm$ 0.02 &   0 \\
 %     1594 &  265.181030 & -53.695374 &  6460 $\pm$ 18 &  4.16  &  -2.45 $\pm$ 0.09 &   0 \\
 %    10772 &  265.171173 & -53.664795 &  6244 $\pm$ 32 &   4.1  &  -2.33 $\pm$ 0.13 &   0 \\
 %     6412 &  265.167297 & -53.675369 &  5587 $\pm$ 12 &  3.31  &  -2.14 $\pm$ 0.02 &   0 \\
 %     9358 &  265.194162 & -53.668321 &  5757 $\pm$ 12 &  3.58  &  -2.08 $\pm$ 0.03 &   0 \\
 %     5758 &  265.175751 & -53.676296 &  6454 $\pm$ 12 &  4.03  &   -2.5 $\pm$ 0.06 &   0 \\
 % 15000102 &  265.204025 & -53.638992 &  6437 $\pm$ 11 &  4.12  &  -2.57 $\pm$ 0.06 &   0 \\
 %    10653 &  265.173187 & -53.666718 &  5927 $\pm$ 12 &  3.66  &  -2.17 $\pm$ 0.03 &   0 \\
 %    15961 &  265.173844 & -53.640767 &  6443 $\pm$ 13 &  4.18  &  -2.47 $\pm$ 0.06 &   0 \\
 %    11386 &  265.160905 & -53.668405 &  5910 $\pm$ 13 &  3.64  &   -2 $\pm$ 0.03 &   0 \\
 %     1049 &  265.196613 & -53.688007 &  6181 $\pm$ 16 &  3.84  &  -2.58 $\pm$ 0.07 &   0 \\
 %    11759 &  265.153198 & -53.666210 &  6208 $\pm$ 20 &  3.99  &   -3  &   0 \\
 % 18000198 &  265.114493 & -53.655990 &  6376 $\pm$ 12 &   4.1  &  -2.29 $\pm$ 0.05 &   1 \\
 %     1965 &  265.171631 & -53.688999 &  6318 $\pm$ 16 &  4.07  &  -2.85 $\pm$ 0.08 &   0 \\
 %     4620 &  265.192937 & -53.682777 &  6247 $\pm$ 12 &  3.88  &  -2.42 $\pm$ 0.06 &   0 \\
 %    11906 &  265.149750 & -53.669487 &  6314 $\pm$ 14 &   4.1  &  -2.63 $\pm$ 0.07 &   1 \\
 %      868 &  265.203591 & -53.687782 &   5060 $\pm$ 3 &  1.61  &  -2.01 $\pm$ 0.01 &   0 \\
 % 24000133 &  265.187263 & -53.622997 &  6385 $\pm$ 11 &  4.07  &  -2.34 $\pm$ 0.05 &   0 \\
 %     1120 &  265.194458 & -53.691685 &  6314 $\pm$ 15 &  4.09  &   -2.9 $\pm$ 0.07 &   0 \\
 %    11173 &  265.164787 & -53.664002 &  5943 $\pm$ 15 &  3.73  &  -2.31 $\pm$ 0.04 &   0 \\
 %     5587 &  265.177679 & -53.675042 &  6326 $\pm$ 29 &  4.05  &  -1.93 $\pm$ 0.09 &   0 \\
 % 13000501 &  265.182389 & -53.707961 &  6342 $\pm$ 11 &  4.03  &  -2.43 $\pm$ 0.05 &   0 \\
 % 15000104 &  265.209703 & -53.638638 &  6065 $\pm$ 11 &  3.77  &  -2.37 $\pm$ 0.04 &   0 \\
 %     7194 &  265.151428 & -53.687237 &  6333 $\pm$ 14 &   4  &  -2.74 $\pm$ 0.07 &   0 \\
 % 22000150 &  265.236571 & -53.676358 &  5923 $\pm$ 16 &  3.68  &   -2.4 $\pm$ 0.05 &   0 \\
 %    10552 &  265.175110 & -53.660034 &  6131 $\pm$ 22 &  3.86  &  -2.14 $\pm$ 0.07 &   0 \\
 %    12481 &  265.131805 & -53.665073 &  5686 $\pm$ 15 &  3.53  &  -2.24 $\pm$ 0.04 &   0 \\
 %    12878 &  265.117577 & -53.661330 &  6424 $\pm$ 18 &  4.19  &  -2.28 $\pm$ 0.08 &   0 \\
 %     1609 &  265.180817 & -53.699070 &  6279 $\pm$ 10 &  3.65  &  -2.33 $\pm$ 0.04 &   0 \\
 %      796 &  265.206879 & -53.690479 &  6356 $\pm$ 20 &  4.03  &   -2.55 $\pm$ 0.1 &   0 \\
 %     1793 &  265.176375 & -53.689163 &  6326 $\pm$ 16 &  4.08  &  -2.05 $\pm$ 0.05 &   0 \\
 % 11000063 &  265.131237 & -53.693576 &  6370 $\pm$ 12 &  4.06  &  -2.51 $\pm$ 0.05 &   0 \\
 %     6262 &  265.169739 & -53.674530 &  5459 $\pm$ 10 &  2.92  &   -2.2 $\pm$ 0.02 &   0 \\
 %     4685 &  265.191890 & -53.674613 &  6453 $\pm$ 19 &  4.11  &  -2.22 $\pm$ 0.09 &   0 \\
 %     2493 &  265.157684 & -53.700962 &  5712 $\pm$ 15 &  3.48  &  -2.16 $\pm$ 0.03 &   0 \\
 %     4747 &  265.190723 & -53.680974 &  6072 $\pm$ 13 &   3.8  &  -2.32 $\pm$ 0.04 &   0 \\
 %     4967 &  265.186371 & -53.679169 &  6098 $\pm$ 38 &  3.85  &  -2.51 $\pm$ 0.15 &   0 \\
 %     5909 &  265.174530 & -53.675228 &  5729 $\pm$ 13 &  3.54  &  -2.22 $\pm$ 0.03 &   0 \\
 %    13609 &  265.191864 & -53.648830 &  6193 $\pm$ 14 &  3.88  &  -2.51 $\pm$ 0.06 &   0 \\
 %     8774 &  265.208466 & -53.662148 &  6479 $\pm$ 17 &  4.15  &   -2.7 $\pm$ 0.09 &   0 \\
 % 21000114 &  265.245197 & -53.682556 &  6375 $\pm$ 11 &  4.04  &  -2.28 $\pm$ 0.04 &   0 \\
      851 &  265.204102 & -53.689709 &  6363 $\pm$ 16 &  4.16  &  -2.29 $\pm$ 0.07 &   0 \\
    13360 &  265.199603 & -53.646712 &  5625 $\pm$ 10 &  3.44  &  -2.07 $\pm$ 0.02 &   0 \\
      775 &  265.207814 & -53.694752 &  6387 $\pm$ 12 &  4.09  &  -2.33 $\pm$ 0.05 &   1 \\
 12000001 &  265.150307 & -53.727032 &  6461 $\pm$ 13 &  4.09  &  -2.35 $\pm$ 0.06 &   0 \\
 18000148 &  265.131086 & -53.651625 &  6318 $\pm$ 12 &  4.09  &  -2.15 $\pm$ 0.04 &   0 \\
\hline
\end{tabular}
\tablefoot{The $\logg$ values are fixed to the photometric values and are adopted from H16.}
